FPIM: Field-Programmable Ising Machines for Solving SAT

On-chip analog Ising Machines (IMs) are a promising means to solve difficult combinatorial optimization problems. For scalable on-chip realizations to be practical, 1) the problem should map scalably to Ising form, 2) interconnectivity between spins should be sparse, 3) the number of bits of coupling resolution (BCR) needed for programming interconnection weights should be small, and 4) the chip should be capable of solving problems with different connection topologies. We explore these issues for the SATisfiability problem and devise FPIM, a reconfigurable on-chip analog Ising machine scheme well suited for SAT. To map SAT problems onto FPIMs, we leverage Boolean logic synthesis as a first step, but replace synthesized logic gates with Ising equivalent circuits whose analog dynamics solve SAT by minimizing the Ising Hamiltonian. We apply our approach to 2000 benchmark problems from SATLIB,demonstrating excellent scaling, together with low sparsity and low BCR that are independent of problem scale. Placement/routing reveals a very feasible requirement of less than 10 routing tracks to implement all the benchmarks, translating to an area requirement of about 10mm^2 for a programmable 1000-spin FPIM in 65nm technology.

==> bib/0-README-bibentry-rules-IGNORE-AT-YOUR-OWN-PERIL <==
1. NO DUPLICATION: 

    - Before putting in a new entry, CHECK that it is not already there in any
      of the .bib files:
            - grep -i <terms> *.bib
    - You may move entries from one .bib file to another, but DO NOT DUPLICATE
      ENTRIES

2. COMPLETE BACKWARD COMPATIBILITY: 

    - DO NOT CHANGE THE BibTeX KEY OF ANY EXISTING ENTRY!
      - (even if the entry was authored by you).

3. EMBRACE (or at least OBEY) the following jrgroup BIBTEX CONVENTIONS in your entries:

    - Enter the name of any new conference/journal in stringsdefs.bib. Example:
      - BEFORE YOU DO SO, CHECK THAT ISN'T ALREADY DEFINED:
        - grep -i dac stringdefs.bib
      - Example:
        - @STRING{aeu = {Archiv F\:ur Elektronik und \:Ubertragungstechnik}}

    - Keep string definitions SHORT and SENSIBLE (keeping in mind citation traditions that are brief while being clear - look at the bibliographies of some GOOD papers to get a sense):

        - DON'T make definitions like these:

          - @STRING{aspdac14 = {ASPDAC~'14:~Proceedings of the $19^{th}$ Asia and South Pacific Design Automation Conference}} # too long and too specialized (year or location should NOT be part of the string def; other bibtex fields will fill these in.)

          - @STRING{ADAC = {Proc. of IEEE ASP-DAC}} # neither here nor there

        - instead of the above, DO make definitions like this:

           - @STRING{aspdac = {Proc. IEEE ASP-DAC}}

           - @STRING{aspdacNoHyphen = {Proc. IEEE ASPDAC}}

           - @STRING{aspdaclong = {Proc. IEEE Asia-South Pacific Design Automation Conference}}

           - @STRING{TCAD = {IEEE Trans. Computer-Aided Design}}

           - @STRING{tcad = {IEEE Trans. CAD}}

    
    - Use ONLY string definitions for the workshop/conference/journal name. 
      - Example:
        - @article{myGreatArticle,
             ...,
             journal = aeu,
             ...
          }

    - Keep lists of author names short. Use initials and avoid first and middle names. Also, don't rely on latex/bibtex to format the name list properly; do it yourself, by enclosing in {{ }}. For example:

      - DON'T do these:

        - author={Hisamoto,~D. and Lee,~W.~C. and Kedzierski,~J. and Takeuchi,~H. and Asano,~K. and Kuo,~C. and Anderson,~E. and King,~T.-J. and Bokor,~J. and Hu, ~C.} # this relies on latex/bibtex to format

        - author={Hakim, Roy and Mentovich, Elad D. and Richter, Shachar} # first names AND relying on latex/bibtex to format.

      - instead, do these:

        - author={{D. Hisamoto, W.C. Lee, J. Kedzierski, H. Takeuchi, K. Asano, C. Kuo, E. Anderson, T.-J King, J. Bokor and C. Hu}} 

        - author={{R. Hakim, E.D. Mentovich and S. Richter}}
    
    - titles of bibtex entries: follow the same general idea as for authors, ie, format it yourself and don't rely on latex/bibtex to format. Be careful to make the title look EXACTLY as it appears in the paper, maintaining the correct capitalization. Eg:

      - DON'T do this:
        - title={Introduction to Quantum Mechanics} # some latex styles will show this as "Introduction to quantum mechanics" or even "introduction to quantum mechanics"

      - instead, DO do:
        - title={{Introduction to Quantum Mechanics}}

    - BE CAREFUL ABOUT CASE in BibTeX tags - latex gets confused if there
      are multiple entries differing only in case (and it's hard to debug).

    - DO USE \putDOI: for any article that's available on the web, find its DOI index (google scholar, IEEExplore, etc will tell you), make a valid dx.doi.org URL out of it and put it in _as a note_, thus:

      - note = "\putDOI{\href{http://dx.doi.org/10.1109/JPROC.2010.2070050}{DOI
                      link.}}"

      - DON'T use bibtex fields like url, doi, etc. - they don't work properly in many bibtex styles (such as IEEE). Use note, as above.

      - \putDOI is defined by us, see below. Depending what you want for a given document, you can show the DOI link (clickable in PDF!), or just ignore it (eg, for a shorter bibliography).
    
    - There are a number of newcommands you can/should use in your BibTeX
      entries:

      - See 1-example-paper-template/newcommands-for-bibtex.tex for a list and definitions (see also test-bibs.tex, which contains a subset). Also see
        {jr,aadithya}.bib for examples. Here is a (probably incomplete) list:
        - \presenter{arg}
        - \BP\/ (Best Paper)
        - \BPnom\/ or \BPNOM\/ (Best Paper Nomination)
        - \IP\/ (Invited Paper)
        - \ignore{arg}
        - \putDOI{<DOI link>}
        - \myurl{URL}

    - the first line of each bibtex entry should contain the {, eg,
        @inproceedings{AaRoEtAlICASSP2012DAE2FSM,
        ...
      - Vim syntax highlighting depends on this. DO NOT DO, eg, 
        @inproceedings
        {
        AaRoEtAlICASSP2012DAE2FSM,
        ...

    - Use the following template for your BibTeX entries.
      (Note the naming scheme for the BibTeX key; use something similar)
      - MAKE SURE THE YEAR IS PART OF the key; also the month, preferably.

        % conference was in Kyoto
        @inproceedings{AaRoEtAlICASSP2012DAE2FSM,
          author    = {{\IP\/ K.V. Aadithya,
                       Y. Lin, C. Gu,  A. Xu,
                       \presenter{J. Roychowdhury} and N.R. Shanbhag}},
          title     = {{A Fully Automated Technique For Constructing FSM
                       Abstractions of Non-Ideal Latches in Communication
                       Systems}},
          booktitle = ICASSP,
          year      = 2012,
          month     = Mar,
          pages     = {5289-5292}
        }
      
      - for conference, workshop, and journal entries, make sure the YEAR and
        MONTH are explicitly entered; also for any other entries where it makes
        sense.
      - for conference publications, make sure the PAGES are entered.
      - for journal publications, make sure the VOLUME, NUMBER and PAGES are entered.

4. [TODO: automate this with a perl script] ADD NEW TESTS for new entries to
   test-bibs.tex and CHECK BEFORE COMMITTING.
    - put your newest tests FIRST in the file. 
      - look inside test-bib.tex for illustrative examples.
    - use, eg, a script like script to get a list of tests:
      - echo "\\cite{" > test-von-neumann-jr.tex
      - grep "^@" von-Neumann-jr.bib | sed -e s/.*{// >> test-von-neumann-jr.tex
      - echo "}" >> test-von-neumann-jr.tex
    - edit test-von-neumann-jr.tex manually and check that there are no 
      mistakes (like blank lines) 
    - use '\input{test-von-neumann-jr}' to exercise these bib entries.

5. If you have added any NEW BIB FILES: 
    - make sure you add them to Makefile
        - look inside Makefile for examples. (Eg, search for jr.bib).

6. Run make, and xdvi test-bibs.dvi manually, to make sure it all looks OK.
   - CHECK latex and bibtex messages for any errors. Make sure there are none.
     - look for undefined reference warnings.
   - Make sure there are no [?] citations in your visual examination of the 
     .dvi file.
   - Make sure your new entries appear in the tests!


==> bib/0-quick-vim-tips <==
^O and ^I (jumps forward and back to previous cursor positions, 
    including across files)
gq and qq (justification)

* and #: word search

) : go to the next sentence.

vie, vae: select text delimited by \begin{...} \end{...} - inner and outer

yaourt -S vim-ultisnips: then


==> bib/0-using-latexmk-for-almost-WYSIWYG <==
The short version:

- make sure zathura and xdotool are installed

- git clone vim-tex (vimtex--github-lervag), eg:
  - cd ~/git-managed/
  - git clone git@github.com:lervag/vimtex vimtex--github-lervag

- make vim aware of vimtex:
  - cd ~/.vim/
  - ln -s ~/git-managed/vimtex--github-lervag ./vimtex-git

- add the following to your ~/.vimrc:

    "for use with vim-tex plugin and latexmk
    let g:vimtex_view_method = 'zathura'
    "don't open the quickfix window if there are errors (quickfix_mode=0)
    let g:vimtex_quickfix_mode = 0
    "forward search using gb
    nnoremap <expr><buffer><silent> gb  ':!zathura --synctex-forward '.line(".").':'.col('.').':% ' . shellescape(g:latex#data[b:latex.id].out()) . ' >/dev/null<CR> <C-L>'

- if there is more than one file in your latex document (with a main file top.tex including/inputting other files), then indicate which is the main latex file by making a soft link to it that ends in .latexmain, eg:
  - ln -s top.tex top.tex.latexmain
  This is needed for forward search (\lv) and maybe reverse search (Ctrl-leftclick in the zathura window) to work properly when there are multiple files.
  If you don't do this, and, eg, you are in an included file subfile.tex in gvim and you hit \ll, it will try to find subfile.pdf (and fail), giving you an error message to that effect.

- gvim --servername SOME-ARBITRARY-STRING top.tex
  - and hit \ll (in command mode) to start vimtex compiling the file.
    It should bring up a zathura window.
  - hit \lv in the gvim window for forward search
  - hit Ctrl-leftclick in zathura for reverse search
  - every time you write to the file (with changes), it will recompile (using latexmk) and update the zathura file.

- other possibly useful commands:
    quickfix window/list
    - :cl (shows all latex messages)
    - :cope (opens the quickfix list - just lists warnings/errors)
    - \le - vimtex compile errors
    - \lo - vimtex compile output
    - \lg - vimtex status
    - \lG - vimtex status all



------------------------------------------------------------------------
Date: Thu, 5 May 2016 16:53:59 -0700                                            
From: "A. Gokcen Mahmutoglu" <amahmutoglu@berkeley.edu>                         
To: Jaijeet Roychowdhury <jr@berkeley.edu>                                      
Subject: LaTeX setup                                                            

1. Install vimtex plugin for vim

        https://github.com/lervag/vimtex

   - or yaourt -S vim-vimtex

2. install zathura (pdf viewer -> uses vim keys for navigation) and xdotool

3. Add the following line to your vimrc
 
let g:vimtex_view_method = 'zathura'
    
4. Let latexmk know which is your main latex file:
    There are different methods to do this. My preferred method is to create a file with the '.latexmain' extension.

     For example, if your main file is
          book-top.tex
     Then create an empty file with the name
          book-top.tex.latexmain, i.e.,
                touch book-top.tex.latexmain
   
     and latexmk will know that book-top.tex is your main file.
   

4.5: start vim or gvim on one of your latex files with:
    vim/gvim --servername <myprojectname> file.tex
    - <myprojectname>=VIM tested, works fine

5. Vim shortcuts for compilation

    - hit <leader>ll (usually \ll) in the file: it should start auto-compile
      mode and bring up zathura.
   
    <leader>ll -> compile continuously (once called, it will re-compile the
                  file after a change)

    [
    - vim-tex's viewer start cmd, which \ll calls, needs some setup, but you
      can get by by invoking the following command manually:

      zathura  -x "gvim --servername <myprojectname> --remote +%{line} %{input}"
                                                            thePDFfile.pdf &

    - :VimtexView in gvim also works to start the viewer manually
    ]

    <leader>lv -> view pdf (jumps to the position in pdf that corresponds
        to the position of the cursor in the latex file)
    <leader>li -> shows debugging information in the vim window

6. Zathura shortcut for jumping back from pdf to tex file
   
     ctrl + first mouse button (make sure you click the text and not the white space)

7. quickfix window/list
    - :cl (shows all latex messages)
    - :cope (opens the quickfix list - just lists warnings/errors)
    - \le - vimtex compile errors
    - \lo - vimtex compile output
    - \lg - vimtex status
    - \lG - vimtex status all

8. vimtex help in vim
   - help vimtex


I might have left something out. Call me if something does not work.

Gokcen.

--                                                    

----
From: "A. Gokcen Mahmutoglu" <amahmutoglu@berkeley.edu>
Date: Thu, 5 May 2016 17:08:54 -0700
Subject: Re: LaTeX setup
To: Jaijeet Roychowdhury <jr@berkeley.edu>

Vim has a special key, usually used to call user defined functions. It's
called the "leader". The default leader key is backslash (\). I.e.,
For compilation: \ll
For viewing: \lv

On Thu, May 5, 2016 at 5:05 PM, Jaijeet Roychowdhury <jr@berkeley.edu>
wrote:

> What does <leader> mean, below?
>
>
> --


==> bib/1-example-paper-template/Makefile <==
include Makefile.common # first target all is checkfiles
#
# YOU SHOULD NOT NEED TO CHANGE ANYTHING BELOW: CHANGE ONLY Makefile.common

helpmsg: 
	- @echo "try make [pdf|pdfs|clean|pristine|mrproper]"
	- @echo ""

%.pdf: %.tex $(OTHERSRCS) $(REQDSOFTLINKS)
	@i=1; export TEXINPUTS=$(TEXINPUTS); while [[ $$i -le 4 ]] ; do \
		echo $$i; \
		((i=i+1)); \
		echo TEXINPUTS=.:$(TEXINPUTS) pdflatex $<; \
		TEXINPUTS=.:$(TEXINPUTS) pdflatex $<; \
		BUFILES=bu*.aux; \
		for bufile in $$BUFILES; do \
			echo TEXINPUTS=.:$(TEXINPUTS) bibtex $$bufile; \
			TEXINPUTS=.:$(TEXINPUTS) bibtex $$bufile; \
		done; \
		echo TEXINPUTS=.:$(TEXINPUTS) bibtex $(<:.tex=); \
		TEXINPUTS=.:$(TEXINPUTS) bibtex $(<:.tex=); \
		echo TEXINPUTS=.:$(TEXINPUTS) pdflatex $<; \
		TEXINPUTS=.:$(TEXINPUTS) pdflatex $<; \
	done

pdf pdfs: $(PDFS)
	- @ echo ""
	- @ echo "$^ ready."
	- @ echo "Check that latex shows NO undefined reference or other warnings above."
	- @ echo "Now run xpdf/zathura $^ manually and check that it looks right."
	- @ echo ""

.PHONY: pdfs helpmsg


==> bib/1-example-paper-template/Makefile.latex <==
include Makefile.common # first target all is checkfiles helpmsg

# YOU SHOULD NOT NEED TO CHANGE ANYTHING BELOW: CHANGE ONLY Makefile.common

DVIS = $(TOP:.tex=.dvi)
%.dvi: %.tex $(OTHERSRCS) $(REQDSOFTLINKS)
	@i=1; export TEXINPUTS=$(TEXINPUTS); while [[ $$i -le 4 ]] ; do \
		echo $$i; \
		((i=i+1)); \
		echo TEXINPUTS=.:$(TEXINPUTS) latex $<; \
		TEXINPUTS=.:$(TEXINPUTS) latex $<; \
		BUFILES=bu*.aux; \
		for bufile in $$BUFILES; do \
			echo TEXINPUTS=.:$(TEXINPUTS) bibtex $$bufile; \
			TEXINPUTS=.:$(TEXINPUTS) bibtex $$bufile; \
		done; \
		echo TEXINPUTS=.:$(TEXINPUTS) bibtex $(<:.tex=); \
		TEXINPUTS=.:$(TEXINPUTS) bibtex $(<:.tex=); \
		echo TEXINPUTS=.:$(TEXINPUTS) latex $<; \
		TEXINPUTS=.:$(TEXINPUTS) latex $<; \
	done

include Makefile.dvi-to-ps-to-pdf-rules

# vim: filetype=make


==> bib/1-example-paper-template/SET-UP-NEW-DOCUMENT <==
#!/bin/bash

# call this script to:
# - make all the soft links needed for the Makefile system
# - make all the soft links needed for latex include files
# - copy a skeleton Makefile.config (as Makefile.config-template)

#BIBGIT=$HOME/git-managed/bib--hagrid/
if [[ "$1" == "" ]]; then
    echo "usage: ${0/*\//} <PATH-TO-BIB-GIT>"
    echo "       eg, clone bib-git here (as a submodule, if this is already under git,"
    echo "see 1-example-paper-template/00-README-first for instructions) called ./bib/, and"
    echo "       ${0/*\//} ./bib"
    echo "or, ${0/*\//} ~/git-managed/bib--hagrid/"
    echo ""
    exit 1;
else
    BIBGIT="$1"
fi


MAKEFILES="
    Makefile.common
    Makefile.dvi-to-ps-to-pdf-rules
    Makefile.latex
    Makefile.latexmk
    Makefile.latexmkpdf
    Makefile.pdflatex
"

STYSCLSS="
    llncs.cls
    splncs04.bst
    sscol.cls
    siam10.clo
    siamltex.cls
    siamltex.sty
    algorithm2e.sty
    bibspacing.sty
    proposal.cls
"
# IEEEtran.bst - not recommended. Use the texlive builtin IEEEtran.bst
# IEEEtran.cls - not recommended. Use the texlive builtin IEEEtran.bst
# IEEEtranv1.7a-modified-by-aadithya.cls - 
# IEEEtranv1.7a.cls
# IEEEtranv1.8.cls
# tweaklist.sty - not recommended. enumitem is now used instead

PACKAGESNEWCMDS="
    package-and-newcommand-includes.tex
    package-and-newcommand-includes-llncs.tex
    package-and-newcommand-includes-cambridge.tex
    newcommands-eg-ie-etc.tex
    newcommands-for-bibtex.tex
    newcommands-highlight-ignore-comments-annotations.tex
    newcommands-labels-refs.tex
    newcommands-math.tex
    newcommands-misc.tex
    newcommands-squeeze-spaces.tex
    newcommands-thm-env.tex
    code-inclusion-config.tex
    colour-defs.tex
"

BIBFILES="
    stringdefs.bib
    PHLOGON-jr.bib
    aadithya.bib
    adiabatic-reversible.bib
    ag.bib
    amahmutoglu.bib
    gcj.bib
    jr-disto.bib
    jr.bib
    osc-SHIL-jr.bib
    tianshi.bib
    verification-hybrid-systems-CPS.bib
    von-Neumann-jr.bib
"

for i in $MAKEFILES; do
    ln -s $BIBGIT/1-example-paper-templates/$i .
done

for i in $STYSCLSS; do
    ln -s $BIBGIT/1-example-paper-templates/$i .
done

for i in $PACKAGESNEWCMDS; do
    ln -s $BIBGIT/1-example-paper-templates/$i .
done

echo ""
echo "done setting up soft links."

echo ""
echo "Making a soft link Makefile -> Makefile.latexmkpdf. Please change it, if you like."
ln -s Makefile.latexmkpdf Makefile

if [[ -e Makefile.config-template ]]; then
    echo ""
    echo "Makefile.config-template already exists, not touching it."
else
    echo "TOP = FILLTHISIN" > Makefile.config-template
    echo "OTHERSRCS = "$STYSCLSS $PACKAGESNEWCMDS >> Makefile.config-template
    echo "BIBGIT = $BIBGIT" >> Makefile.config-template 

    echo "SOFTLINKSTOSETUP = \\" >> Makefile.config-template 
    for bibfile in $BIBFILES; do
        echo "      "'$(BIBGIT)/'"$bibfile \\" >> Makefile.config-template 
    done
    echo "" >> Makefile.config-template 
    echo ""
    echo "Please copy Makefile.config-template to Makefile.config and update for your document."
    echo ""
    echo "If you want to dereference all the soft links (eg, for documents to be shared with"
    echo "people who don't have access to bib--github, run deference-softlinks"
    echo "in the directory [bib]/1-example-paper-template/."
    echo ""
fi



==> bib/1-example-paper-template/acronyms-ABCD.tex <==
\begin{acronym}[abcd-cps]
	\acro{IO}[IO]{Input-Output}
	\acro{PD}[PD]{Proportional-Derivative}
	\acro{FSM}[FSM]{Finite State Machine}
	\acro{DAE}[DAE]{Differential Algebraic Equation}
	\acro{DAEs}[DAEs]{Differential Algebraic Equations}
	\acro{AMS}[AMS]{Analog-Mixed Signal}
	\acro{ABCD}[ABCD]{Accurate Booleanization of Continuous Dynamics}
	\acro{MAPP}[MAPP]{Berkeley Model and Algorithm Prototyping Platform}
	\acro{VAPP}[VAPP]{Verilog-A Parser and Processor}
	\acro{MODSPEC}[MODSPEC]{MODel SPECification}
	\acro{CPS}[CPS]{Cyber-Physical Systems}
	\acro{ABCD-CPS}[ABCD-CPS]{\ac{ABCD}-\ac{CPS}}
	\acro{ODE}[ODE]{Ordinary Differential Equation}
	\acro{ODEs}{ODEs}{Ordinary Differential Equations}
	\acro{HJI}[HJI]{Hamilton-Jacobi-Issacs}
	\acro{CTCV}[CT-CV]{Continuous-Time, Continuous-Valued}
	\acro{DTDV}[DT-DV]{Discrete-Time, Discrete-Valued}
\end{acronym}


==> bib/1-example-paper-template/acronyms-STEAM.tex <==
\begin{acronym}[simulation]
        \acro{MNA}[MNA]{Modified Nodal Analysis}
	\acro{STEAM}[STEAM]{Spline-based Tables for Efficient and Accurate device Modelling}
	\acro{PSP}[PSP]{Penn State-Phillips}
	\acro{BSIM}[BSIM]{Berkeley Short-channel IGFET Model}
	\acro{BSIM3}[BSIM3v3.2.4]{Berkeley Short-channel IGFET Model - Version 3.2.4}
	\acro{MVS}[MVS]{MIT Virtual Source}
	\acro{MAPP}[MAPP]{Berkeley Modelling and Prototyping Platform}
        \acro{LMS}[LMS]{Linear Multi-Step}
        \acro{DAE}[DAE]{Differential-Algebraic Equation}
        \acro{GEAR}[GEAR]{GEAR}
        \acro{TRAP}[TRAP]{Trapeziodal}
        \acro{MODSPEC}[MODSPEC]{MODel SPECification}
        \acro{NR}[NR]{Newton-Raphson}
        \acro{wrt}[w.r.t]{with respect to}
\end{acronym}


==> bib/1-example-paper-template/code-inclusion-config.tex <==
\lstloadlanguages{Matlab}
\lstset{language=Matlab,
        frame=single, % Single frame around code
        basicstyle=\scriptsize\ttfamily,
        % keywordstyle=[1]\color{blue}\bf, % Perl functions bold and blue
        keywordstyle=[3]\color{blue}\underbar, % Custom functions underlined and blue
        identifierstyle=, % Nothing special about identifiers                                         
        commentstyle=\usefont{T1}{pcr}{m}{sl}\color{MyDarkGreen}\scriptsize, 
            % Comments are in small dark green courier font
        stringstyle=\color{MyDarkRed}, 
        showstringspaces=false, % Don't put marks in string spaces
        tabsize=4, % 5 spaces per tab
        % 
        % Put standard functions not included in the default language here
        %morekeywords={rand},
        % Put function parameters here
        %morekeywords=[2]{on, off, interp},
        % Put user defined functions here
        %morekeywords=[3]{test},
        %
        morecomment=[l][\color{blue}]{...}, % Line continuation (...) like blue comment
        % numbers=left, % Line numbers on left
        % firstnumber=1, % Line numbers start with line 1
        % numberstyle=\tiny\color{blue}, % Line numbers are blue and small
        % stepnumber=5 % Line numbers go in steps of 5
}

% Creates a new command to include an Matlab script, the first parameter is the
% filename of the script (without .pl), the second parameter is the caption
\newcommand{\matlabscript}[2]{
    \begin{itemize}
    \item[]\lstinputlisting[caption=#2,label=#1]{#1}
    \end{itemize}
}



==> bib/1-example-paper-template/colour-defs.tex <==
% various colours
\definecolor{mylightgrey}{rgb}{0.6,0.6,0.6}
\definecolor{mydarkgrey}{rgb}{0.3,0.3,0.3}
\definecolor{mybrown}{rgb}{0.6,0.2,0}
\definecolor{mylightgreen}{rgb}{0,1,0}
\definecolor{mydarkgreen}{rgb}{0,0.5,0}
\definecolor{MyDarkGreen}{rgb}{0.0,0.4,0.0} % This is the color used for comments
\definecolor{myorange}{rgb}{1,0.4,0}
\definecolor{mypurple}{rgb}{0.8,0,0.8}
\definecolor{MyDarkRed}{rgb}{0.4,0.0,0.0} % This is the color used for strings


==> bib/1-example-paper-template/leeseshia-examples-environment.tex <==
% copied from Lee and Seshia's definitions.tex. JR, 2013/09/02.

% File giving definitions of commands and environments.
% Because of a latex bug with counters, this has to be included
% using \input not \include.
%
% Amount of indent in colored boxes
\def\boxIndent{0.3in}

%--------------------------------------------------------------------------
% Blocks of code and variables
\newcommand{\code}[1]{\texttt{#1}}
%--------------------------------------------------------------------------

% Colors. 
\definecolor{exampleColor}{rgb}{0.85,0.92,1.0}
%\definecolor{exampleColor}{rgb}{0.9, 0.9, 0.9}


%--------------------------------------------------------------------------
% Examples environment 
% NOTE: Because of this line, this has to be included using \input
% not \include.
\newcounter{example}
\numberwithin{example}{chapter}
% Allow the @ character to be part of a name
\makeatletter
\newenvironment{example}{
\refstepcounter{example}
\def\FrameCommand{\colorbox{exampleColor}}
\MakeFramed {\advance\hsize-\width \FrameRestore}
\begin{list}{}{
\setlength{\leftmargin}{\boxIndent}
\setlength{\rightmargin}{0in}}
\item
\textbf{Example \thechapter.\arabic{example}:}
} {
\end{list}
\endMakeFramed
}
% restore the @ character to special status
\makeatother
\renewcommand \theexample {\thechapter.\arabic{example}}

%--------------------------------------------------------------------------
% For examples that are to be kept on one page.
% NOTE: Because of this line, this has to be included using \input
% not \include.
\newcounter{exampleKeep}
% Allow the @ character to be part of a name
\makeatletter
\newenvironment{exampleKeep}{
\refstepcounter{example} % so that the examples are numbered properly for now
\begin{lrbox}{\@tempboxa}
\begin{minipage} {\columnwidth}
\refstepcounter{example}
% Unfortunately, quote also results in the color box not going to the
% right margin.
%\begin{quote}
\begin{list}{}{
\setlength{\leftmargin}{\boxIndent}
\setlength{\rightmargin}{0in}}
\item
\textbf{Example \thechapter.\arabic{example}:}
} {
%\end{quote}
\end{list}
\end{minipage}
\end{lrbox}
\colorbox{exampleColor}{\usebox{\@tempboxa}}
}
\newenvironment{exampleContinued}[1]{
\begin{lrbox}{\@tempboxa}
\begin{minipage} {\columnwidth}
\begin{list}{}{
\setlength{\leftmargin}{\boxIndent}
\setlength{\rightmargin}{0in}}
\item
\textbf{Example \ref{#1} (continued):}
} {
%\end{quote}
\end{list}
\end{minipage}
\end{lrbox}
\colorbox{exampleColor}{\usebox{\@tempboxa}}
}
% restore the @ character to special status
\makeatother
\renewcommand \theexample {\thechapter.\arabic{example}}



==> bib/1-example-paper-template/newcommands-eg-ie-etc.tex <==
% eg, ie, etc, wrt, viz newcommands
\newcommand{\eg}{{\it e.g.\@}} % \@ for normal spacing after. use: \eg\/ or \eg,
\newcommand{\ie}{{\it i.e.\@}} 
\newcommand{\wrt}{{\it w.r.t.\@}}
\newcommand{\viz}{{\it viz.\@}}
\newcommand{\vs}{{\it vs.\@}}
\newcommand{\aka}{{\it aka}}
\newcommand{\apriori}{{\it a priori}}
\newcommand{\adhoc}{{\it ad-hoc}}
\newcommand{\etc}{\textit{etc.\@}}                                                
\newcommand{\perse}{\textit{per se\@}}                                                
\newcommand{\etal}{\textit{et. al.\@}}                                                
% etc defined so that there is only a single period after it if it is followed 
% by a period
% see: http://en.wikibooks.org/wiki/TeX/def                                      
% see: http://www.tug.org/pipermail/texhax/2004-July/002449.html                 
% see: http://en.wikibooks.org/wiki/TeX/if                                       
%\ifx \etc \undefined  DOES NOT WORK
%  %\def\myarg{#1}                                                                
%  %\def\myfullstop{.}                                                            
%  %\def\etc{#1}{\textit{etc} arg is ``\myarg'' \ifx\myarg\myfullstop\then.\else.#1\fi\/}
%\fi                                                                              
%\def\etc#1{\textit{etc}\ifx#1..\else.#1\fi} % WORKS                                     
%                        


==> bib/1-example-paper-template/newcommands-for-bibtex.tex <==
\newcommand{\BP}{({\textbf{Best Paper}})} % used in bibliography
\newcommand{\BPnom}{({\textbf{Best Paper Nomination}})} % used in bibliography
\newcommand{\IP}{({\textbf{Invited}})} % used in bibliography
\newcommand{\presenter}[1]{#1} % used in bibliography
%\newcommand{\putDOI}[1]{#1}
\newcommand{\putDOI}[1]{}
\newcommand{\DP}{\textbf{(Distinguished Paper)}}


==> bib/1-example-paper-template/newcommands-highlight-ignore-comments-annotations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% newcommands for ignoring, commenting, annotating, highlighting
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ignore}[1]{}
\let\IGNORE=\ignore
%\newcommand{\comment}[1]{} % conflicts with something predefined
\newcommand{\COMMENT}[1]{}
\newcommand{\jrcomment}[1]{{\color{blue}#1}}
\newcommand{\agcomment}[1]{{\color{mydarkgreen}#1}}
\let\agc=\agcomment
\let\jc=\jrcomment
\newcommand{\redHL}[1]{{\color{red}\bf #1}}
\newcommand{\REDHL}[1]{{\color{red}\bf #1}}
\newcommand{\blueHL}[1]{\textbf{\color{blue}#1}}
\newcommand{\greenHL}[1]{\textbf{\color{mydarkgreen}#1}}
\newcommand{\jsugg}[1]{\textit{\color{blue}#1}}
\newcommand{\jpvt}[1]{\textit{\color{red}#1}}
%\newcommand{\jsumm}[1]{{\color{blue}{{\uline{\textit{#1}}}}}}
\newcommand{\jsumm}[1]{\centerline{\color{blue}{{\uline{\textit{#1}}}}\\}}
\newcommand{\jkill}[1]{{\color{blue}\sout{#1}}}
\newcommand{\toputback}[1]{{\blueHL{PUT THIS BACK:} #1}}
\newcommand{\jemph}[1]{\textbf{\uline{#1}}}
\newcommand{\jques}[1]{{\color{blue}#1?}}
\let\jnoteignored=\ignore
	
%\newcommand{\jnote}[1]{\textit{\color{blue}#1}}
%\newcommand{\jnote}[1]{\centerline{\color{mydarkgreen}{{\uline{\textit{#1}}}}\\}}
%\newcommand{\jnote}[1]{{\color{mydarkgreen}\textit{\uline{#1}}}}
\newcommand{\jnote}[1]{{\color{mydarkgreen}\textit{{#1}}}}
\ignore{
    \newcommand{\jnote}[1]{% using fixme
    	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
    	\renewcommand{\fixmelogo}{}%
    	\hspace*{-0.35em}\raisebox{0.7em}[\height][\depth]
                {\\\makebox[0em][l]{\fxnote{\tiny{\color{myred}JR: }
                \textit{\color{mydarkgreen}#1}}}}%
    }
}
\let\jn=\jnote
\newcommand{\TOFIX}[1]{% using fixme
	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
	\renewcommand{\fixmelogo}{}%
	{\fxfatal{\bf\normalsize\textit{\color{myred}#1}}}%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END newcommands for ignoring, commenting, ....
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> bib/1-example-paper-template/newcommands-labels-refs.tex <==
% label and ref newcommands
% now mostly deprecated (but redefined and kept for backward compatibility) - move to \cref from the cleveref package
%\crefname{algocf}{alg.}{algs.}
\crefname{algocf}{Algorithm}{Algorithms}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefname{equation}{}{}
\Crefname{equation}{}{}

%DONE: xyzref{} should be able to handle multiple arguments so that you can
%reference multiple figures/equations at the same time -AG
%Now fixed with some package/command CREF.
\newcommand{\eqnlabel}[1]{\label{#1}}
\newcommand{\eqnref}[1]{\cref{#1}}
\newcommand{\algolabel}[1]{\label{#1}}
\newcommand{\algoref}[1]{\cref{#1}}
\newcommand{\corrlabel}[1]{\label{corr:#1}}
\newcommand{\corrref}[1]{Corollary \ref{corr:#1}}
\newcommand{\assref}[1]{Assumption \ref{ass:#1}}
\newcommand{\asslabel}[1]{\label{ass:#1}}
%\newcommand{\eqnref}[1]{(\ref{eq:#1})}
%\newcommand{\eqnlabel}[1]{\label{eq:#1}}
%\newcommand{\figlabel}[1]{\label{fig:#1}}
%\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\lstlabel}[1]{\label{lst:#1}}
\newcommand{\lstref}[1]{Listing~\ref{lst:#1}}
\newcommand{\figlabel}[1]{\label{#1}}
\newcommand{\figref}[1]{\cref{#1}}
\newcommand{\chaplabel}[1]{\label{chap:#1}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\tablabel}[1]{\label{#1}}
\newcommand{\tabref}[1]{\cref{#1}}
\newcommand{\thlabel}[1]{\label{th:#1}}
\newcommand{\thref}[1]{Theorem~\ref{th:#1}}
\newcommand{\thmlabel}[1]{\label{thm:#1}}
\newcommand{\thmref}[1]{Theorem \ref{thm:#1}}
\newcommand{\remlabel}[1]{\label{rem:#1}}
\newcommand{\remref}[1]{Remark \ref{rem:#1}}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\lemlabel}[1]{\label{lem:#1}}
\newcommand{\lemref}[1]{Lemma \ref{lem:#1}}
\newcommand{\examplelabel}[1]{\label{#1}}
\newcommand{\exampleref}[1]{Example \cref{#1}}
%\newcommand{\labexample}[1]{\label{example:#1}}
\newcommand{\httpref}[1]{}
\let\el=\eqnlabel
\let\er=\eqnref


==> bib/1-example-paper-template/newcommands-math.tex <==
%\newcommand{\ddt}[2]{{\frac{d}{d #2}\left. #1 \right.}}
\newcommand{\ddt}[2]{{\frac{d #1}{d #2}}}
\newcommand{\ddx}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand{\Ddx}[2]{{\frac{D}{d{#2}}\left[ #1 \right]}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\deq}{\triangleq}
\newcommand{\I}{I\left[\right]}
\newcommand{\ELL}[1]{L\left[#1\right]}
\newcommand{\w}{\omega}
\newcommand{\calD}{{\cal D}}
\renewcommand{\jmath}{j}
\newcommand{\Pinvt}{{P(t)}^{-1}}
\newcommand{\halmos}{\hskip\textwidth minus\textwidth \rule{6pt}{6pt}}
\newcommand{\calA}{{\cal A}}
\newcommand{\calAT}{{\cal A}^T}
\newcommand{\calL}{{\cal L}}
\newcommand{\calLadj}{\calL^\dagger}
\newcommand{\calR}{{\cal R}}
%\newcommand{\Reals}{\Bbb{R}}
%\newcommand{\Real}{\Bbb{R}}
\newcommand{\Reals}{\mathbf{R}}
\newcommand{\Real}{\mathbf{R}}
\newcommand{\Safe}{\ensuremath{{\bf S}}}
\newcommand{\Pade}{{Pad\'e}}
\newcommand{\Complexes}{\Bbb{C}}
\newcommand{\HvecqLanc}{\Hvec^{(L)}_q}
\newcommand{\HvecqArn}{\Hvec^{(A)}_q}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\calDT}{{\cal D}^T}
\newcommand{\calCtil}{\tilde{\cal C}}
\newcommand{\calJtil}{\tilde{\cal J}}
\newcommand{\calDtil}{\tilde{\cal D}}
\newcommand{\JstarDphi}{J_{\Delta \phi}^*}
\newcommand{\Jstarphi}{J_{\phi}^*}
\newcommand{\vecbphi}{\vec b_{\phi}}
\newcommand{\vecbext}{\vec b_{\text{ext}}}
\newcommand{\phistarIdeal}{\phi_{\text{ideal}}^*}
\newcommand{\apdx}[1]{\appref{#1}} 
\newcommand{\delbydel}[2]{\ensuremath{\frac{\partial {#1}}{\partial {#2}}}}
\newcommand{\delbydeln}[3]{\ensuremath{\frac{\partial^{{#1}}
{#2}}{\partial{#3}^{{#1}}}}}
\newcommand{\delbydelat}[3]{\ensuremath{\left. \frac{\partial
{#1}}{\partial {#2}} \right|_{{#3}}}}
\newcommand{\dee}{\ensuremath{\mathrm{d}}}
\newcommand{\dbyd}[2]{\ensuremath{\frac{\mathrm{d} {#1}}{\mathrm{d}
{#2}}}}
\newcommand{\dbydn}[3]{\ensuremath{\frac{\mathrm{d}^{{#1}}{#2}}
{\mathrm{d}{#3}^{{#1}}}}}
\newcommand {\dist}[1] {{{\rm dist}\left({#1}\right)}}
\def\Matrix#1{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\textdiag}{{\text{diag}}}
\newcommand{\ihat}{\hat{\imath}}
\newcommand{\jhat}{\hat{\jmath}}
\newcommand{\khat}{\hat{k}}
\newcommand{\del}{\nabla}
\newcommand{\Rxx}{R_{\vec x \vec x}}
\newcommand{\Sxx}{S_{\vec x \vec x}}
\newcommand{\Snn}{S_{\vec n \vec n}}
\newcommand{\vecphi}{\vec \phi}
\newcommand{\Dphi}{\Delta \phi}
\newcommand{\vecDphi}{\vv{\Delta \phi}}
\newcommand{\dphi}{\delta \phi}
\newcommand{\vecdphi}{\vv{\delta \phi}}
\newcommand{\ah}{\alpha_g} % g for group
%\newcommand{\tDagger}{{\tilde t}}
\newcommand{\tDagger}{{t^{\!\dagger}}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\texthyphen}{\text{--}}
\DeclareMathOperator*{\argmax}{arg\,max} % depends on amsmath. Use \argmax_x
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\sgn}{sgn}

%The substack command can be used to produce a multi-line subscripts or superscripts:
%\sum_{\substack{0\le i\le m\\ 0<j<n}} P(i,j) produces a two-line subscript underneath the sum.
%A slightly more general form is the subarray environment which allows you to specify that each line should be left-aligned instead of centered, as here:
% \sum_{\begin{subarray}{l} i\in\Lambda\\ 0<j<n \end{subarray}} P(i,j) 

%\newcommand{\be}[1]{\begin{equation}\eqnlabel{#1}} % now moved to cleveref
\newcommand{\be}[1]{\begin{equation}\label{#1}}
\def\ee{\end{equation}}


==> bib/1-example-paper-template/newcommands-misc.tex <==
% Misc. commands
%\newcommand{\website}{http://www.eecs.berkeley.edu/\char126 jr/NOW-FT-Monograph/}

%\newcommand{\figdir}{./figures} % best to define this in the main tex file

% \newcommand{\bibdir}{.} % ditto

\newif\ifjournalsub
\newcommand{\ifthen}[2]{\ifthenelse{#1}{#2}{}}
\newcommand{\iftr}[1]{\boolean{#1}}

\newcommand{\DAEtoFSM}{ABCD}
\newcommand{\Brangluin}{Brangluin}
\newcommand{\LTIMORrefs}{pillage1,FeFr95a,OdCePiTCAD98,PhDaSiDAC2002,PhSiPMTBRDATE2004}
\newcommand{\nonlinearMORrefs}{RoTVPTCAS99,ReWhTCAD2003,PhTCAD2003,DoRoTCADPWP2008,
                               GuRoICCAD2008maniMOR}
\newcommand{\MORrefs}{\LTIMORrefs,\nonlinearMORrefs}
\newcommand{\proposalAcronym}{THz-PHLOGON}
\newcommand{\website}{http://www.eecs.berkeley.edu/$\sim$jr/NOW-FT-Monograph/}
\newcommand{\PNJLIM}{\textsf{\small PNJLIM}}
%\newcommand{\MATLAB}{\textbf{MATLAB}$^{\texttrademark}$}
\newcommand{\MATLAB}{MATLAB$^\text{\textregistered}$}

%%%% misc formatting setup
\newlength{\colwidth}
\newcommand{\pswidthcoeff}{0.9}
\newcommand{\psheightcoeff}{0.6}
\newlength{\pgwid}



% make LaTeX less fussy about line breaks, so that it typsets inline 
% math without overflowing -- perhaps remove if it causes trouble.
\sloppy 
\setcounter{secnumdepth}{5}  % numbered \paragraph == \subsubsubsection

% remove indentation from subparagraph
\makeatletter
\renewcommand\subparagraph{%
 \@startsection {subparagraph}{5}{\z@ }{3.25ex \@plus 1ex
 \@minus .2ex}{-1em}{\normalfont \normalsize \bfseries }}%
\makeatother

%a proper longemdash, that doesn't make me feel like putting spaces around it:
\newcommand{\longemdash}{\rule[.5ex]{1.3em}{0.5pt}}

\pagenumbering{arabic}
%\renewcommand{\thepage} {Body--\arabic{page}}
\hyphenation{op-tical net-works semi-conduc-tor} % correct bad hyphenation here



==> bib/1-example-paper-template/newcommands-squeeze-spaces--no-titlesec.tex <==
\ignore{ TWEAKLIST OFTEN CAUSES ERRORS
%%% tweaklist renewcommands - 
\newcommand{\modifiedListParamters}{
  \setlength{\topsep}{0pt}%
  \setlength{\itemsep}{-0.1em}
  \setlength{\partopsep}{0em}
  \setlength{\parsep}{0em}
  \setlength{\leftmargin}{1.1em}
  \setlength{\itemindent}{0.0em}
}
\renewcommand{\enumhook}{
  \modifiedListParamters
  \setlength{\itemindent}{0.2em}
}
\renewcommand{\itemhook}{
  \modifiedListParamters
}
\renewcommand{\descripthook}{
  \modifiedListParamters
  \setlength{\itemindent}{-1.0em}
}
%%% end tweaklist renewcommands
}

% same functionality as tweaklist (but better?)
\let\labelindent\relax % to fix conflict with IEEEtran,otherwise not reqd?
\usepackage{enumitem}
\setenumerate{leftmargin=1em,itemindent=0em,labelindent=0em,itemsep=0em} % sets it globally.
% you can do it on a per list basis like this:
% \begin{enumerate}[leftmargin=1em,itemindent=0em,labelindent=0em,itemsep=0em]
%   \item ...
% \end{enumerate}


\ignore{not usually needed, but the definitions have useful info
		Space saving List environment for enumerations.

	\newcounter{myctr}
	\newenvironment{mylist}{\begin{list}{\arabic{myctr}.}
   		{\usecounter{myctr}
   		%\setlength{\topsep}{1mm}\setlength{\itemsep}{0.5mm}
   		\setlength{\topsep}{0.3mm}
   		\setlength{\itemsep}{0mm}
   		\setlength{\parsep}{0.3mm}
   		\setlength{\itemindent}{0mm}
   		\setlength{\partopsep}{0mm}
   		\setlength{\labelwidth}{15mm}
   		\setlength{\leftmargin}{4mm}
   		}
	}{\end{list}}

	\newenvironment{myitemize}{\begin{list}{$\bullet$}
	  \ignore{\setlength{\topsep}{0.8mm}\setlength{\itemsep}{0.25mm}}
	  {\setlength{\topsep}{1mm}\setlength{\itemsep}{0.25mm}
	  \setlength{\parsep}{0.1mm}
	  \setlength{\itemindent}{0mm}\setlength{\partopsep}{0mm}
	  \setlength{\labelwidth}{15mm}
	  \setlength{\leftmargin}{4mm}}
	}{\end{list}}
}

%%%%% titlesec: squeezing whitespace between section headings
%	\titlespacing{\section}{0pt}{*0}{*0.1} % {0pt} is indentation; {*0} is 
%                                           % space above; {*0.5} is space below
%	%\titlespacing{\subsection}{0pt}{*0.1}{*0.7}
%	\titlespacing{\subsection}{0pt}{*0.1}{*0.1}
%	\titlespacing{\subsubsection}{0pt}{*0.1}{*0}
%%%%% end titlesec

%%%% squeezing whitespace in and around figures
    \floatsep=0em % space left between floats.
    \textfloatsep=0em % space between last top float or first bottom float and the text.
    \intextsep=0em % space left on top and bottom of an in-text float.
    %\dbltextfloatsep is \textfloatsep for 2 column output.
    %\dblfloatsep is \floatsep for 2 column output.
    \abovecaptionskip=0em % space above caption
    \belowcaptionskip=0em % space below caption
%%%% END squeezing whitespace in and around figures

\makeatletter
\g@addto@macro\normalsize{%
  \setlength\abovedisplayskip{1pt}
  \setlength\belowdisplayskip{1pt}
  \setlength\abovedisplayshortskip{1pt}
  \setlength\belowdisplayshortskip{1pt}
}
\makeatother

%\newcommand{\mycaption}[1]{\caption{\small #1}}
\newcommand{\mycaption}[1]{\caption{\tiny #1}}

% for captions spacing
%\captionsetup[table]{font={scriptsize},format=hang,indention=0em}     %% change 1.2 as you like
\captionsetup[table]{font={small},indention=0.2em}     %% change 1.2 as you like
%\captionsetup[figure]{font={scriptsize},format=hang,indention=0em}    %% change as you like
\captionsetup[figure]{font={small},indention=0.2em}    %% change as you like
 %% or
 %% \captionsetup{font={stretch=1.2}}  %% this affects both figure and table

% replace Figure x in captions by Fig. x
%\renewcommand{\figurename}{Fig.} % doesn't work.
%but \usepackage[figurename=Fig.]{caption} in packages-headers.tex does work.


%\renewcommand{\baselinestretch}{1.5}
%\setstretch{1.5}

%\def\baselinestretch{0.8593}\large\normalsize - this form works locally?
%\renewcommand{\baselinestretch}{0.94} - this form works only in the preamble
%\renewcommand{\baselinestretch}{0.90}
%\renewcommand{\baselinestretch}{0.5}
%\linespread{0.5} % 0.5 -> 7 lines per inch; 0.9 -> a bit more than 6 lines 
%                 % per vertical inch
% \linespread{0.99}

% baselinestretch fixes for squeezing. See also linespread
%\def\ssp{\def\baselinestretch{0.95645}\large\normalsize} % "single space"
%\def\ssp{\def\baselinestretch{0.905}\large\normalsize} % "single space"
\def\ssp{\def\baselinestretch{0.9}\large\normalsize} % "single space"
\def\dsp{\def\baselinestretch{1.35}\large\normalsize} % "double space"
\ssp

% indent paragraphs less (saves space)
\parindent 	1em
% do not indent paragraphs (saves more space)
\parindent 	0em
% adjust space between paragraphs (0em can obscure paragraph breaks)
\parskip 0.3em

% vim: guifont=mono\ 11


==> bib/1-example-paper-template/newcommands-squeeze-spaces.tex <==
\input newcommands-squeeze-spaces--no-titlesec
%%%% titlesec: squeezing whitespace between section headings
	\titlespacing{\section}{0pt}{*0}{*0.1} % {0pt} is indentation; {*0} is 
                                           % space above; {*0.5} is space below
	%\titlespacing{\subsection}{0pt}{*0.1}{*0.7}
	\titlespacing{\subsection}{0pt}{*0.1}{*0.1}
	\titlespacing{\subsubsection}{0pt}{*0.1}{*0}
%%%% end titlesec

% vim: guifont=mono\ 11


==> bib/1-example-paper-template/newcommands-thm-env.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% theorem-like environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\EndProof{\hfill \quad \vrule width 1ex height 1ex depth 0pt  }
\newtheorem{corollary}{Corollary}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
%\newtheorem{illustration}{Illustration}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{defn}{Definition}[section]
\newtheorem{notation}{Notation}
\newtheorem{theorem}{Theorem}
\newenvironment{sketch}{\noindent{\bf Sketch of Proof}:}{\halmos}
\newenvironment{conjecture}{\noindent{\bf Conjecture}: \em}{}
\newcommand{\numberedtheorem}[3]{
	\ifthen{\not\equal{#1}{}}{
		\let\oof=\thetheorem
		\renewcommand{\thetheorem}{#1}
	}
	\begin{theorem}
	\ifthen{\not\equal{#2}{}}{
		\thmlabel{#2}
	}
	#3
	\end{theorem}
	\ifthen{\not\equal{#1}{}}{
		\let\thetheorem=\oof
		\addtocounter{theorem}{-1}
	}
}
\newcommand{\numberedlemma}[3]{
	\ifthen{\not\equal{#1}{}}{
		\let\oof=\thelemma
		\renewcommand{\thelemma}{#1}
	}
	\begin{lemma}
	\ifthen{\not\equal{#2}{}}{
		\lemlabel{#2}
	}
	#3
	\end{lemma}
	\ifthen{\not\equal{#1}{}}{
		\let\thelemma=\oof
		\addtocounter{lemma}{-1}
	}
}


==> bib/1-example-paper-template/package-and-newcommand-includes-cambridge.tex <==
  \usepackage{subfigure}
  \usepackage{fancyvrb} % to work around problems with listings, below
  \usepackage{savesym} % to work around problems with listings, below
  \savesymbol{abovecaptionskip}
  \savesymbol{belowcaptionskip}
  \usepackage{listings} % - conflicts with EngC - \abovecaptionskip already defined
  \usepackage{lstautogobble} % gobbles initial spaces
  \restoresymbol{EngC}{abovecaptionskip} % now EngC's abovecaptionskip is \EngCabovecaptionskip
  \restoresymbol{EngC}{belowcaptionskip} % 
  \usepackage[dvipsnames]{xcolor} % for color commands

    \lstset{ %
      %backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
      %basicstyle=\tt\small,        % the size of the fonts that are used for the code
      basicstyle=\tt\scriptsize,        % the size of the fonts that are used for the code
      breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
      breaklines=false,                 % sets automatic line breaking
      captionpos=b,                    % sets the caption-position to bottom
      commentstyle=\color{OliveGreen},    % comment style
      deletekeywords={...},            % if you want to delete keywords from the given language
      escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
      extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
      keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
      keywordstyle=\color{blue},       % keyword style
      language=python,                 % the language of the code
      morekeywords={*,...},            % if you want to add more keywords to the set
      numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
      numbersep=5pt,                   % how far the line-numbers are from the code
      numberstyle=\tiny\color{black}, % the style that is used for the line-numbers
      rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
      showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
      showstringspaces=true,          % underline spaces within strings only
      showtabs=true,                  % show tabs within strings adding particular underscores
      stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
      stringstyle=\color{black},     % string literal style
      tabsize=1,                       % sets default tabsize to 2 spaces
      frame = none,
      frame=single,                    % adds a frame around the code
      fancyvrb = true,
      columns = fullflexible,
      autogobble = true                % gobble up leading spaces
    }


  \usepackage{sverb} % defines the listing environment
% \documentclass[multi]{EngC} % multi-contributor option
% \documentclass[prodtf]{EngC}% if you have helvetica neue condensed fonts

  \usepackage[rightcaption,raggedright]{sidecap}% for side captions
  \usepackage{framed}         % for floatingboxes
  \usepackage{soul}           % for letterspacing in theorem-style headings

% for the Harvard author-date referencing system
  %\usepackage[agsm]{harvard}

% if you are using either vancouver.bst or IEEEtran.bst and wish to remove
% square braces in the reference list, uncomment the line below
% \removesquarebraces

  \usepackage{rotating}
  \usepackage{floatpag}
  \rotfloatpagestyle{empty}

  \usepackage{amsmath}% if you are using this package,
                     % it must be loaded before amsthm.sty

  %\usepackage{amstext} % provides \text, but this is included by amsmath
  \usepackage{amsthm}
  \usepackage{amssymb} % provides mathbb, replacement for \Bbb
% \usepackage{txfonts}% times font (used to produce EngCguide.pdf)
                      % this package must be loaded after amsthm.sty
  \usepackage{amsxtra} % \sphat, \sptilde (A\sphat)
  \usepackage{graphicx}
  \usepackage{epsfig}
  %\usepackage[subfigure]{tocloft} % to solve problem with BYUTextbook
  %\usepackage{mathptmx} % conflict with tocloft % old/deprecated; see https://tex.stackexchange.com/questions/347244/how-can-i-adjust-the-fontsize-of-greek-letters-only
  \usepackage{newtxtext} % https://tex.stackexchange.com/questions/347244/how-can-i-adjust-the-fontsize-of-greek-letters-only
  \usepackage{newtxmath} % https://tex.stackexchange.com/questions/347244/how-can-i-adjust-the-fontsize-of-greek-letters-only
  \usepackage[compress,capitalise,noabbrev]{cleveref} % conflict with tocloft
  \usepackage{algorithm2e}
  %\usepackage[noend, boxruled, linesnumbered] {algorithm2e}


  %\usepackage[final]{showlabels}


% indexes
% uncomment the relevant set of commands

% for a single index
% \usepackage{makeidx}
% \makeindex

% for multiple indexes using multind.sty
  % \usepackage{multind}\ProvidesPackage{multind} % EngC only
  % \makeindex{authors}
  % \makeindex{subject}

%% showlabels should be the LAST package loaded
%\RequirePackage{showkeys}
\RequirePackage[outer,draft]{showlabels}
%\RequirePackage[inline]{showlabels}
%\showlabel{cite}
%\showlabel{label}
\renewcommand{\showlabelfont}{\tiny\ttfamily\color{blue}}
%\renewcommand{\showlabelsetlabel}[1]{\tiny #1}

%%%%%%%%%%%%%%%%%% END PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%

% for code listings

% for multiple indexes using index.sty
% \usepackage{index}
% \newindex{aut}{adx}{and}{Author index}
% \makeindex

  \newcommand\cambridge{EngC}

% see chapter 3 for details
  %\theoremstyle{plain}% default
  %\newtheorem{theorem}{Theorem}[chapter]
  %\newtheorem{lemma}[theorem]{Lemma}
  %\newtheorem*{corollary}{Corollary}

  %\theoremstyle{definition}
  %\newtheorem{definition}[theorem]{Definition}
  %\newtheorem{condition}[theorem]{Condition}

  %\theoremstyle{remark}
  %\newtheorem{remark}{Remark}[chapter]
  %\newtheorem{notation}[remark]{Notation}
  %\newtheorem*{case}{Case}

  \hyphenation{line-break line-breaks docu-ment triangle cambridge amsthdoc
    cambridgemods baseline-skip author authors cambridgestyle en-vir-on-ment polar}

  \setcounter{tocdepth}{2}% the toc normally lists sections;
% for the purposes of this document, this has been extended to subsections

\input colour-defs
\let\ignore\relax % undefines \ignore, which EngC seems to define to something
\input newcommands-highlight-ignore-comments-annotations
\input newcommands-eg-ie-etc
\input newcommands-labels-refs
\input newcommands-math
%\input newcommands-thm-env
\input newcommands-for-bibtex
%\input newcommands-squeeze-spaces
%\input leeseshia-examples-environment
\input newcommands-misc

% figdir



==> bib/1-example-paper-template/package-and-newcommand-includes-llncs.tex <==
%%%%%%%%%%%%%%%%%% PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%
\RequirePackage{times}
\RequirePackage{mathptm} % - AG (Don't like \mathcal{C} that this produces
\RequirePackage{mathptmx} % times (smaller) math fonts, greek characters also italicized
%\RequirePackage[usenames]{pstcol} 
\RequirePackage[usenames]{pstricks} 

% Graphics (figures/images etc.)
%\usepackage[pdftex]{graphicx}
\RequirePackage{graphicx} % supplies \includegraphics
\graphicspath{{./octave-figures/}{./results/}{./figures/}{./snapshots/}}
\DeclareGraphicsExtensions{.eps,.pdf,.jpeg,.png,.jpg}

\RequirePackage{rotating}
\RequirePackage{indentfirst} 
\RequirePackage{color} 
%\RequirePackage{picins} 
\RequirePackage{bmpsize} 
\RequirePackage{epsfig} % good old way of including figures
\RequirePackage{eepic} 
\RequirePackage{subfigure} % put figures side-by-side
\RequirePackage{wrapfig} % wrap text around figures
\RequirePackage{picinpar} % alternative to wrapfig, less useful

% Math (symbols/equations etc.)
\usepackage{cancel}
\RequirePackage{amsmath,amssymb,amsbsy,amsfonts,dotlessj} 
\RequirePackage{latexsym}
\RequirePackage{bm} % boldmath
\DeclareMathVersion{bold} 

% Formatting
\RequirePackage{multicol}
\RequirePackage{esvect} % defines \vv{}
\RequirePackage{ifthen}
\RequirePackage{etoolbox}
\RequirePackage{relsize}
\RequirePackage{soul}   % Provides \hl{some-text}
%\RequirePackage{showkeys} 
%\RequirePackage[final,notref]{showkeys} 
%\RequirePackage[top=0.8cm,bottom=0.8cm,left=0.8cm,right=0.8cm,nohead,nofoot]{geometry}
%\RequirePackage[top=1.2cm,bottom=1.3cm,left=1.2cm,right=1.2cm,nohead,nofoot]{geometry}

\usepackage[nolist,nohyperlinks]{acronym}
\RequirePackage{setspace}
\RequirePackage{moreverb}
\RequirePackage{ulem} % provides \uline
        \let\em=\it % ulem package redefines \em=\uline
\RequirePackage[sectionbib]{chapterbib}
\RequirePackage{fancyhdr}
\RequirePackage{array}
\RequirePackage{floatflt} % does (to some extent) work inside itemize environment %
                          % use \fltditem, see $LATEXDOCS/floatflt.pdf, esp. Sec 3.1
\RequirePackage{srcltx}
\RequirePackage{chemarrow}

% Utilities
\RequirePackage{todonotes}
\RequirePackage{tcolorbox}
\RequirePackage{fixme}
\RequirePackage[footnotesize,bf,figurename=Fig.,hang]{caption}
%\usepackage[scriptsize,hang,bf]{caption}
%\RequirePackage[hypertex]{hyperref} 
\RequirePackage[bookmarks,hidelinks=true]{hyperref} 
\RequirePackage[depth=subsection]{bookmark}
%\definecolor{linkColor}{rgb}{0.1,0.1,0.8}
%\usepackage[colorlinks=true,bookmarks,pdfpagemode=UseOutlines,linkcolor=linkColor,citecolor=linkColor,pagecolor=blue,urlcolor=blue,pdftitle={Verification, Learning, Control},pdfauthor={Jaijeet Roychowdhury},plainpages=false]{hyperref}

%\usepackage{./tweaklist} % allow changing of item spacings in standard itemize,
                         % enumerate, description environments
					     %%% tweaklist: compress lists. Also check out 
                         %%% \usepackage{mdwlist} (use itemize*, enumerate*, 
                         %%% description* with that)
                         % enumhook for the enumerate environment, itemhook for
                         % the itemize environment, and descripthook for the
                         % description environment.
                         % HOWEVER, CAUSES ERRORS. Use enumitem instead.

% enumitem package included from newcommands-squeeze-spaces.tex

\providecommand{\subparagraph}{} % needed for IEEEtran.cls (which does not define subparagraph); \providecommand checks if it is already defined
\RequirePackage[small,compact]{titlesec} % squeezing whitespace between section heading
\RequirePackage[sectionbib,square,sort&compress,numbers]{natbib} % needed for IEEEtran; but proposal.cls pulls it in automatically
%\RequirePackage{cite} % natbib doesn't like this
\RequirePackage{lipsum}
\RequirePackage{microtype}
\RequirePackage{url}
\RequirePackage{listings} % Required for insertion of code
\RequirePackage{multirow}
\RequirePackage{booktabs}
% load cleveref last, but before algorithm2e (which breaks cleveref)
\RequirePackage[compress,capitalise,noabbrev]{cleveref} % defines \cref, \Cref, etc; options are compress (don't sort), sort (don't compress), sort&compress (default), nosort (neither sort nor compress)
%\RequirePackage{algorithmic}
%\RequirePackage{algorithm}
%\RequirePackage[boxed,algoruled]{algorithm2e}
\RequirePackage[boxed,algoruled,linesnumbered,vlined,nofillcomment]{algorithm2e}
%\usepackage[yyyymmdd,hhmmss]{datetime} % use: Compiled on \today\ at \currenttime
\usepackage{datetime2} % ]use: Compiled on \DTMnow. And do \documentstyle[pacific]{...}

%%%%%%%%%%%%%%%%%% END PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%

% fixme package setup
\fxsetup{ status=draft,
		  %author={\tiny JR},
	  	  layout=footnote,
		  layout=inline, % also try footnote or pdfnote
		  theme=color,
	  	  marginclue
}
\definecolor{mydarkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{myred}{rgb}{0.9,0.0,0.0}
%\definecolor{fxnote}{rgb}{0.8000,0.0000,0.0000}
\renewcommand{\englishlistfixmename}{List of changes needed}
% Decrease spacing between items in bib
\newcommand{\BIBdecl}{\setlength{\itemsep}{0.25 em}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Multi-column the bib
%\patchcmd{\thebibliography}
%  {\list}
%  {\begin{multicols}{2}\list}
%    {}
%    {}
%\appto{\endthebibliography}{\end{multicols}}

%------------------------------------------------------------------------------
%   CODE INCLUSION CONFIGURATION
%------------------------------------------------------------------------------

\lstloadlanguages{Matlab}
\lstset{language=Matlab,
        frame=single, % Single frame around code
        basicstyle=\scriptsize\ttfamily,
        % keywordstyle=[1]\color{blue}\bf, % Perl functions bold and blue
        keywordstyle=[3]\color{blue}\underbar, % Custom functions underlined and blue
        identifierstyle=, % Nothing special about identifiers                                         
        commentstyle=\usefont{T1}{pcr}{m}{sl}\color{green}\scriptsize, 
            % Comments are in small dark green courier font
        stringstyle=\color{red}, 
        showstringspaces=false, % Don't put marks in string spaces
        tabsize=4, % 5 spaces per tab
        % 
        % Put standard functions not included in the default language here
        %morekeywords={rand},
        % Put function parameters here
        %morekeywords=[2]{on, off, interp},
        % Put user defined functions here
        %morekeywords=[3]{test},
        %
        morecomment=[l][\color{blue}]{...}, % Line continuation (...) like blue comment
        % numbers=left, % Line numbers on left
        % firstnumber=1, % Line numbers start with line 1
        % numberstyle=\tiny\color{blue}, % Line numbers are blue and small
        % stepnumber=5 % Line numbers go in steps of 5
}

% Creates a new command to include an Matlab script, the first parameter is the
% filename of the script (without .pl), the second parameter is the caption
\newcommand{\matlabscript}[2]{
    \begin{itemize}
    \item[]\lstinputlisting[caption=#2,label=#1]{#1}
    \end{itemize}
}

\input{colour-defs}
\input{newcommands-highlight-ignore-comments-annotations}
\input{newcommands-labels-refs}
\input{newcommands-eg-ie-etc}
\input{newcommands-for-bibtex} % BP, BPnom, IP, presenter, putDOI, DP, etc
\input{newcommands-misc}
\input{newcommands-squeeze-spaces}
\input{newcommands-math}
% \input newcommands-thm-env




==> bib/1-example-paper-template/package-and-newcommand-includes-plain-llncs-noTimes.tex <==
%%%%%%%%%%%%%%%%%% PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%

% Graphics (figures/images etc.)
%\usepackage[pdftex]{graphicx}
\RequirePackage{graphicx} % supplies \includegraphics
\graphicspath{{./octave-figures/}{./results/}{./figures/}{./snapshots/}}
\DeclareGraphicsExtensions{.eps,.pdf,.jpeg,.png,.jpg}

\RequirePackage{color} 
\RequirePackage{epsfig} % good old way of including figures
\RequirePackage{subfigure} % put figures side-by-side
\RequirePackage{wrapfig} % wrap text around figures

% Math (symbols/equations etc.)
\usepackage{cancel}
\RequirePackage{amsmath,amssymb,amsbsy,amsfonts,dotlessj} 
\RequirePackage{latexsym}
\RequirePackage{bm} % boldmath
\DeclareMathVersion{bold} 

% Formatting
%\RequirePackage{showkeys} 
%\RequirePackage[final,notref]{showkeys} 
%\RequirePackage[top=0.8cm,bottom=0.8cm,left=0.8cm,right=0.8cm,nohead,nofoot]{geometry}
%\RequirePackage[top=1.2cm,bottom=1.3cm,left=1.2cm,right=1.2cm,nohead,nofoot]{geometry}

\usepackage[nolist,nohyperlinks]{acronym}
%\RequirePackage{setspace}
\RequirePackage{ulem} % provides \uline
        \let\em=\it % ulem package redefines \em=\uline
%\RequirePackage[sectionbib]{chapterbib}
%\RequirePackage{fancyhdr}
%\RequirePackage{array}
%\RequirePackage{floatflt} % does (to some extent) work inside itemize environment %
                          % use \fltditem, see $LATEXDOCS/floatflt.pdf, esp. Sec 3.1
%\RequirePackage{srcltx}
%\RequirePackage{chemarrow}

% Utilities
%\RequirePackage{todonotes}
%\RequirePackage{tcolorbox}
\RequirePackage{fixme}
\RequirePackage[footnotesize,bf,figurename=Fig.,hang]{caption}
%\usepackage[scriptsize,hang,bf]{caption}
%%\RequirePackage[hypertex]{hyperref} 
\RequirePackage[bookmarks,hidelinks=true]{hyperref} 
%\RequirePackage[depth=subsection]{bookmark}
%\definecolor{linkColor}{rgb}{0.1,0.1,0.8}
%\usepackage[colorlinks=true,bookmarks,pdfpagemode=UseOutlines,linkcolor=linkColor,citecolor=linkColor,pagecolor=blue,urlcolor=blue,pdftitle={Verification, Learning, Control},pdfauthor={Jaijeet Roychowdhury},plainpages=false]{hyperref}

%\usepackage{./tweaklist} % allow changing of item spacings in standard itemize,
                         % enumerate, description environments
					     %%% tweaklist: compress lists. Also check out 
                         %%% \usepackage{mdwlist} (use itemize*, enumerate*, 
                         %%% description* with that)
                         % enumhook for the enumerate environment, itemhook for
                         % the itemize environment, and descripthook for the
                         % description environment.
                         % HOWEVER, CAUSES ERRORS. Use enumitem instead.

% enumitem package included from newcommands-squeeze-spaces.tex

%\providecommand{\subparagraph}{} % needed for IEEEtran.cls (which does not define subparagraph); \providecommand checks if it is already defined
%\RequirePackage[small,compact]{titlesec} % squeezing whitespace between section heading
%\RequirePackage[sectionbib,square,sort&compress,numbers]{natbib} % needed for IEEEtran; but proposal.cls pulls it in automatically
%\RequirePackage{cite} % natbib doesn't like this
%\RequirePackage{lipsum}
%\RequirePackage{microtype}
\RequirePackage{url}
%\RequirePackage{listings} % Required for insertion of code
%\RequirePackage{multirow}
%\RequirePackage{booktabs}
% load cleveref last, but before algorithm2e (which breaks cleveref)
\RequirePackage[compress,capitalise,noabbrev]{cleveref} % defines \cref, \Cref, etc; options are compress (don't sort), sort (don't compress), sort&compress (default), nosort (neither sort nor compress)
%\RequirePackage{algorithmic}
%\RequirePackage{algorithm}
%\RequirePackage[boxed,algoruled]{algorithm2e}
%\RequirePackage[boxed,algoruled,linesnumbered,vlined,nofillcomment]{algorithm2e}
%\usepackage[yyyymmdd,hhmmss]{datetime} % use: Compiled on \today\ at \currenttime
%\usepackage{datetime2} % ]use: Compiled on \DTMnow. And do \documentstyle[pacific]{...}

%%%%%%%%%%%%%%%%%% END PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%

% fixme package setup
\fxsetup{ status=draft,
		  %author={\tiny JR},
	  	  layout=footnote,
		  layout=inline, % also try footnote or pdfnote
		  theme=color,
	  	  marginclue
}
\definecolor{mydarkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{myred}{rgb}{0.9,0.0,0.0}
%\definecolor{fxnote}{rgb}{0.8000,0.0000,0.0000}
\renewcommand{\englishlistfixmename}{List of changes needed}
%% Decrease spacing between items in bib
%\newcommand{\BIBdecl}{\setlength{\itemsep}{0.25 em}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Multi-column the bib
%\patchcmd{\thebibliography}
%  {\list}
%  {\begin{multicols}{2}\list}
%    {}
%    {}
%\appto{\endthebibliography}{\end{multicols}}

%------------------------------------------------------------------------------
%   CODE INCLUSION CONFIGURATION
%------------------------------------------------------------------------------

% \lstloadlanguages{Matlab}
% \lstset{language=Matlab,
%         frame=single, % Single frame around code
%         basicstyle=\scriptsize\ttfamily,
%         % keywordstyle=[1]\color{blue}\bf, % Perl functions bold and blue
%         keywordstyle=[3]\color{blue}\underbar, % Custom functions underlined and blue
%         identifierstyle=, % Nothing special about identifiers                                         
%         commentstyle=\usefont{T1}{pcr}{m}{sl}\color{green}\scriptsize, 
%             % Comments are in small dark green courier font
%         stringstyle=\color{red}, 
%         showstringspaces=false, % Don't put marks in string spaces
%         tabsize=4, % 5 spaces per tab
%         % 
%         % Put standard functions not included in the default language here
%         %morekeywords={rand},
%         % Put function parameters here
%         %morekeywords=[2]{on, off, interp},
%         % Put user defined functions here
%         %morekeywords=[3]{test},
%         %
%         morecomment=[l][\color{blue}]{...}, % Line continuation (...) like blue comment
%         % numbers=left, % Line numbers on left
%         % firstnumber=1, % Line numbers start with line 1
%         % numberstyle=\tiny\color{blue}, % Line numbers are blue and small
%         % stepnumber=5 % Line numbers go in steps of 5
% }

% Creates a new command to include an Matlab script, the first parameter is the
% filename of the script (without .pl), the second parameter is the caption
%\newcommand{\matlabscript}[2]{
%    \begin{itemize}
%    \item[]\lstinputlisting[caption=#2,label=#1]{#1}
%    \end{itemize}
%}

\input{colour-defs}
\input{newcommands-highlight-ignore-comments-annotations}
\input{newcommands-labels-refs}
\input{newcommands-eg-ie-etc}
\input{newcommands-for-bibtex} % BP, BPnom, IP, presenter, putDOI, DP, etc
\input{newcommands-misc}
\input{newcommands-squeeze-spaces--no-titlesec}
%\input{newcommands-squeeze-spaces}
\input{newcommands-math}
% \input newcommands-thm-env




==> bib/1-example-paper-template/package-and-newcommand-includes.tex <==
%%%%%%%%%%%%%%%%%% PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%
\RequirePackage{times}
\RequirePackage[usenames]{pstcol} 
%\RequirePackage[usenames]{pstricks} 

% Graphics (figures/images etc.)
%\usepackage[pdftex]{graphicx}
\RequirePackage{graphicx} % supplies \includegraphics
\graphicspath{{./octave-figures/}{./results/}{./figures/}{./snapshots/}}
\DeclareGraphicsExtensions{.eps,.pdf,.jpeg,.png,.jpg}

\RequirePackage{rotating}
\RequirePackage{indentfirst} 
\RequirePackage{color} 
%\RequirePackage{picins} 
\RequirePackage{bmpsize} 
\RequirePackage{epsfig} % good old way of including figures
\RequirePackage{eepic} 
\RequirePackage{subfigure} % put figures side-by-side
%\RequirePackage{subfig} % apparently supercedes subfigure, but too many problems/differences with subfigure
%\RequirePackage{subcaption} % too many problems/differences with subfigure
\RequirePackage{wrapfig} % wrap text around figures
\RequirePackage{picinpar} % alternative to wrapfig, less useful

% Math (symbols/equations etc.)
\usepackage{cancel}
\RequirePackage{amsmath,amssymb,amsthm,amsbsy,amsfonts,dotlessj} 
\RequirePackage{latexsym}
\RequirePackage{mathptm} % - AG (Don't like \mathcal{C} that this produces
\RequirePackage{mathptmx} % times (smaller) math fonts, greek characters also italicized
\RequirePackage{bm} % boldmath
\DeclareMathVersion{bold} 


% Formatting
\RequirePackage{multicol}
\RequirePackage{esvect} % defines \vv{}
\RequirePackage{ifthen}
\RequirePackage{etoolbox}
\RequirePackage{relsize}
\RequirePackage{soul}   % Provides \hl{some-text}
%\RequirePackage{showlabels} 
\RequirePackage[final]{showkeys} 
%\RequirePackage[final,notref]{showkeys} 
\makeatletter
\newcommand{\vtiny}{\@setfontsize\vtiny{4}{5}}
\makeatother
\renewcommand*\showkeyslabelformat[1]{%
  \hbox{\parbox[t]{\marginparwidth}{\raggedright\normalfont\vtiny\ttfamily#1}}}
\newcommand{\fullrlap}[1]{%
  \rlap{\kern\dimexpr-\@totalleftmargin+\textwidth+\marginparsep\relax#1}}
\makeatletter
\patchcmd{\SK@@label}{\llap}{\fullrlap}{}{}% Insert appropriate (full)rlap patch
\patchcmd{\SK@@ref}{\footnotesize}{\vtiny}{}{}% reduce font size
\makeatother
%\RequirePackage[top=0.8cm,bottom=0.8cm,left=0.8cm,right=0.8cm,nohead,nofoot]{geometry}
%\RequirePackage[top=1.2cm,bottom=1.3cm,left=1.2cm,right=1.2cm,nohead,nofoot]{geometry}


\usepackage{tikz}
\usetikzlibrary{calc}
\usepackage[american,siunitx]{circuitikz}
\usepackage{pgfplots}

\usepackage[nolist,nohyperlinks]{acronym}
\RequirePackage{setspace}
\RequirePackage{moreverb}
\RequirePackage{ulem} % provides \uline
        \let\em=\it % ulem package redefines \em=\uline
\RequirePackage[sectionbib]{chapterbib}
\RequirePackage{fancyhdr}
\RequirePackage{array}
\RequirePackage{floatflt} % does (to some extent) work inside itemize environment %
                          % use \fltditem, see $LATEXDOCS/floatflt.pdf, esp. Sec 3.1
\RequirePackage{srcltx}
\RequirePackage{chemarrow}

% Utilities
\RequirePackage{todonotes}
\RequirePackage{tcolorbox}
\RequirePackage{fixme}
%\RequirePackage[footnotesize,bf,figurename=Fig.,hang]{caption}
\RequirePackage[footnotesize,bf,figurename=Fig.]{caption} % hang not great for small figures
%\usepackage[scriptsize,hang,bf]{caption}
%\RequirePackage[hypertex]{hyperref} 
\RequirePackage[implicit=false]{hyperref}  % implicit=false => href only (not figs/footnotes/citations/etc.)
%\RequirePackage[hidelinks]{hyperref} 
%\definecolor{linkColor}{rgb}{0.1,0.1,0.8}
%\usepackage[colorlinks=true,bookmarks,pdfpagemode=UseOutlines,linkcolor=linkColor,citecolor=linkColor,pagecolor=blue,urlcolor=blue,pdftitle={Verification, Learning, Control},pdfauthor={Jaijeet Roychowdhury},plainpages=false]{hyperref}
\hypersetup{ % get rid of annoying boxes, more muted links
    colorlinks,
    linkcolor={red!50!black},
    citecolor={blue!50!black},
    urlcolor={blue!80!black}
}


%\usepackage{./tweaklist} % allow changing of item spacings in standard itemize,
                         % enumerate, description environments
					     %%% tweaklist: compress lists. Also check out 
                         %%% \usepackage{mdwlist} (use itemize*, enumerate*, 
                         %%% description* with that)
                         % enumhook for the enumerate environment, itemhook for
                         % the itemize environment, and descripthook for the
                         % description environment.
                         % HOWEVER, CAUSES ERRORS. Use enumitem instead.

% enumitem package included from newcommands-squeeze-spaces.tex

\providecommand{\subparagraph}{} % needed for IEEEtran.cls (which does not define subparagraph); \providecommand checks if it is already defined
\RequirePackage[small,compact]{titlesec} % squeezing whitespace between section heading
\RequirePackage[square,sort&compress,numbers]{natbib} % needed for IEEEtran; but proposal.cls pulls it in automatically
%\RequirePackage{cite} % natbib doesn't like this
\RequirePackage{lipsum}
\RequirePackage{microtype}
\RequirePackage{url}
\RequirePackage{listings} % Required for insertion of code
\RequirePackage{multirow}
\RequirePackage{booktabs}
% load cleveref last, but before algorithm2e (which breaks cleveref)
\RequirePackage[compress,capitalise,noabbrev]{cleveref} % defines \cref, \Cref, etc; options are compress (don't sort), sort (don't compress), sort&compress (default), nosort (neither sort nor compress)
%\RequirePackage{algorithmic}
%\RequirePackage{algorithm}
%\RequirePackage[boxed,algoruled]{algorithm2e}
\RequirePackage[boxed,algoruled,linesnumbered,vlined,nofillcomment]{algorithm2e}
%\usepackage[yyyymmdd,hhmmss]{datetime} % use: Compiled on \today\ at \currenttime
\usepackage{datetime2} % ]use: Compiled on \DTMnow. And do \documentstyle[pacific]{...}

%%%%%%%%%%%%%%%%%% END PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%

% fixme package setup
\fxsetup{ status=draft,
		  %author={\tiny JR},
	  	  layout=footnote,
		  layout=inline, % also try footnote or pdfnote
		  theme=color,
	  	  marginclue
}
\definecolor{mydarkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{myred}{rgb}{0.9,0.0,0.0}
%\definecolor{fxnote}{rgb}{0.8000,0.0000,0.0000}
\renewcommand{\englishlistfixmename}{List of changes needed}
% Decrease spacing between items in bib
\newcommand{\BIBdecl}{\setlength{\itemsep}{0.25 em}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Multi-column the bib
%\patchcmd{\thebibliography}
%  {\list}
%  {\begin{multicols}{2}\list}
%    {}
%    {}
%\appto{\endthebibliography}{\end{multicols}}

%------------------------------------------------------------------------------
%   CODE INCLUSION CONFIGURATION
%------------------------------------------------------------------------------

\lstloadlanguages{Matlab}
\lstset{language=Matlab,
        frame=single, % Single frame around code
        basicstyle=\scriptsize\ttfamily,
        % keywordstyle=[1]\color{blue}\bf, % Perl functions bold and blue
        keywordstyle=[3]\color{blue}\underbar, % Custom functions underlined and blue
        identifierstyle=, % Nothing special about identifiers                                         
        commentstyle=\usefont{T1}{pcr}{m}{sl}\color{green}\scriptsize, 
            % Comments are in small dark green courier font
        stringstyle=\color{red}, 
        showstringspaces=false, % Don't put marks in string spaces
        tabsize=4, % 5 spaces per tab
        % 
        % Put standard functions not included in the default language here
        %morekeywords={rand},
        % Put function parameters here
        %morekeywords=[2]{on, off, interp},
        % Put user defined functions here
        %morekeywords=[3]{test},
        %
        morecomment=[l][\color{blue}]{...}, % Line continuation (...) like blue comment
        % numbers=left, % Line numbers on left
        % firstnumber=1, % Line numbers start with line 1
        % numberstyle=\tiny\color{blue}, % Line numbers are blue and small
        % stepnumber=5 % Line numbers go in steps of 5
}

% Creates a new command to include an Matlab script, the first parameter is the
% filename of the script (without .pl), the second parameter is the caption
\newcommand{\matlabscript}[2]{
    \begin{itemize}
    \item[]\lstinputlisting[caption=#2,label=#1]{#1}
    \end{itemize}
}

\input colour-defs
\input newcommands-highlight-ignore-comments-annotations
\input newcommands-labels-refs
\input newcommands-eg-ie-etc
\input newcommands-for-bibtex % BP, BPnom, IP, presenter, putDOI, DP, etc
\input newcommands-misc
\input newcommands-squeeze-spaces
\input newcommands-math
\input newcommands-thm-env


% vim: guifont=mono\ 11


==> bib/1-example-paper-templates/Makefile <==
include Makefile.common # first target all is checkfiles
#
# YOU SHOULD NOT NEED TO CHANGE ANYTHING BELOW: CHANGE ONLY Makefile.common

helpmsg: 
	- @echo "try make [pdf|pdfs|clean|pristine|mrproper]"
	- @echo ""

%.pdf: %.tex $(OTHERSRCS) $(REQDSOFTLINKS)
	@i=1; export TEXINPUTS=$(TEXINPUTS); while [[ $$i -le 4 ]] ; do \
		echo $$i; \
		((i=i+1)); \
		echo TEXINPUTS=.:$(TEXINPUTS) pdflatex $<; \
		TEXINPUTS=.:$(TEXINPUTS) pdflatex $<; \
		BUFILES=bu*.aux; \
		for bufile in $$BUFILES; do \
			echo TEXINPUTS=.:$(TEXINPUTS) bibtex $$bufile; \
			TEXINPUTS=.:$(TEXINPUTS) bibtex $$bufile; \
		done; \
		echo TEXINPUTS=.:$(TEXINPUTS) bibtex $(<:.tex=); \
		TEXINPUTS=.:$(TEXINPUTS) bibtex $(<:.tex=); \
		echo TEXINPUTS=.:$(TEXINPUTS) pdflatex $<; \
		TEXINPUTS=.:$(TEXINPUTS) pdflatex $<; \
	done

pdf pdfs: $(PDFS)
	- @ echo ""
	- @ echo "$^ ready."
	- @ echo "Check that latex shows NO undefined reference or other warnings above."
	- @ echo "Now run xpdf/zathura $^ manually and check that it looks right."
	- @ echo ""

.PHONY: pdfs helpmsg


==> bib/1-example-paper-templates/Makefile.latex <==
include Makefile.common # first target all is checkfiles helpmsg

# YOU SHOULD NOT NEED TO CHANGE ANYTHING BELOW: CHANGE ONLY Makefile.common

DVIS = $(TOP:.tex=.dvi)
%.dvi: %.tex $(OTHERSRCS) $(REQDSOFTLINKS)
	@i=1; export TEXINPUTS=$(TEXINPUTS); while [[ $$i -le 4 ]] ; do \
		echo $$i; \
		((i=i+1)); \
		echo TEXINPUTS=.:$(TEXINPUTS) latex $<; \
		TEXINPUTS=.:$(TEXINPUTS) latex $<; \
		BUFILES=bu*.aux; \
		for bufile in $$BUFILES; do \
			echo TEXINPUTS=.:$(TEXINPUTS) bibtex $$bufile; \
			TEXINPUTS=.:$(TEXINPUTS) bibtex $$bufile; \
		done; \
		echo TEXINPUTS=.:$(TEXINPUTS) bibtex $(<:.tex=); \
		TEXINPUTS=.:$(TEXINPUTS) bibtex $(<:.tex=); \
		echo TEXINPUTS=.:$(TEXINPUTS) latex $<; \
		TEXINPUTS=.:$(TEXINPUTS) latex $<; \
	done

include Makefile.dvi-to-ps-to-pdf-rules

# vim: filetype=make


==> bib/1-example-paper-templates/SET-UP-NEW-DOCUMENT <==
#!/bin/bash

# call this script to:
# - make all the soft links needed for the Makefile system
# - make all the soft links needed for latex include files
# - copy a skeleton Makefile.config (as Makefile.config-template)

#BIBGIT=$HOME/git-managed/bib--hagrid/
if [[ "$1" == "" ]]; then
    echo "usage: ${0/*\//} <PATH-TO-BIB-GIT>"
    echo "       eg, clone bib-git here (as a submodule, if this is already under git,"
    echo "see 1-example-paper-template/00-README-first for instructions) called ./bib/, and"
    echo "       ${0/*\//} ./bib"
    echo "or, ${0/*\//} ~/git-managed/bib--hagrid/"
    echo ""
    exit 1;
else
    BIBGIT="$1"
fi


MAKEFILES="
    Makefile.common
    Makefile.dvi-to-ps-to-pdf-rules
    Makefile.latex
    Makefile.latexmk
    Makefile.latexmkpdf
    Makefile.pdflatex
"

STYSCLSS="
    llncs.cls
    splncs04.bst
    sscol.cls
    siam10.clo
    siamltex.cls
    siamltex.sty
    algorithm2e.sty
    bibspacing.sty
    proposal.cls
"
# IEEEtran.bst - not recommended. Use the texlive builtin IEEEtran.bst
# IEEEtran.cls - not recommended. Use the texlive builtin IEEEtran.bst
# IEEEtranv1.7a-modified-by-aadithya.cls - 
# IEEEtranv1.7a.cls
# IEEEtranv1.8.cls
# tweaklist.sty - not recommended. enumitem is now used instead

PACKAGESNEWCMDS="
    package-and-newcommand-includes.tex
    package-and-newcommand-includes-llncs.tex
    package-and-newcommand-includes-cambridge.tex
    newcommands-eg-ie-etc.tex
    newcommands-for-bibtex.tex
    newcommands-highlight-ignore-comments-annotations.tex
    newcommands-labels-refs.tex
    newcommands-math.tex
    newcommands-misc.tex
    newcommands-squeeze-spaces.tex
    newcommands-thm-env.tex
    code-inclusion-config.tex
    colour-defs.tex
"

BIBFILES="
    stringdefs.bib
    PHLOGON-jr.bib
    aadithya.bib
    adiabatic-reversible.bib
    ag.bib
    amahmutoglu.bib
    gcj.bib
    jr-disto.bib
    jr.bib
    osc-SHIL-jr.bib
    tianshi.bib
    verification-hybrid-systems-CPS.bib
    von-Neumann-jr.bib
"

for i in $MAKEFILES; do
    ln -s $BIBGIT/1-example-paper-templates/$i .
done

for i in $STYSCLSS; do
    ln -s $BIBGIT/1-example-paper-templates/$i .
done

for i in $PACKAGESNEWCMDS; do
    ln -s $BIBGIT/1-example-paper-templates/$i .
done

echo ""
echo "done setting up soft links."

echo ""
echo "Making a soft link Makefile -> Makefile.latexmkpdf. Please change it, if you like."
ln -s Makefile.latexmkpdf Makefile

if [[ -e Makefile.config-template ]]; then
    echo ""
    echo "Makefile.config-template already exists, not touching it."
else
    echo "TOP = FILLTHISIN" > Makefile.config-template
    echo "OTHERSRCS = "$STYSCLSS $PACKAGESNEWCMDS >> Makefile.config-template
    echo "BIBGIT = $BIBGIT" >> Makefile.config-template 

    echo "SOFTLINKSTOSETUP = \\" >> Makefile.config-template 
    for bibfile in $BIBFILES; do
        echo "      "'$(BIBGIT)/'"$bibfile \\" >> Makefile.config-template 
    done
    echo "" >> Makefile.config-template 
    echo ""
    echo "Please copy Makefile.config-template to Makefile.config and update for your document."
    echo ""
    echo "If you want to dereference all the soft links (eg, for documents to be shared with"
    echo "people who don't have access to bib--github, run deference-softlinks"
    echo "in the directory [bib]/1-example-paper-template/."
    echo ""
fi



==> bib/1-example-paper-templates/acronyms-ABCD.tex <==
\begin{acronym}[abcd-cps]
	\acro{IO}[IO]{Input-Output}
	\acro{PD}[PD]{Proportional-Derivative}
	\acro{FSM}[FSM]{Finite State Machine}
	\acro{DAE}[DAE]{Differential Algebraic Equation}
	\acro{DAEs}[DAEs]{Differential Algebraic Equations}
	\acro{AMS}[AMS]{Analog-Mixed Signal}
	\acro{ABCD}[ABCD]{Accurate Booleanization of Continuous Dynamics}
	\acro{MAPP}[MAPP]{Berkeley Model and Algorithm Prototyping Platform}
	\acro{VAPP}[VAPP]{Verilog-A Parser and Processor}
	\acro{MODSPEC}[MODSPEC]{MODel SPECification}
	\acro{CPS}[CPS]{Cyber-Physical Systems}
	\acro{ABCD-CPS}[ABCD-CPS]{\ac{ABCD}-\ac{CPS}}
	\acro{ODE}[ODE]{Ordinary Differential Equation}
	\acro{ODEs}{ODEs}{Ordinary Differential Equations}
	\acro{HJI}[HJI]{Hamilton-Jacobi-Issacs}
	\acro{CTCV}[CT-CV]{Continuous-Time, Continuous-Valued}
	\acro{DTDV}[DT-DV]{Discrete-Time, Discrete-Valued}
\end{acronym}


==> bib/1-example-paper-templates/acronyms-STEAM.tex <==
\begin{acronym}[simulation]
        \acro{MNA}[MNA]{Modified Nodal Analysis}
	\acro{STEAM}[STEAM]{Spline-based Tables for Efficient and Accurate device Modelling}
	\acro{PSP}[PSP]{Penn State-Phillips}
	\acro{BSIM}[BSIM]{Berkeley Short-channel IGFET Model}
	\acro{BSIM3}[BSIM3v3.2.4]{Berkeley Short-channel IGFET Model - Version 3.2.4}
	\acro{MVS}[MVS]{MIT Virtual Source}
	\acro{MAPP}[MAPP]{Berkeley Modelling and Prototyping Platform}
        \acro{LMS}[LMS]{Linear Multi-Step}
        \acro{DAE}[DAE]{Differential-Algebraic Equation}
        \acro{GEAR}[GEAR]{GEAR}
        \acro{TRAP}[TRAP]{Trapeziodal}
        \acro{MODSPEC}[MODSPEC]{MODel SPECification}
        \acro{NR}[NR]{Newton-Raphson}
        \acro{wrt}[w.r.t]{with respect to}
\end{acronym}


==> bib/1-example-paper-templates/code-inclusion-config.tex <==
\lstloadlanguages{Matlab}
\lstset{language=Matlab,
        frame=single, % Single frame around code
        basicstyle=\scriptsize\ttfamily,
        % keywordstyle=[1]\color{blue}\bf, % Perl functions bold and blue
        keywordstyle=[3]\color{blue}\underbar, % Custom functions underlined and blue
        identifierstyle=, % Nothing special about identifiers                                         
        commentstyle=\usefont{T1}{pcr}{m}{sl}\color{MyDarkGreen}\scriptsize, 
            % Comments are in small dark green courier font
        stringstyle=\color{MyDarkRed}, 
        showstringspaces=false, % Don't put marks in string spaces
        tabsize=4, % 5 spaces per tab
        % 
        % Put standard functions not included in the default language here
        %morekeywords={rand},
        % Put function parameters here
        %morekeywords=[2]{on, off, interp},
        % Put user defined functions here
        %morekeywords=[3]{test},
        %
        morecomment=[l][\color{blue}]{...}, % Line continuation (...) like blue comment
        % numbers=left, % Line numbers on left
        % firstnumber=1, % Line numbers start with line 1
        % numberstyle=\tiny\color{blue}, % Line numbers are blue and small
        % stepnumber=5 % Line numbers go in steps of 5
}

% Creates a new command to include an Matlab script, the first parameter is the
% filename of the script (without .pl), the second parameter is the caption
\newcommand{\matlabscript}[2]{
    \begin{itemize}
    \item[]\lstinputlisting[caption=#2,label=#1]{#1}
    \end{itemize}
}



==> bib/1-example-paper-templates/colour-defs.tex <==
% various colours
\definecolor{mylightgrey}{rgb}{0.6,0.6,0.6}
\definecolor{mydarkgrey}{rgb}{0.3,0.3,0.3}
\definecolor{mybrown}{rgb}{0.6,0.2,0}
\definecolor{mylightgreen}{rgb}{0,1,0}
\definecolor{mydarkgreen}{rgb}{0,0.5,0}
\definecolor{MyDarkGreen}{rgb}{0.0,0.4,0.0} % This is the color used for comments
\definecolor{myorange}{rgb}{1,0.4,0}
\definecolor{mypurple}{rgb}{0.8,0,0.8}
\definecolor{MyDarkRed}{rgb}{0.4,0.0,0.0} % This is the color used for strings


==> bib/1-example-paper-templates/leeseshia-examples-environment.tex <==
% copied from Lee and Seshia's definitions.tex. JR, 2013/09/02.

% File giving definitions of commands and environments.
% Because of a latex bug with counters, this has to be included
% using \input not \include.
%
% Amount of indent in colored boxes
\def\boxIndent{0.3in}

%--------------------------------------------------------------------------
% Blocks of code and variables
\newcommand{\code}[1]{\texttt{#1}}
%--------------------------------------------------------------------------

% Colors. 
\definecolor{exampleColor}{rgb}{0.85,0.92,1.0}
%\definecolor{exampleColor}{rgb}{0.9, 0.9, 0.9}


%--------------------------------------------------------------------------
% Examples environment 
% NOTE: Because of this line, this has to be included using \input
% not \include.
\newcounter{example}
\numberwithin{example}{chapter}
% Allow the @ character to be part of a name
\makeatletter
\newenvironment{example}{
\refstepcounter{example}
\def\FrameCommand{\colorbox{exampleColor}}
\MakeFramed {\advance\hsize-\width \FrameRestore}
\begin{list}{}{
\setlength{\leftmargin}{\boxIndent}
\setlength{\rightmargin}{0in}}
\item
\textbf{Example \thechapter.\arabic{example}:}
} {
\end{list}
\endMakeFramed
}
% restore the @ character to special status
\makeatother
\renewcommand \theexample {\thechapter.\arabic{example}}

%--------------------------------------------------------------------------
% For examples that are to be kept on one page.
% NOTE: Because of this line, this has to be included using \input
% not \include.
\newcounter{exampleKeep}
% Allow the @ character to be part of a name
\makeatletter
\newenvironment{exampleKeep}{
\refstepcounter{example} % so that the examples are numbered properly for now
\begin{lrbox}{\@tempboxa}
\begin{minipage} {\columnwidth}
\refstepcounter{example}
% Unfortunately, quote also results in the color box not going to the
% right margin.
%\begin{quote}
\begin{list}{}{
\setlength{\leftmargin}{\boxIndent}
\setlength{\rightmargin}{0in}}
\item
\textbf{Example \thechapter.\arabic{example}:}
} {
%\end{quote}
\end{list}
\end{minipage}
\end{lrbox}
\colorbox{exampleColor}{\usebox{\@tempboxa}}
}
\newenvironment{exampleContinued}[1]{
\begin{lrbox}{\@tempboxa}
\begin{minipage} {\columnwidth}
\begin{list}{}{
\setlength{\leftmargin}{\boxIndent}
\setlength{\rightmargin}{0in}}
\item
\textbf{Example \ref{#1} (continued):}
} {
%\end{quote}
\end{list}
\end{minipage}
\end{lrbox}
\colorbox{exampleColor}{\usebox{\@tempboxa}}
}
% restore the @ character to special status
\makeatother
\renewcommand \theexample {\thechapter.\arabic{example}}



==> bib/1-example-paper-templates/newcommands-eg-ie-etc.tex <==
% eg, ie, etc, wrt, viz newcommands
\newcommand{\eg}{{\it e.g.\@}} % \@ for normal spacing after. use: \eg\/ or \eg,
\newcommand{\ie}{{\it i.e.\@}} 
\newcommand{\wrt}{{\it w.r.t.\@}}
\newcommand{\viz}{{\it viz.\@}}
\newcommand{\vs}{{\it vs.\@}}
\newcommand{\aka}{{\it aka}}
\newcommand{\apriori}{{\it a priori}}
\newcommand{\adhoc}{{\it ad-hoc}}
\newcommand{\etc}{\textit{etc.\@}}                                                
\newcommand{\perse}{\textit{per se\@}}                                                
\newcommand{\etal}{\textit{et. al.\@}}                                                
% etc defined so that there is only a single period after it if it is followed 
% by a period
% see: http://en.wikibooks.org/wiki/TeX/def                                      
% see: http://www.tug.org/pipermail/texhax/2004-July/002449.html                 
% see: http://en.wikibooks.org/wiki/TeX/if                                       
%\ifx \etc \undefined  DOES NOT WORK
%  %\def\myarg{#1}                                                                
%  %\def\myfullstop{.}                                                            
%  %\def\etc{#1}{\textit{etc} arg is ``\myarg'' \ifx\myarg\myfullstop\then.\else.#1\fi\/}
%\fi                                                                              
%\def\etc#1{\textit{etc}\ifx#1..\else.#1\fi} % WORKS                                     
%                        


==> bib/1-example-paper-templates/newcommands-for-bibtex.tex <==
\newcommand{\BP}{({\textbf{Best Paper}})} % used in bibliography
\newcommand{\BPnom}{({\textbf{Best Paper Nomination}})} % used in bibliography
\newcommand{\IP}{({\textbf{Invited}})} % used in bibliography
\newcommand{\presenter}[1]{#1} % used in bibliography
%\newcommand{\putDOI}[1]{#1}
\newcommand{\putDOI}[1]{}
\newcommand{\DP}{\textbf{(Distinguished Paper)}}


==> bib/1-example-paper-templates/newcommands-highlight-ignore-comments-annotations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% newcommands for ignoring, commenting, annotating, highlighting
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ignore}[1]{}
\let\IGNORE=\ignore
%\newcommand{\comment}[1]{} % conflicts with something predefined
\newcommand{\COMMENT}[1]{}
\newcommand{\jrcomment}[1]{{\color{blue}#1}}
\newcommand{\agcomment}[1]{{\color{mydarkgreen}#1}}
\let\agc=\agcomment
\let\jc=\jrcomment
\newcommand{\redHL}[1]{{\color{red}\bf #1}}
\newcommand{\REDHL}[1]{{\color{red}\bf #1}}
\newcommand{\blueHL}[1]{\textbf{\color{blue}#1}}
\newcommand{\greenHL}[1]{\textbf{\color{mydarkgreen}#1}}
\newcommand{\jsugg}[1]{\textit{\color{blue}#1}}
\newcommand{\jpvt}[1]{\textit{\color{red}#1}}
%\newcommand{\jsumm}[1]{{\color{blue}{{\uline{\textit{#1}}}}}}
\newcommand{\jsumm}[1]{\centerline{\color{blue}{{\uline{\textit{#1}}}}\\}}
\newcommand{\jkill}[1]{{\color{blue}\sout{#1}}}
\newcommand{\toputback}[1]{{\blueHL{PUT THIS BACK:} #1}}
\newcommand{\jemph}[1]{\textbf{\uline{#1}}}
\newcommand{\jques}[1]{{\color{blue}#1?}}
\let\jnoteignored=\ignore
	
%\newcommand{\jnote}[1]{\textit{\color{blue}#1}}
%\newcommand{\jnote}[1]{\centerline{\color{mydarkgreen}{{\uline{\textit{#1}}}}\\}}
%\newcommand{\jnote}[1]{{\color{mydarkgreen}\textit{\uline{#1}}}}
\newcommand{\jnote}[1]{{\color{mydarkgreen}\textit{{#1}}}}
\ignore{
    \newcommand{\jnote}[1]{% using fixme
    	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
    	\renewcommand{\fixmelogo}{}%
    	\hspace*{-0.35em}\raisebox{0.7em}[\height][\depth]
                {\\\makebox[0em][l]{\fxnote{\tiny{\color{myred}JR: }
                \textit{\color{mydarkgreen}#1}}}}%
    }
}
\let\jn=\jnote
\newcommand{\TOFIX}[1]{% using fixme
	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
	\renewcommand{\fixmelogo}{}%
	{\fxfatal{\bf\normalsize\textit{\color{myred}#1}}}%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END newcommands for ignoring, commenting, ....
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> bib/1-example-paper-templates/newcommands-labels-refs.tex <==
% label and ref newcommands
% now mostly deprecated (but redefined and kept for backward compatibility) - move to \cref from the cleveref package
%\crefname{algocf}{alg.}{algs.}
\crefname{algocf}{Algorithm}{Algorithms}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefname{equation}{}{}
\Crefname{equation}{}{}

%DONE: xyzref{} should be able to handle multiple arguments so that you can
%reference multiple figures/equations at the same time -AG
%Now fixed with some package/command CREF.
\newcommand{\eqnlabel}[1]{\label{#1}}
\newcommand{\eqnref}[1]{\cref{#1}}
\newcommand{\algolabel}[1]{\label{#1}}
\newcommand{\algoref}[1]{\cref{#1}}
\newcommand{\corrlabel}[1]{\label{corr:#1}}
\newcommand{\corrref}[1]{Corollary \ref{corr:#1}}
\newcommand{\assref}[1]{Assumption \ref{ass:#1}}
\newcommand{\asslabel}[1]{\label{ass:#1}}
%\newcommand{\eqnref}[1]{(\ref{eq:#1})}
%\newcommand{\eqnlabel}[1]{\label{eq:#1}}
%\newcommand{\figlabel}[1]{\label{fig:#1}}
%\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\lstlabel}[1]{\label{lst:#1}}
\newcommand{\lstref}[1]{Listing~\ref{lst:#1}}
\newcommand{\figlabel}[1]{\label{#1}}
\newcommand{\figref}[1]{\cref{#1}}
\newcommand{\chaplabel}[1]{\label{chap:#1}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\tablabel}[1]{\label{#1}}
\newcommand{\tabref}[1]{\cref{#1}}
\newcommand{\thlabel}[1]{\label{th:#1}}
\newcommand{\thref}[1]{Theorem~\ref{th:#1}}
\newcommand{\thmlabel}[1]{\label{thm:#1}}
\newcommand{\thmref}[1]{Theorem \ref{thm:#1}}
\newcommand{\remlabel}[1]{\label{rem:#1}}
\newcommand{\remref}[1]{Remark \ref{rem:#1}}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\lemlabel}[1]{\label{lem:#1}}
\newcommand{\lemref}[1]{Lemma \ref{lem:#1}}
\newcommand{\examplelabel}[1]{\label{#1}}
\newcommand{\exampleref}[1]{Example \cref{#1}}
%\newcommand{\labexample}[1]{\label{example:#1}}
\newcommand{\httpref}[1]{}
\let\el=\eqnlabel
\let\er=\eqnref


==> bib/1-example-paper-templates/newcommands-math.tex <==
%\newcommand{\ddt}[2]{{\frac{d}{d #2}\left. #1 \right.}}
\newcommand{\ddt}[2]{{\frac{d #1}{d #2}}}
\newcommand{\ddx}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand{\Ddx}[2]{{\frac{D}{d{#2}}\left[ #1 \right]}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\deq}{\triangleq}
\newcommand{\I}{I\left[\right]}
\newcommand{\ELL}[1]{L\left[#1\right]}
\newcommand{\w}{\omega}
\newcommand{\calD}{{\cal D}}
\renewcommand{\jmath}{j}
\newcommand{\Pinvt}{{P(t)}^{-1}}
\newcommand{\halmos}{\hskip\textwidth minus\textwidth \rule{6pt}{6pt}}
\newcommand{\calA}{{\cal A}}
\newcommand{\calAT}{{\cal A}^T}
\newcommand{\calL}{{\cal L}}
\newcommand{\calLadj}{\calL^\dagger}
\newcommand{\calR}{{\cal R}}
%\newcommand{\Reals}{\Bbb{R}}
%\newcommand{\Real}{\Bbb{R}}
\newcommand{\Reals}{\mathbf{R}}
\newcommand{\Real}{\mathbf{R}}
\newcommand{\Safe}{\ensuremath{{\bf S}}}
\newcommand{\Pade}{{Pad\'e}}
\newcommand{\Complexes}{\Bbb{C}}
\newcommand{\HvecqLanc}{\Hvec^{(L)}_q}
\newcommand{\HvecqArn}{\Hvec^{(A)}_q}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\calDT}{{\cal D}^T}
\newcommand{\calCtil}{\tilde{\cal C}}
\newcommand{\calJtil}{\tilde{\cal J}}
\newcommand{\calDtil}{\tilde{\cal D}}
\newcommand{\JstarDphi}{J_{\Delta \phi}^*}
\newcommand{\Jstarphi}{J_{\phi}^*}
\newcommand{\vecbphi}{\vec b_{\phi}}
\newcommand{\vecbext}{\vec b_{\text{ext}}}
\newcommand{\phistarIdeal}{\phi_{\text{ideal}}^*}
\newcommand{\apdx}[1]{\appref{#1}} 
\newcommand{\delbydel}[2]{\ensuremath{\frac{\partial {#1}}{\partial {#2}}}}
\newcommand{\delbydeln}[3]{\ensuremath{\frac{\partial^{{#1}}
{#2}}{\partial{#3}^{{#1}}}}}
\newcommand{\delbydelat}[3]{\ensuremath{\left. \frac{\partial
{#1}}{\partial {#2}} \right|_{{#3}}}}
\newcommand{\dee}{\ensuremath{\mathrm{d}}}
\newcommand{\dbyd}[2]{\ensuremath{\frac{\mathrm{d} {#1}}{\mathrm{d}
{#2}}}}
\newcommand{\dbydn}[3]{\ensuremath{\frac{\mathrm{d}^{{#1}}{#2}}
{\mathrm{d}{#3}^{{#1}}}}}
\newcommand {\dist}[1] {{{\rm dist}\left({#1}\right)}}
\def\Matrix#1{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\textdiag}{{\text{diag}}}
\newcommand{\ihat}{\hat{\imath}}
\newcommand{\jhat}{\hat{\jmath}}
\newcommand{\khat}{\hat{k}}
\newcommand{\del}{\nabla}
\newcommand{\Rxx}{R_{\vec x \vec x}}
\newcommand{\Sxx}{S_{\vec x \vec x}}
\newcommand{\Snn}{S_{\vec n \vec n}}
\newcommand{\vecphi}{\vec \phi}
\newcommand{\Dphi}{\Delta \phi}
\newcommand{\vecDphi}{\vv{\Delta \phi}}
\newcommand{\dphi}{\delta \phi}
\newcommand{\vecdphi}{\vv{\delta \phi}}
\newcommand{\ah}{\alpha_g} % g for group
%\newcommand{\tDagger}{{\tilde t}}
\newcommand{\tDagger}{{t^{\!\dagger}}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\texthyphen}{\text{--}}
\DeclareMathOperator*{\argmax}{arg\,max} % depends on amsmath. Use \argmax_x
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\sgn}{sgn}

%The substack command can be used to produce a multi-line subscripts or superscripts:
%\sum_{\substack{0\le i\le m\\ 0<j<n}} P(i,j) produces a two-line subscript underneath the sum.
%A slightly more general form is the subarray environment which allows you to specify that each line should be left-aligned instead of centered, as here:
% \sum_{\begin{subarray}{l} i\in\Lambda\\ 0<j<n \end{subarray}} P(i,j) 

%\newcommand{\be}[1]{\begin{equation}\eqnlabel{#1}} % now moved to cleveref
\newcommand{\be}[1]{\begin{equation}\label{#1}}
\def\ee{\end{equation}}


==> bib/1-example-paper-templates/newcommands-misc.tex <==
% Misc. commands
%\newcommand{\website}{http://www.eecs.berkeley.edu/\char126 jr/NOW-FT-Monograph/}

%\newcommand{\figdir}{./figures} % best to define this in the main tex file

% \newcommand{\bibdir}{.} % ditto

\newif\ifjournalsub
\newcommand{\ifthen}[2]{\ifthenelse{#1}{#2}{}}
\newcommand{\iftr}[1]{\boolean{#1}}

\newcommand{\DAEtoFSM}{ABCD}
\newcommand{\Brangluin}{Brangluin}
\newcommand{\LTIMORrefs}{pillage1,FeFr95a,OdCePiTCAD98,PhDaSiDAC2002,PhSiPMTBRDATE2004}
\newcommand{\nonlinearMORrefs}{RoTVPTCAS99,ReWhTCAD2003,PhTCAD2003,DoRoTCADPWP2008,
                               GuRoICCAD2008maniMOR}
\newcommand{\MORrefs}{\LTIMORrefs,\nonlinearMORrefs}
\newcommand{\proposalAcronym}{THz-PHLOGON}
\newcommand{\website}{http://www.eecs.berkeley.edu/$\sim$jr/NOW-FT-Monograph/}
\newcommand{\PNJLIM}{\textsf{\small PNJLIM}}
%\newcommand{\MATLAB}{\textbf{MATLAB}$^{\texttrademark}$}
\newcommand{\MATLAB}{MATLAB$^\text{\textregistered}$}

%%%% misc formatting setup
\newlength{\colwidth}
\newcommand{\pswidthcoeff}{0.9}
\newcommand{\psheightcoeff}{0.6}
\newlength{\pgwid}



% make LaTeX less fussy about line breaks, so that it typsets inline 
% math without overflowing -- perhaps remove if it causes trouble.
\sloppy 
\setcounter{secnumdepth}{5}  % numbered \paragraph == \subsubsubsection

% remove indentation from subparagraph
\makeatletter
\renewcommand\subparagraph{%
 \@startsection {subparagraph}{5}{\z@ }{3.25ex \@plus 1ex
 \@minus .2ex}{-1em}{\normalfont \normalsize \bfseries }}%
\makeatother

%a proper longemdash, that doesn't make me feel like putting spaces around it:
\newcommand{\longemdash}{\rule[.5ex]{1.3em}{0.5pt}}

\pagenumbering{arabic}
%\renewcommand{\thepage} {Body--\arabic{page}}
\hyphenation{op-tical net-works semi-conduc-tor} % correct bad hyphenation here



==> bib/1-example-paper-templates/newcommands-squeeze-spaces--no-titlesec.tex <==
\ignore{ TWEAKLIST OFTEN CAUSES ERRORS
%%% tweaklist renewcommands - 
\newcommand{\modifiedListParamters}{
  \setlength{\topsep}{0pt}%
  \setlength{\itemsep}{-0.1em}
  \setlength{\partopsep}{0em}
  \setlength{\parsep}{0em}
  \setlength{\leftmargin}{1.1em}
  \setlength{\itemindent}{0.0em}
}
\renewcommand{\enumhook}{
  \modifiedListParamters
  \setlength{\itemindent}{0.2em}
}
\renewcommand{\itemhook}{
  \modifiedListParamters
}
\renewcommand{\descripthook}{
  \modifiedListParamters
  \setlength{\itemindent}{-1.0em}
}
%%% end tweaklist renewcommands
}

% same functionality as tweaklist (but better?)
\let\labelindent\relax % to fix conflict with IEEEtran,otherwise not reqd?
\usepackage{enumitem}
\setenumerate{leftmargin=1em,itemindent=0em,labelindent=0em,itemsep=0em} % sets it globally.
% you can do it on a per list basis like this:
% \begin{enumerate}[leftmargin=1em,itemindent=0em,labelindent=0em,itemsep=0em]
%   \item ...
% \end{enumerate}


\ignore{not usually needed, but the definitions have useful info
		Space saving List environment for enumerations.

	\newcounter{myctr}
	\newenvironment{mylist}{\begin{list}{\arabic{myctr}.}
   		{\usecounter{myctr}
   		%\setlength{\topsep}{1mm}\setlength{\itemsep}{0.5mm}
   		\setlength{\topsep}{0.3mm}
   		\setlength{\itemsep}{0mm}
   		\setlength{\parsep}{0.3mm}
   		\setlength{\itemindent}{0mm}
   		\setlength{\partopsep}{0mm}
   		\setlength{\labelwidth}{15mm}
   		\setlength{\leftmargin}{4mm}
   		}
	}{\end{list}}

	\newenvironment{myitemize}{\begin{list}{$\bullet$}
	  \ignore{\setlength{\topsep}{0.8mm}\setlength{\itemsep}{0.25mm}}
	  {\setlength{\topsep}{1mm}\setlength{\itemsep}{0.25mm}
	  \setlength{\parsep}{0.1mm}
	  \setlength{\itemindent}{0mm}\setlength{\partopsep}{0mm}
	  \setlength{\labelwidth}{15mm}
	  \setlength{\leftmargin}{4mm}}
	}{\end{list}}
}

%%%%% titlesec: squeezing whitespace between section headings
%	\titlespacing{\section}{0pt}{*0}{*0.1} % {0pt} is indentation; {*0} is 
%                                           % space above; {*0.5} is space below
%	%\titlespacing{\subsection}{0pt}{*0.1}{*0.7}
%	\titlespacing{\subsection}{0pt}{*0.1}{*0.1}
%	\titlespacing{\subsubsection}{0pt}{*0.1}{*0}
%%%%% end titlesec

%%%% squeezing whitespace in and around figures
    \floatsep=0em % space left between floats.
    \textfloatsep=0em % space between last top float or first bottom float and the text.
    \intextsep=0em % space left on top and bottom of an in-text float.
    %\dbltextfloatsep is \textfloatsep for 2 column output.
    %\dblfloatsep is \floatsep for 2 column output.
    \abovecaptionskip=0em % space above caption
    \belowcaptionskip=0em % space below caption
%%%% END squeezing whitespace in and around figures

\makeatletter
\g@addto@macro\normalsize{%
  \setlength\abovedisplayskip{1pt}
  \setlength\belowdisplayskip{1pt}
  \setlength\abovedisplayshortskip{1pt}
  \setlength\belowdisplayshortskip{1pt}
}
\makeatother

%\newcommand{\mycaption}[1]{\caption{\small #1}}
\newcommand{\mycaption}[1]{\caption{\tiny #1}}

% for captions spacing
%\captionsetup[table]{font={scriptsize},format=hang,indention=0em}     %% change 1.2 as you like
\captionsetup[table]{font={small},indention=0.2em}     %% change 1.2 as you like
%\captionsetup[figure]{font={scriptsize},format=hang,indention=0em}    %% change as you like
\captionsetup[figure]{font={small},indention=0.2em}    %% change as you like
 %% or
 %% \captionsetup{font={stretch=1.2}}  %% this affects both figure and table

% replace Figure x in captions by Fig. x
%\renewcommand{\figurename}{Fig.} % doesn't work.
%but \usepackage[figurename=Fig.]{caption} in packages-headers.tex does work.


%\renewcommand{\baselinestretch}{1.5}
%\setstretch{1.5}

%\def\baselinestretch{0.8593}\large\normalsize - this form works locally?
%\renewcommand{\baselinestretch}{0.94} - this form works only in the preamble
%\renewcommand{\baselinestretch}{0.90}
%\renewcommand{\baselinestretch}{0.5}
%\linespread{0.5} % 0.5 -> 7 lines per inch; 0.9 -> a bit more than 6 lines 
%                 % per vertical inch
% \linespread{0.99}

% baselinestretch fixes for squeezing. See also linespread
%\def\ssp{\def\baselinestretch{0.95645}\large\normalsize} % "single space"
%\def\ssp{\def\baselinestretch{0.905}\large\normalsize} % "single space"
\def\ssp{\def\baselinestretch{0.9}\large\normalsize} % "single space"
\def\dsp{\def\baselinestretch{1.35}\large\normalsize} % "double space"
\ssp

% indent paragraphs less (saves space)
\parindent 	1em
% do not indent paragraphs (saves more space)
\parindent 	0em
% adjust space between paragraphs (0em can obscure paragraph breaks)
\parskip 0.3em

% vim: guifont=mono\ 11


==> bib/1-example-paper-templates/newcommands-squeeze-spaces.tex <==
\input newcommands-squeeze-spaces--no-titlesec
%%%% titlesec: squeezing whitespace between section headings
	\titlespacing{\section}{0pt}{*0}{*0.1} % {0pt} is indentation; {*0} is 
                                           % space above; {*0.5} is space below
	%\titlespacing{\subsection}{0pt}{*0.1}{*0.7}
	\titlespacing{\subsection}{0pt}{*0.1}{*0.1}
	\titlespacing{\subsubsection}{0pt}{*0.1}{*0}
%%%% end titlesec

% vim: guifont=mono\ 11


==> bib/1-example-paper-templates/newcommands-thm-env.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% theorem-like environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\EndProof{\hfill \quad \vrule width 1ex height 1ex depth 0pt  }
\newtheorem{corollary}{Corollary}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
%\newtheorem{illustration}{Illustration}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{defn}{Definition}[section]
\newtheorem{notation}{Notation}
\newtheorem{theorem}{Theorem}
\newenvironment{sketch}{\noindent{\bf Sketch of Proof}:}{\halmos}
\newenvironment{conjecture}{\noindent{\bf Conjecture}: \em}{}
\newcommand{\numberedtheorem}[3]{
	\ifthen{\not\equal{#1}{}}{
		\let\oof=\thetheorem
		\renewcommand{\thetheorem}{#1}
	}
	\begin{theorem}
	\ifthen{\not\equal{#2}{}}{
		\thmlabel{#2}
	}
	#3
	\end{theorem}
	\ifthen{\not\equal{#1}{}}{
		\let\thetheorem=\oof
		\addtocounter{theorem}{-1}
	}
}
\newcommand{\numberedlemma}[3]{
	\ifthen{\not\equal{#1}{}}{
		\let\oof=\thelemma
		\renewcommand{\thelemma}{#1}
	}
	\begin{lemma}
	\ifthen{\not\equal{#2}{}}{
		\lemlabel{#2}
	}
	#3
	\end{lemma}
	\ifthen{\not\equal{#1}{}}{
		\let\thelemma=\oof
		\addtocounter{lemma}{-1}
	}
}


==> bib/1-example-paper-templates/package-and-newcommand-includes-cambridge.tex <==
  \usepackage{subfigure}
  \usepackage{fancyvrb} % to work around problems with listings, below
  \usepackage{savesym} % to work around problems with listings, below
  \savesymbol{abovecaptionskip}
  \savesymbol{belowcaptionskip}
  \usepackage{listings} % - conflicts with EngC - \abovecaptionskip already defined
  \usepackage{lstautogobble} % gobbles initial spaces
  \restoresymbol{EngC}{abovecaptionskip} % now EngC's abovecaptionskip is \EngCabovecaptionskip
  \restoresymbol{EngC}{belowcaptionskip} % 
  \usepackage[dvipsnames]{xcolor} % for color commands

    \lstset{ %
      %backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
      %basicstyle=\tt\small,        % the size of the fonts that are used for the code
      basicstyle=\tt\scriptsize,        % the size of the fonts that are used for the code
      breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
      breaklines=false,                 % sets automatic line breaking
      captionpos=b,                    % sets the caption-position to bottom
      commentstyle=\color{OliveGreen},    % comment style
      deletekeywords={...},            % if you want to delete keywords from the given language
      escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
      extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
      keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
      keywordstyle=\color{blue},       % keyword style
      language=python,                 % the language of the code
      morekeywords={*,...},            % if you want to add more keywords to the set
      numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
      numbersep=5pt,                   % how far the line-numbers are from the code
      numberstyle=\tiny\color{black}, % the style that is used for the line-numbers
      rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
      showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
      showstringspaces=true,          % underline spaces within strings only
      showtabs=true,                  % show tabs within strings adding particular underscores
      stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
      stringstyle=\color{black},     % string literal style
      tabsize=1,                       % sets default tabsize to 2 spaces
      frame = none,
      frame=single,                    % adds a frame around the code
      fancyvrb = true,
      columns = fullflexible,
      autogobble = true                % gobble up leading spaces
    }


  \usepackage{sverb} % defines the listing environment
% \documentclass[multi]{EngC} % multi-contributor option
% \documentclass[prodtf]{EngC}% if you have helvetica neue condensed fonts

  \usepackage[rightcaption,raggedright]{sidecap}% for side captions
  \usepackage{framed}         % for floatingboxes
  \usepackage{soul}           % for letterspacing in theorem-style headings

% for the Harvard author-date referencing system
  %\usepackage[agsm]{harvard}

% if you are using either vancouver.bst or IEEEtran.bst and wish to remove
% square braces in the reference list, uncomment the line below
% \removesquarebraces

  \usepackage{rotating}
  \usepackage{floatpag}
  \rotfloatpagestyle{empty}

  \usepackage{amsmath}% if you are using this package,
                     % it must be loaded before amsthm.sty

  %\usepackage{amstext} % provides \text, but this is included by amsmath
  \usepackage{amsthm}
  \usepackage{amssymb} % provides mathbb, replacement for \Bbb
% \usepackage{txfonts}% times font (used to produce EngCguide.pdf)
                      % this package must be loaded after amsthm.sty
  \usepackage{amsxtra} % \sphat, \sptilde (A\sphat)
  \usepackage{graphicx}
  \usepackage{epsfig}
  %\usepackage[subfigure]{tocloft} % to solve problem with BYUTextbook
  %\usepackage{mathptmx} % conflict with tocloft % old/deprecated; see https://tex.stackexchange.com/questions/347244/how-can-i-adjust-the-fontsize-of-greek-letters-only
  \usepackage{newtxtext} % https://tex.stackexchange.com/questions/347244/how-can-i-adjust-the-fontsize-of-greek-letters-only
  \usepackage{newtxmath} % https://tex.stackexchange.com/questions/347244/how-can-i-adjust-the-fontsize-of-greek-letters-only
  \usepackage[compress,capitalise,noabbrev]{cleveref} % conflict with tocloft
  \usepackage{algorithm2e}
  %\usepackage[noend, boxruled, linesnumbered] {algorithm2e}


  %\usepackage[final]{showlabels}


% indexes
% uncomment the relevant set of commands

% for a single index
% \usepackage{makeidx}
% \makeindex

% for multiple indexes using multind.sty
  % \usepackage{multind}\ProvidesPackage{multind} % EngC only
  % \makeindex{authors}
  % \makeindex{subject}

%% showlabels should be the LAST package loaded
%\RequirePackage{showkeys}
\RequirePackage[outer,draft]{showlabels}
%\RequirePackage[inline]{showlabels}
%\showlabel{cite}
%\showlabel{label}
\renewcommand{\showlabelfont}{\tiny\ttfamily\color{blue}}
%\renewcommand{\showlabelsetlabel}[1]{\tiny #1}

%%%%%%%%%%%%%%%%%% END PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%

% for code listings

% for multiple indexes using index.sty
% \usepackage{index}
% \newindex{aut}{adx}{and}{Author index}
% \makeindex

  \newcommand\cambridge{EngC}

% see chapter 3 for details
  %\theoremstyle{plain}% default
  %\newtheorem{theorem}{Theorem}[chapter]
  %\newtheorem{lemma}[theorem]{Lemma}
  %\newtheorem*{corollary}{Corollary}

  %\theoremstyle{definition}
  %\newtheorem{definition}[theorem]{Definition}
  %\newtheorem{condition}[theorem]{Condition}

  %\theoremstyle{remark}
  %\newtheorem{remark}{Remark}[chapter]
  %\newtheorem{notation}[remark]{Notation}
  %\newtheorem*{case}{Case}

  \hyphenation{line-break line-breaks docu-ment triangle cambridge amsthdoc
    cambridgemods baseline-skip author authors cambridgestyle en-vir-on-ment polar}

  \setcounter{tocdepth}{2}% the toc normally lists sections;
% for the purposes of this document, this has been extended to subsections

\input colour-defs
\let\ignore\relax % undefines \ignore, which EngC seems to define to something
\input newcommands-highlight-ignore-comments-annotations
\input newcommands-eg-ie-etc
\input newcommands-labels-refs
\input newcommands-math
%\input newcommands-thm-env
\input newcommands-for-bibtex
%\input newcommands-squeeze-spaces
%\input leeseshia-examples-environment
\input newcommands-misc

% figdir



==> bib/1-example-paper-templates/package-and-newcommand-includes-llncs.tex <==
%%%%%%%%%%%%%%%%%% PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%
\RequirePackage{times}
\RequirePackage{mathptm} % - AG (Don't like \mathcal{C} that this produces
\RequirePackage{mathptmx} % times (smaller) math fonts, greek characters also italicized
%\RequirePackage[usenames]{pstcol} 
\RequirePackage[usenames]{pstricks} 

% Graphics (figures/images etc.)
%\usepackage[pdftex]{graphicx}
\RequirePackage{graphicx} % supplies \includegraphics
\graphicspath{{./octave-figures/}{./results/}{./figures/}{./snapshots/}}
\DeclareGraphicsExtensions{.eps,.pdf,.jpeg,.png,.jpg}

\RequirePackage{rotating}
\RequirePackage{indentfirst} 
\RequirePackage{color} 
%\RequirePackage{picins} 
\RequirePackage{bmpsize} 
\RequirePackage{epsfig} % good old way of including figures
\RequirePackage{eepic} 
\RequirePackage{subfigure} % put figures side-by-side
\RequirePackage{wrapfig} % wrap text around figures
\RequirePackage{picinpar} % alternative to wrapfig, less useful

% Math (symbols/equations etc.)
\usepackage{cancel}
\RequirePackage{amsmath,amssymb,amsbsy,amsfonts,dotlessj} 
\RequirePackage{latexsym}
\RequirePackage{bm} % boldmath
\DeclareMathVersion{bold} 

% Formatting
\RequirePackage{multicol}
\RequirePackage{esvect} % defines \vv{}
\RequirePackage{ifthen}
\RequirePackage{etoolbox}
\RequirePackage{relsize}
\RequirePackage{soul}   % Provides \hl{some-text}
%\RequirePackage{showkeys} 
%\RequirePackage[final,notref]{showkeys} 
%\RequirePackage[top=0.8cm,bottom=0.8cm,left=0.8cm,right=0.8cm,nohead,nofoot]{geometry}
%\RequirePackage[top=1.2cm,bottom=1.3cm,left=1.2cm,right=1.2cm,nohead,nofoot]{geometry}

\usepackage[nolist,nohyperlinks]{acronym}
\RequirePackage{setspace}
\RequirePackage{moreverb}
\RequirePackage{ulem} % provides \uline
        \let\em=\it % ulem package redefines \em=\uline
\RequirePackage[sectionbib]{chapterbib}
\RequirePackage{fancyhdr}
\RequirePackage{array}
\RequirePackage{floatflt} % does (to some extent) work inside itemize environment %
                          % use \fltditem, see $LATEXDOCS/floatflt.pdf, esp. Sec 3.1
\RequirePackage{srcltx}
\RequirePackage{chemarrow}

% Utilities
\RequirePackage{todonotes}
\RequirePackage{tcolorbox}
\RequirePackage{fixme}
\RequirePackage[footnotesize,bf,figurename=Fig.,hang]{caption}
%\usepackage[scriptsize,hang,bf]{caption}
%\RequirePackage[hypertex]{hyperref} 
\RequirePackage[bookmarks,hidelinks=true]{hyperref} 
\RequirePackage[depth=subsection]{bookmark}
%\definecolor{linkColor}{rgb}{0.1,0.1,0.8}
%\usepackage[colorlinks=true,bookmarks,pdfpagemode=UseOutlines,linkcolor=linkColor,citecolor=linkColor,pagecolor=blue,urlcolor=blue,pdftitle={Verification, Learning, Control},pdfauthor={Jaijeet Roychowdhury},plainpages=false]{hyperref}

%\usepackage{./tweaklist} % allow changing of item spacings in standard itemize,
                         % enumerate, description environments
					     %%% tweaklist: compress lists. Also check out 
                         %%% \usepackage{mdwlist} (use itemize*, enumerate*, 
                         %%% description* with that)
                         % enumhook for the enumerate environment, itemhook for
                         % the itemize environment, and descripthook for the
                         % description environment.
                         % HOWEVER, CAUSES ERRORS. Use enumitem instead.

% enumitem package included from newcommands-squeeze-spaces.tex

\providecommand{\subparagraph}{} % needed for IEEEtran.cls (which does not define subparagraph); \providecommand checks if it is already defined
\RequirePackage[small,compact]{titlesec} % squeezing whitespace between section heading
\RequirePackage[sectionbib,square,sort&compress,numbers]{natbib} % needed for IEEEtran; but proposal.cls pulls it in automatically
%\RequirePackage{cite} % natbib doesn't like this
\RequirePackage{lipsum}
\RequirePackage{microtype}
\RequirePackage{url}
\RequirePackage{listings} % Required for insertion of code
\RequirePackage{multirow}
\RequirePackage{booktabs}
% load cleveref last, but before algorithm2e (which breaks cleveref)
\RequirePackage[compress,capitalise,noabbrev]{cleveref} % defines \cref, \Cref, etc; options are compress (don't sort), sort (don't compress), sort&compress (default), nosort (neither sort nor compress)
%\RequirePackage{algorithmic}
%\RequirePackage{algorithm}
%\RequirePackage[boxed,algoruled]{algorithm2e}
\RequirePackage[boxed,algoruled,linesnumbered,vlined,nofillcomment]{algorithm2e}
%\usepackage[yyyymmdd,hhmmss]{datetime} % use: Compiled on \today\ at \currenttime
\usepackage{datetime2} % ]use: Compiled on \DTMnow. And do \documentstyle[pacific]{...}

%%%%%%%%%%%%%%%%%% END PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%

% fixme package setup
\fxsetup{ status=draft,
		  %author={\tiny JR},
	  	  layout=footnote,
		  layout=inline, % also try footnote or pdfnote
		  theme=color,
	  	  marginclue
}
\definecolor{mydarkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{myred}{rgb}{0.9,0.0,0.0}
%\definecolor{fxnote}{rgb}{0.8000,0.0000,0.0000}
\renewcommand{\englishlistfixmename}{List of changes needed}
% Decrease spacing between items in bib
\newcommand{\BIBdecl}{\setlength{\itemsep}{0.25 em}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Multi-column the bib
%\patchcmd{\thebibliography}
%  {\list}
%  {\begin{multicols}{2}\list}
%    {}
%    {}
%\appto{\endthebibliography}{\end{multicols}}

%------------------------------------------------------------------------------
%   CODE INCLUSION CONFIGURATION
%------------------------------------------------------------------------------

\lstloadlanguages{Matlab}
\lstset{language=Matlab,
        frame=single, % Single frame around code
        basicstyle=\scriptsize\ttfamily,
        % keywordstyle=[1]\color{blue}\bf, % Perl functions bold and blue
        keywordstyle=[3]\color{blue}\underbar, % Custom functions underlined and blue
        identifierstyle=, % Nothing special about identifiers                                         
        commentstyle=\usefont{T1}{pcr}{m}{sl}\color{green}\scriptsize, 
            % Comments are in small dark green courier font
        stringstyle=\color{red}, 
        showstringspaces=false, % Don't put marks in string spaces
        tabsize=4, % 5 spaces per tab
        % 
        % Put standard functions not included in the default language here
        %morekeywords={rand},
        % Put function parameters here
        %morekeywords=[2]{on, off, interp},
        % Put user defined functions here
        %morekeywords=[3]{test},
        %
        morecomment=[l][\color{blue}]{...}, % Line continuation (...) like blue comment
        % numbers=left, % Line numbers on left
        % firstnumber=1, % Line numbers start with line 1
        % numberstyle=\tiny\color{blue}, % Line numbers are blue and small
        % stepnumber=5 % Line numbers go in steps of 5
}

% Creates a new command to include an Matlab script, the first parameter is the
% filename of the script (without .pl), the second parameter is the caption
\newcommand{\matlabscript}[2]{
    \begin{itemize}
    \item[]\lstinputlisting[caption=#2,label=#1]{#1}
    \end{itemize}
}

\input{colour-defs}
\input{newcommands-highlight-ignore-comments-annotations}
\input{newcommands-labels-refs}
\input{newcommands-eg-ie-etc}
\input{newcommands-for-bibtex} % BP, BPnom, IP, presenter, putDOI, DP, etc
\input{newcommands-misc}
\input{newcommands-squeeze-spaces}
\input{newcommands-math}
% \input newcommands-thm-env




==> bib/1-example-paper-templates/package-and-newcommand-includes-plain-llncs-noTimes.tex <==
%%%%%%%%%%%%%%%%%% PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%

% Graphics (figures/images etc.)
%\usepackage[pdftex]{graphicx}
\RequirePackage{graphicx} % supplies \includegraphics
\graphicspath{{./octave-figures/}{./results/}{./figures/}{./snapshots/}}
\DeclareGraphicsExtensions{.eps,.pdf,.jpeg,.png,.jpg}

\RequirePackage{color} 
\RequirePackage{epsfig} % good old way of including figures
\RequirePackage{subfigure} % put figures side-by-side
\RequirePackage{wrapfig} % wrap text around figures

% Math (symbols/equations etc.)
\usepackage{cancel}
\RequirePackage{amsmath,amssymb,amsbsy,amsfonts,dotlessj} 
\RequirePackage{latexsym}
\RequirePackage{bm} % boldmath
\DeclareMathVersion{bold} 

% Formatting
%\RequirePackage{showkeys} 
%\RequirePackage[final,notref]{showkeys} 
%\RequirePackage[top=0.8cm,bottom=0.8cm,left=0.8cm,right=0.8cm,nohead,nofoot]{geometry}
%\RequirePackage[top=1.2cm,bottom=1.3cm,left=1.2cm,right=1.2cm,nohead,nofoot]{geometry}

\usepackage[nolist,nohyperlinks]{acronym}
%\RequirePackage{setspace}
\RequirePackage{ulem} % provides \uline
        \let\em=\it % ulem package redefines \em=\uline
%\RequirePackage[sectionbib]{chapterbib}
%\RequirePackage{fancyhdr}
%\RequirePackage{array}
%\RequirePackage{floatflt} % does (to some extent) work inside itemize environment %
                          % use \fltditem, see $LATEXDOCS/floatflt.pdf, esp. Sec 3.1
%\RequirePackage{srcltx}
%\RequirePackage{chemarrow}

% Utilities
%\RequirePackage{todonotes}
%\RequirePackage{tcolorbox}
\RequirePackage{fixme}
\RequirePackage[footnotesize,bf,figurename=Fig.,hang]{caption}
%\usepackage[scriptsize,hang,bf]{caption}
%%\RequirePackage[hypertex]{hyperref} 
\RequirePackage[bookmarks,hidelinks=true]{hyperref} 
%\RequirePackage[depth=subsection]{bookmark}
%\definecolor{linkColor}{rgb}{0.1,0.1,0.8}
%\usepackage[colorlinks=true,bookmarks,pdfpagemode=UseOutlines,linkcolor=linkColor,citecolor=linkColor,pagecolor=blue,urlcolor=blue,pdftitle={Verification, Learning, Control},pdfauthor={Jaijeet Roychowdhury},plainpages=false]{hyperref}

%\usepackage{./tweaklist} % allow changing of item spacings in standard itemize,
                         % enumerate, description environments
					     %%% tweaklist: compress lists. Also check out 
                         %%% \usepackage{mdwlist} (use itemize*, enumerate*, 
                         %%% description* with that)
                         % enumhook for the enumerate environment, itemhook for
                         % the itemize environment, and descripthook for the
                         % description environment.
                         % HOWEVER, CAUSES ERRORS. Use enumitem instead.

% enumitem package included from newcommands-squeeze-spaces.tex

%\providecommand{\subparagraph}{} % needed for IEEEtran.cls (which does not define subparagraph); \providecommand checks if it is already defined
%\RequirePackage[small,compact]{titlesec} % squeezing whitespace between section heading
%\RequirePackage[sectionbib,square,sort&compress,numbers]{natbib} % needed for IEEEtran; but proposal.cls pulls it in automatically
%\RequirePackage{cite} % natbib doesn't like this
%\RequirePackage{lipsum}
%\RequirePackage{microtype}
\RequirePackage{url}
%\RequirePackage{listings} % Required for insertion of code
%\RequirePackage{multirow}
%\RequirePackage{booktabs}
% load cleveref last, but before algorithm2e (which breaks cleveref)
\RequirePackage[compress,capitalise,noabbrev]{cleveref} % defines \cref, \Cref, etc; options are compress (don't sort), sort (don't compress), sort&compress (default), nosort (neither sort nor compress)
%\RequirePackage{algorithmic}
%\RequirePackage{algorithm}
%\RequirePackage[boxed,algoruled]{algorithm2e}
%\RequirePackage[boxed,algoruled,linesnumbered,vlined,nofillcomment]{algorithm2e}
%\usepackage[yyyymmdd,hhmmss]{datetime} % use: Compiled on \today\ at \currenttime
%\usepackage{datetime2} % ]use: Compiled on \DTMnow. And do \documentstyle[pacific]{...}

%%%%%%%%%%%%%%%%%% END PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%

% fixme package setup
\fxsetup{ status=draft,
		  %author={\tiny JR},
	  	  layout=footnote,
		  layout=inline, % also try footnote or pdfnote
		  theme=color,
	  	  marginclue
}
\definecolor{mydarkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{myred}{rgb}{0.9,0.0,0.0}
%\definecolor{fxnote}{rgb}{0.8000,0.0000,0.0000}
\renewcommand{\englishlistfixmename}{List of changes needed}
%% Decrease spacing between items in bib
%\newcommand{\BIBdecl}{\setlength{\itemsep}{0.25 em}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Multi-column the bib
%\patchcmd{\thebibliography}
%  {\list}
%  {\begin{multicols}{2}\list}
%    {}
%    {}
%\appto{\endthebibliography}{\end{multicols}}

%------------------------------------------------------------------------------
%   CODE INCLUSION CONFIGURATION
%------------------------------------------------------------------------------

% \lstloadlanguages{Matlab}
% \lstset{language=Matlab,
%         frame=single, % Single frame around code
%         basicstyle=\scriptsize\ttfamily,
%         % keywordstyle=[1]\color{blue}\bf, % Perl functions bold and blue
%         keywordstyle=[3]\color{blue}\underbar, % Custom functions underlined and blue
%         identifierstyle=, % Nothing special about identifiers                                         
%         commentstyle=\usefont{T1}{pcr}{m}{sl}\color{green}\scriptsize, 
%             % Comments are in small dark green courier font
%         stringstyle=\color{red}, 
%         showstringspaces=false, % Don't put marks in string spaces
%         tabsize=4, % 5 spaces per tab
%         % 
%         % Put standard functions not included in the default language here
%         %morekeywords={rand},
%         % Put function parameters here
%         %morekeywords=[2]{on, off, interp},
%         % Put user defined functions here
%         %morekeywords=[3]{test},
%         %
%         morecomment=[l][\color{blue}]{...}, % Line continuation (...) like blue comment
%         % numbers=left, % Line numbers on left
%         % firstnumber=1, % Line numbers start with line 1
%         % numberstyle=\tiny\color{blue}, % Line numbers are blue and small
%         % stepnumber=5 % Line numbers go in steps of 5
% }

% Creates a new command to include an Matlab script, the first parameter is the
% filename of the script (without .pl), the second parameter is the caption
%\newcommand{\matlabscript}[2]{
%    \begin{itemize}
%    \item[]\lstinputlisting[caption=#2,label=#1]{#1}
%    \end{itemize}
%}

\input{colour-defs}
\input{newcommands-highlight-ignore-comments-annotations}
\input{newcommands-labels-refs}
\input{newcommands-eg-ie-etc}
\input{newcommands-for-bibtex} % BP, BPnom, IP, presenter, putDOI, DP, etc
\input{newcommands-misc}
\input{newcommands-squeeze-spaces--no-titlesec}
%\input{newcommands-squeeze-spaces}
\input{newcommands-math}
% \input newcommands-thm-env




==> bib/1-example-paper-templates/package-and-newcommand-includes.tex <==
%%%%%%%%%%%%%%%%%% PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%
\RequirePackage{times}
\RequirePackage[usenames]{pstcol} 
%\RequirePackage[usenames]{pstricks} 

% Graphics (figures/images etc.)
%\usepackage[pdftex]{graphicx}
\RequirePackage{graphicx} % supplies \includegraphics
\graphicspath{{./octave-figures/}{./results/}{./figures/}{./snapshots/}}
\DeclareGraphicsExtensions{.eps,.pdf,.jpeg,.png,.jpg}

\RequirePackage{rotating}
\RequirePackage{indentfirst} 
\RequirePackage{color} 
%\RequirePackage{picins} 
\RequirePackage{bmpsize} 
\RequirePackage{epsfig} % good old way of including figures
\RequirePackage{eepic} 
\RequirePackage{subfigure} % put figures side-by-side
%\RequirePackage{subfig} % apparently supercedes subfigure, but too many problems/differences with subfigure
%\RequirePackage{subcaption} % too many problems/differences with subfigure
\RequirePackage{wrapfig} % wrap text around figures
\RequirePackage{picinpar} % alternative to wrapfig, less useful

% Math (symbols/equations etc.)
\usepackage{cancel}
\RequirePackage{amsmath,amssymb,amsthm,amsbsy,amsfonts,dotlessj} 
\RequirePackage{latexsym}
\RequirePackage{mathptm} % - AG (Don't like \mathcal{C} that this produces
\RequirePackage{mathptmx} % times (smaller) math fonts, greek characters also italicized
\RequirePackage{bm} % boldmath
\DeclareMathVersion{bold} 


% Formatting
\RequirePackage{multicol}
\RequirePackage{esvect} % defines \vv{}
\RequirePackage{ifthen}
\RequirePackage{etoolbox}
\RequirePackage{relsize}
\RequirePackage{soul}   % Provides \hl{some-text}
%\RequirePackage{showlabels} 
\RequirePackage[final]{showkeys} 
%\RequirePackage[final,notref]{showkeys} 
\makeatletter
\newcommand{\vtiny}{\@setfontsize\vtiny{4}{5}}
\makeatother
\renewcommand*\showkeyslabelformat[1]{%
  \hbox{\parbox[t]{\marginparwidth}{\raggedright\normalfont\vtiny\ttfamily#1}}}
\newcommand{\fullrlap}[1]{%
  \rlap{\kern\dimexpr-\@totalleftmargin+\textwidth+\marginparsep\relax#1}}
\makeatletter
\patchcmd{\SK@@label}{\llap}{\fullrlap}{}{}% Insert appropriate (full)rlap patch
\patchcmd{\SK@@ref}{\footnotesize}{\vtiny}{}{}% reduce font size
\makeatother
%\RequirePackage[top=0.8cm,bottom=0.8cm,left=0.8cm,right=0.8cm,nohead,nofoot]{geometry}
%\RequirePackage[top=1.2cm,bottom=1.3cm,left=1.2cm,right=1.2cm,nohead,nofoot]{geometry}


\usepackage{tikz}
\usetikzlibrary{calc}
\usepackage[american,siunitx]{circuitikz}
\usepackage{pgfplots}

\usepackage[nolist,nohyperlinks]{acronym}
\RequirePackage{setspace}
\RequirePackage{moreverb}
\RequirePackage{ulem} % provides \uline
        \let\em=\it % ulem package redefines \em=\uline
\RequirePackage[sectionbib]{chapterbib}
\RequirePackage{fancyhdr}
\RequirePackage{array}
\RequirePackage{floatflt} % does (to some extent) work inside itemize environment %
                          % use \fltditem, see $LATEXDOCS/floatflt.pdf, esp. Sec 3.1
\RequirePackage{srcltx}
\RequirePackage{chemarrow}

% Utilities
\RequirePackage{todonotes}
\RequirePackage{tcolorbox}
\RequirePackage{fixme}
%\RequirePackage[footnotesize,bf,figurename=Fig.,hang]{caption}
\RequirePackage[footnotesize,bf,figurename=Fig.]{caption} % hang not great for small figures
%\usepackage[scriptsize,hang,bf]{caption}
%\RequirePackage[hypertex]{hyperref} 
\RequirePackage[implicit=false]{hyperref}  % implicit=false => href only (not figs/footnotes/citations/etc.)
%\RequirePackage[hidelinks]{hyperref} 
%\definecolor{linkColor}{rgb}{0.1,0.1,0.8}
%\usepackage[colorlinks=true,bookmarks,pdfpagemode=UseOutlines,linkcolor=linkColor,citecolor=linkColor,pagecolor=blue,urlcolor=blue,pdftitle={Verification, Learning, Control},pdfauthor={Jaijeet Roychowdhury},plainpages=false]{hyperref}
\hypersetup{ % get rid of annoying boxes, more muted links
    colorlinks,
    linkcolor={red!50!black},
    citecolor={blue!50!black},
    urlcolor={blue!80!black}
}


%\usepackage{./tweaklist} % allow changing of item spacings in standard itemize,
                         % enumerate, description environments
					     %%% tweaklist: compress lists. Also check out 
                         %%% \usepackage{mdwlist} (use itemize*, enumerate*, 
                         %%% description* with that)
                         % enumhook for the enumerate environment, itemhook for
                         % the itemize environment, and descripthook for the
                         % description environment.
                         % HOWEVER, CAUSES ERRORS. Use enumitem instead.

% enumitem package included from newcommands-squeeze-spaces.tex

\providecommand{\subparagraph}{} % needed for IEEEtran.cls (which does not define subparagraph); \providecommand checks if it is already defined
\RequirePackage[small,compact]{titlesec} % squeezing whitespace between section heading
\RequirePackage[square,sort&compress,numbers]{natbib} % needed for IEEEtran; but proposal.cls pulls it in automatically
%\RequirePackage{cite} % natbib doesn't like this
\RequirePackage{lipsum}
\RequirePackage{microtype}
\RequirePackage{url}
\RequirePackage{listings} % Required for insertion of code
\RequirePackage{multirow}
\RequirePackage{booktabs}
% load cleveref last, but before algorithm2e (which breaks cleveref)
\RequirePackage[compress,capitalise,noabbrev]{cleveref} % defines \cref, \Cref, etc; options are compress (don't sort), sort (don't compress), sort&compress (default), nosort (neither sort nor compress)
%\RequirePackage{algorithmic}
%\RequirePackage{algorithm}
%\RequirePackage[boxed,algoruled]{algorithm2e}
\RequirePackage[boxed,algoruled,linesnumbered,vlined,nofillcomment]{algorithm2e}
%\usepackage[yyyymmdd,hhmmss]{datetime} % use: Compiled on \today\ at \currenttime
\usepackage{datetime2} % ]use: Compiled on \DTMnow. And do \documentstyle[pacific]{...}

%%%%%%%%%%%%%%%%%% END PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%

% fixme package setup
\fxsetup{ status=draft,
		  %author={\tiny JR},
	  	  layout=footnote,
		  layout=inline, % also try footnote or pdfnote
		  theme=color,
	  	  marginclue
}
\definecolor{mydarkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{myred}{rgb}{0.9,0.0,0.0}
%\definecolor{fxnote}{rgb}{0.8000,0.0000,0.0000}
\renewcommand{\englishlistfixmename}{List of changes needed}
% Decrease spacing between items in bib
\newcommand{\BIBdecl}{\setlength{\itemsep}{0.25 em}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Multi-column the bib
%\patchcmd{\thebibliography}
%  {\list}
%  {\begin{multicols}{2}\list}
%    {}
%    {}
%\appto{\endthebibliography}{\end{multicols}}

%------------------------------------------------------------------------------
%   CODE INCLUSION CONFIGURATION
%------------------------------------------------------------------------------

\lstloadlanguages{Matlab}
\lstset{language=Matlab,
        frame=single, % Single frame around code
        basicstyle=\scriptsize\ttfamily,
        % keywordstyle=[1]\color{blue}\bf, % Perl functions bold and blue
        keywordstyle=[3]\color{blue}\underbar, % Custom functions underlined and blue
        identifierstyle=, % Nothing special about identifiers                                         
        commentstyle=\usefont{T1}{pcr}{m}{sl}\color{green}\scriptsize, 
            % Comments are in small dark green courier font
        stringstyle=\color{red}, 
        showstringspaces=false, % Don't put marks in string spaces
        tabsize=4, % 5 spaces per tab
        % 
        % Put standard functions not included in the default language here
        %morekeywords={rand},
        % Put function parameters here
        %morekeywords=[2]{on, off, interp},
        % Put user defined functions here
        %morekeywords=[3]{test},
        %
        morecomment=[l][\color{blue}]{...}, % Line continuation (...) like blue comment
        % numbers=left, % Line numbers on left
        % firstnumber=1, % Line numbers start with line 1
        % numberstyle=\tiny\color{blue}, % Line numbers are blue and small
        % stepnumber=5 % Line numbers go in steps of 5
}

% Creates a new command to include an Matlab script, the first parameter is the
% filename of the script (without .pl), the second parameter is the caption
\newcommand{\matlabscript}[2]{
    \begin{itemize}
    \item[]\lstinputlisting[caption=#2,label=#1]{#1}
    \end{itemize}
}

\input colour-defs
\input newcommands-highlight-ignore-comments-annotations
\input newcommands-labels-refs
\input newcommands-eg-ie-etc
\input newcommands-for-bibtex % BP, BPnom, IP, presenter, putDOI, DP, etc
\input newcommands-misc
\input newcommands-squeeze-spaces
\input newcommands-math
\input newcommands-thm-env


% vim: guifont=mono\ 11


==> bib/3-example-poster-template/Makefile <==
# File Descriptions
TOP = example-poster.tex
OTHERSRCS = package-includes.tex poster-format.tex \
		poster-colors.tex

PDFS = $(TOP:.tex=.pdf)

# Make Rules
all: pdfs
	- @echo "try make pdfs"

pdfs: $(TOP) $(OTHERSRCS)
	pdflatex $<

clean:
	rm -rf *.aux *.log *.nav *.out *.toc *.snm

pristine:
	rm -rf *.aux *.log *.nav *.out *.toc *.snm
	rm -rf *.pdf *.dvi


==> bib/3-example-poster-template/package-includes.tex <==
% Graphics(Pictures/Figures etc.)
% BASIC REQUIREMENTS
\RequirePackage{graphicx}
\usepackage{epstopdf}
\usepackage[justification=centering,bf]{caption}
\graphicspath{{./figures/}{./snapshots}}
\DeclareGraphicsExtensions{.pdf,.jpeg,.jpg,.png,.eps}

% SPLITTING FIGURES/FANCY STUFF
\RequirePackage{subfig}
\RequirePackage{wrapfig}
\RequirePackage{booktabs}
\usepackage[export]{adjustbox}  % Lets you align images to right/left in includegraphics. Use as \includegraphics[width=<whatever>,right]{filename}
                                

% Formatting (Placement/Alignment)

% Math (Equations/fonts etc)
\RequirePackage{amsmath}
\RequirePackage{mathtools}

% Drawing (Flow Charts are almost mandatory for a poster)
\RequirePackage{tikz}
\usetikzlibrary{shapes.geometric, arrows}


==> bib/3-example-poster-template/poster-colors.tex <==
% Defining the various colors used in the poster
\setbeamercolor{block title}{fg=ngreen,bg=white}
\setbeamercolor{block body}{fg=black,bg=white}
\setbeamercolor{block alerted title}{fg=white,bg=dblue!70}
\setbeamercolor{block alerted body}{fg=black,bg=dblue!10}


==> bib/3-example-poster-template/poster-format.tex <==
% Defining column widths, poster size and other stuff like that. This template has been designed for a 3 column layout. These columns can be merged at locations to accomodate bigger figures etc.
\usepackage{fp}	% This package is local to calculations for formatting
\newlength{\sepwid}
\newlength{\onecolwid}
\newlength{\onehalfcolwid}
\newlength{\twocolwid}
\newlength{\threecolwid}
\newlength{\fourcolwid}
\newlength{\twothirdpagewid}
\newlength{\onethirdpagewid}
\def\nCOLsFour{4.0}	% defined as FP because we will be using this is for calculations
\def\nCOLsThree{3.0}
\def\paperwidthVal{91.44}	% defined as FP because we will be using this is for calculations
\def\paperheightVal{121.92}
\setlength{\paperwidth}{\paperwidthVal cm}	% A0' width: 33.1 in
\setlength{\paperheight}{\paperheightVal cm}	%  A0' height: 46.8 in

\FPeval{\sepwidVal}{0.025*\paperwidthVal}
\setlength{\sepwid}{\sepwidVal cm}

% Calculating the values for columnwidths if the sepwid and nCOLs is given
\FPeval{\onecolwidVal}{(\paperwidthVal-(\nCOLsFour+1)*\sepwidVal)/\nCOLsFour}
\FPeval{\onehalfcolwidVal}{1.5*\onecolwidVal+0.5*\sepwidVal}
\FPeval{\twocolwidVal}{(2*\onecolwidVal)+\sepwidVal}
\FPeval{\threecolwidVal}{(3*\onecolwidVal)+(2*\sepwidVal)}
\FPeval{\fourcolwidVal}{(4*\onecolwidVal)+(3*\sepwidVal)}

\FPeval{\onethirdpagewidVal}{(\paperwidthVal-(\nCOLsThree+1)*\sepwidVal)/\nCOLsThree}
\FPeval{\twothirdpagewidVal}{(2*\onethirdpagewidVal+\sepwidVal)}  % Maintaining a consistent margin value

% Assigning the calculated widths to the defined length variables
\setlength{\onecolwid}{\onecolwidVal cm}
\setlength{\twocolwid}{\twocolwidVal cm}
\setlength{\threecolwid}{\threecolwidVal cm}
\setlength{\fourcolwid}{\fourcolwidVal cm}
\setlength{\onehalfcolwid}{\onehalfcolwidVal cm}
\setlength{\onethirdpagewid}{\onethirdpagewidVal cm}
\setlength{\twothirdpagewid}{\twothirdpagewidVal cm}

\setlength{\columnsep}{0cm}

% Custom newcommands for the poster (add margins etc.)
\newcommand{\addmargin}{\begin{column}{\sepwid}\end{column}}



==> bib/Makefile <==
TOP = test-bibs.tex
OTHERSRCS = 
SHELL=/bin/bash

DVIS = $(TOP:.tex=.dvi)
PDFS = $(TOP:.tex=.pdf)

%.dvi: %.tex *.bib test-*.tex
	@i=1; export TEXINPUTS=$(TEXINPUTS); while [[ $$i -le 3 ]] ; do \
		echo $$i; \
		((i=i+1)); \
		echo TEXINPUTS=./texinputs:./texinputs/EngC/:$(TEXINPUTS) latex $<; \
		TEXINPUTS=./texinputs:./texinputs/EngC/:$(TEXINPUTS) latex $<; \
		echo bibtex $(<:.tex=); \
		bibtex $(<:.tex=); \
		echo TEXINPUTS=./texinputs:./texinputs/EngC/:$(TEXINPUTS) latex $<; \
		TEXINPUTS=./texinputs:./texinputs/EngC/:$(TEXINPUTS) latex $<; \
	done
	- @ echo ""
	- @ echo "Check that latex shows NO undefined reference or other warnings above."
	- @ echo ""
	- @ echo "Now run xdvi $(<:.tex=) manually and check that it looks right."
	- @ echo ""

%.ps: %.dvi
	dvips -t letter -Ppdf -G0 -j0 -o $(<:.dvi=.ps) $<
	pkfix $(<:.dvi=.ps) $(<:.dvi=-pkfixed.ps)
	mv $(<:.dvi=-pkfixed.ps) $(<:.dvi=.ps)

%.pdf: %.ps
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.5 -dNOPAUSE -dQUIET -dBATCH \
	   -dPDFSETTINGS=/prepress -dCompressFonts=true -dSubsetFonts=true \
	   -dNOPLATFONTS -dSAFER -dMaxSubsetPct=100 -dEmbedAllFonts=true \
	   -sOutputFile=$(<:.ps=.pdf) -f $<
	# the above creates PDF v1.5 with all fonts embedded
	qpdf --check $(<:.ps=.pdf)
	# the above shows the PDF version and performs some basic checking
	pdffonts $(<:.ps=.pdf)
	# the above shows which fonts are used in the pdf file

#%.pdf: %.dvi
#	dvipdfm $<

###############


all: checkfiles
	-@echo "try make [dvis|pdfs|clean|pristine]"
	-@echo ""

dvis: $(DVIS)
	-@echo ""
	-@echo "$^ ready."
	-@echo ""

pdfs: $(PDFS)
	-@echo ""
	-@echo "$^ ready."
	-@echo ""

checkfiles: 
	@test -s jr.bib -a -s stringdefs.bib -a -s amahmutoglu.bib || { echo "error: jr.bib and/or stringdefs.bib \
	and/or amahmutoglu.bib doesn't exist.\n\
	\nCheck out the bib-SVN repository and make soft links to \n jr.bib \
	, stringdefs.bib and amahmutoglu.bib into this directory.\nExiting..."; exit 1; }

.PHONY: dvis all clean pristine pdfs checkfiles

clean:
	- rm -f *.dvi *.aux *.log *.toc *.lof *.loc *.lofb *.bbl *.blg *.dlog *.fff *.ttt *.lot *.brf *.tmp subject.idx authors.idx vect*.tfm *\~ *.out
	- rm -f *.ps
	- rm -f *_latexmk *.fls
	- rm -f *.synctex.gz

pristine: clean
	- rm -f $(PDFS)


==> bib/example-Makefile-adapt-this-for-your-paper <==
include Makefile.common # first target all is checkfiles
#
# YOU SHOULD NOT NEED TO CHANGE ANYTHING BELOW: CHANGE ONLY Makefile.common

helpmsg: 
	- @echo "try make [pdf|pdfs|clean|pristine|mrproper]"
	- @echo ""

%.pdf: %.tex $(OTHERSRCS) $(REQDSOFTLINKS)
	@i=1; export TEXINPUTS=$(TEXINPUTS); while [[ $$i -le 4 ]] ; do \
		echo $$i; \
		((i=i+1)); \
		echo TEXINPUTS=.:$(TEXINPUTS) pdflatex $<; \
		TEXINPUTS=.:$(TEXINPUTS) pdflatex $<; \
		BUFILES=bu*.aux; \
		for bufile in $$BUFILES; do \
			echo TEXINPUTS=.:$(TEXINPUTS) bibtex $$bufile; \
			TEXINPUTS=.:$(TEXINPUTS) bibtex $$bufile; \
		done; \
		echo TEXINPUTS=.:$(TEXINPUTS) bibtex $(<:.tex=); \
		TEXINPUTS=.:$(TEXINPUTS) bibtex $(<:.tex=); \
		echo TEXINPUTS=.:$(TEXINPUTS) pdflatex $<; \
		TEXINPUTS=.:$(TEXINPUTS) pdflatex $<; \
	done

pdf pdfs: $(PDFS)
	- @ echo ""
	- @ echo "$^ ready."
	- @ echo "Check that latex shows NO undefined reference or other warnings above."
	- @ echo "Now run xpdf/zathura $^ manually and check that it looks right."
	- @ echo ""

.PHONY: pdfs helpmsg


==> bib/test-PHLOGON-jr.tex <==
\cite{Berger:1996,
Slonczewski:1996,
Ventra:2004,
Fuchs:2005,
Huai:2005,
Krivorotov:2005,
Fuchs:2006,
Meng:2006,
Mistral:2006,
Slonczewski:2007,
Deac:2008,
Haney:2008,
Heiliger:2008,
Kubota:2008,
Sankey:2008,
Sun:2008,
Houss:2008,
Houss:2007,
Devolder:2007,
Salahuddin:2007,
Salahuddin:2006,
Salahuddin:PRB_2006,
Salahuddin:arxiv_2009,
Salahuddin:NL_2008,
Lines,
Ramesh:2010,
Weiler:2009,
Hu:2009,
Salahuddin:IEDM_2008,
Wigington:1959:ProcIRE,
ManleyRowe:1956,
Rowe:1958,
Mitchell:1968:IEEEtransComputers,
Elowitz:2000,
Nethercot:1960:STS:1661226.1661229,
FeuerEtAl:1983,
Keyes:1970:MED:1662935.1662942,
Landauer:1961:IBMJRD,
Landauer:1998:Nature,
Shenker:pittphilsci115,
LandauersPrincipleWikipedia,
UFLreversibleComputingWebpage,
DeGrootSpinTorquePictureWebpage,
Norton:pittphilsci1729,
Vitanyi:2005:TSE:1062261.1062335,
JRvonNeumannUsingOscillators,
JRhierarchicalPPVabstraction,
Goto:DCfluxParametron:1986,
Goto:QuantumFluxParametron:1991,
Slavin:2009,
Izhikevich:2000:SIAM,
Malkin:1956,
Malkin:1949,
Salahuddin:2006:arXiv,
SBMLspec:2010,
Huygens:1672,
Strogatz:Stewart:ScientficAmerican:1993,
Gray:1994,
Belousov:1985:reprint,
Zaikin:Zhabotinsky:1970:Nature,
Goto:1954,
Goto:1955,
Oshima:1955,
OshimaEtAl:1955,
Takahashi:1956,
Muroga:Parametron:1958,
ParametronThocpWebpage,
ParametronWikiPedia,
Deen:2003,
Farzeen:2010,
Cilek:2008,
PufallEtAl:2006:PhysRevLett.97.087206,
RippardEtAl:2005:STNO_IL:PhysRevLett.95.067203,
Pufall:2005:STNO_FM:2005ApPhL..86h2506P,
KakaEtAl:STNO_Mutual_Locking:2005Natur.437..389K,
Bourianoff:AlternativeLogic:Computer:2008,
Hosomi:IEDM:2005,
TsukamotoEtAl:IRPS:2010,
Toh:Tsukamoto:EtAl:IEDM:2009,
Grindrod:1996,
Angluin:1987:LRS:36888.36889,
Shahbaz:2009:IMM:1693345.1693363,
Yokomori93learningnon-deterministic,
Bollig:2009:ALN:1661445.1661605,
Angluin:1977:FPA:800105.803393,
TanHe:2007:MORbook,
Celik:Pileggi:Odabasioglu:2002:InterconnecAnalysisBook,
Abramovitch2002ACC,
KimEtAlJSSC1999,
GostiEtAl:1998:ExactInputEncodingFSMs,
OkabeEtAl:2000:SpatialTesselationsVoronoiDiagrams,
GoTaWeBl1983Lasers,
GrRoJComputPhy1987FastParticleSim,
OzNeAlRFIC2006freqdoubler,
RaLeYaISSCC1994CMOSfreqDivider,
Wernick1942LogicallyComplete,
RoskaEtAlOscillatoryCNNassociativeMemory2012,
ThSoQuestForNextSwitchPROCIEEE2010,
WaRoUCNC2014PHLOGON,
ZeEtAl2013ultralowpowerSTNOs,
RoCoupledOscHierPPVsArXiv2011,
RoCoupledOscHierPPVsArXiv2012,
RoPHLOGONarXiVv12014
}


==> bib/test-ag.tex <==
\cite{
coughran1983cazm,
rofougaran1988accurate,
shima1983table,
amsallem2011modspec,
WaAaWuYaRoCICC2015MAPP,
barby1988polynomial,
de1978practical,
hugger2007institute,
li2015mos,
kanj2011accelerated
}


==> bib/test-gcj.tex <==
\cite{
GuRoASPDAC2008,
GuRoASPDACTWENTYELEVENDAETOFSM,
GuRo2010probabilisticHypervolumes,
GuRoASPDAC2010,
GuRoICCAD2010genPPV,
DeGuRoICCAD2010qpPPV,
GuRoICCAD2008maniMOR,
GuICCAD2009qlmor
}


==> bib/test-jr-bib-entries.tex <==
\cite{
MAPPwebsite,
deutsch1,
djordjevic3,
djordjevic2,
ho1,
GrSwLaJeFrMaetal2001,
slmw93,
nayak1,
hwang1,
seki1,
bjorck,
megretski97guide,
DeLoRoICCAD2000,
Ho1998,
JaMoBa,
Abidi1983,
AcBoPeFeSpKuramotoReview,
AcBo1997,
AcBoSp2000,
oea1,
Adler1973,
Adler46,
Ahn00,
AlBoFrHe96,
allgowergeorg,
AminMenezesEtcDAC2005,
ApCoTrProcIEEE1972,
Aprille72p,
ArGR99,
arambepola1,
Armand,
Arnold74,
ArBlPiDAC2001,
Ascher1998,
assadourian1,
SET1,
DahlquistBjorckNumericalMethods,
SET2,
TuTCAD04,
bwmcetc,
BaFeFrICCAD98,
BaBiCh92,
BaZhBi89,
BaZhBi88,
MeyerTsividisMihaiVenu96,
BaCeSPAWC05,
barbeau1,
bellman1,
Be2000,
BogoMitroOscillatorBook,
BoMeRoICCAD2005,
Bo94,
Bole94,
BoGuGh2002,
BoGuGhPi2001,
BrLaLaMeFe2002,
brachtendorf98a,
BrWeLa97a,
brachtendorf96,
bracken1,
Brambilla2003,
Brayton1979,
Brennan1996,
brenner1,
BrHuSeBook,
BruntCS97,
Buck76,
AmDaIsICCAD05,
NgCICC04,
CaPe97,
CeCaTCAD97,
BakerEtAlPade,
GolubVanLoadMatrixComputations,
CurtainZwartIntroInfDimLinSystTh,
CeCaMTT96,
chanho89,
chang3,
chang2,
chang1,
Chang97,
ly:Charbon92,
ChLi97,
ChKiKeutzerICCAD2000,
chiprout,
chisholm1,
ChWh94,
UmakantaMasters,
choudhury1,
ChBa99,
chualin,
ChuaRoska,
rick12,
ChUs81,
chua76a,
Chua92,
ChLi75,
Chua88-1,
Chua88-2,
clark1,
cong93a,
ConnEtcDAC99,
CoramTCAS2001,
cory1,
Costantini02,
cottrell1,
Crank,
CrWoDAC03,
TIswra029,
CaTaShMcPNAS04,
sharrit96,
DaGiSa2002,
davidson1,
Toth97,
deCarlo,
delves1,
DeICCAD98a,
Demir98,
demir94memo,
demir96,
Demir94,
Long00,
DeMeRoTCAS2000,
FiNiPe2008,
DeIJCTA2000,
DeMeRoCICC98,
DeMeRoDAC98,
TR97-1,
mpdeforvcos,
Demir03,
DeRoTCAD2003,
DeRoNTVPdraft98,
orthphase,
Deml1997,
DevganKashyapICCAD2003,
DPBV98,
DiRo69,
djordjevic1,
doetsch1,
ChuaUniversal,
dommel1,
DoRoTCADPWP2008,
DoRoDAC2005,
DoRoDAC2003PWP,
doob,
grigoriu,
giancoli,
middleton,
petrovic2005,
dragone68,
ElLiICCAD97,
cazm1,
Espana96,
EsGiPoSrICASSP2001,
DaMePiTCAD96,
TIperscomms2001,
FaTsWi83a,
Farkas94,
FeFrICCAD97,
FeFrNoiseTM97,
FeFr95a,
FeFr95b,
Feldmann95,
FeMeLo96,
FeRo96a,
fishburn94a,
Fitz92,
fodor1,
foschini,
FrVoMaGi2002,
Freidlin,
FrDAC99,
Freund98c,
freund98a,
FrFeICCAD96,
FrFeICCAD95,
freund91,
Freund94a,
Freund91b,
GaGrVa1994,
GaKuSrSenSys03,
gao1,
Gardiner83,
GardnerPLL,
GardnerRP,
gear1,
Gear1971,
Gear1981,
gertzberg1,
ghme96,
rhme95,
ghausi1,
ghoshal1,
GiSaSymbolicBook,
gilmore91,
goldberg1,
gopal1,
gordon1,
Gottlieb97,
GoUlZhRuGuMu1998,
Gourary2000,
GrayMeyer,
mikegreen,
grimmethesis,
Grimmet92,
Grimshaw,
gruodis1,
gruodis2,
xerox-sun-lsi,
gupta1,
Haaken87,
Hafner66,
Hajimiri97,
hasegawa1,
Hayashi64,
HBDE00,
heinen91,
herskowitz1,
Hess68,
hilbert1,
HoYaTrEp1985,
hoffmankunze,
HongScaglioneJSAC2005,
HoSiRuCa2002,
Hoppensteadt,
HorowitzHill,
HuGaMa03,
huang1,
Huh011,
hull93,
RoISCCSP04,
RoVLSI04,
WaGhVrICCAD04,
GhLiRoASPDAC2004,
JaTAC97,
IBMperscomms2000,
Johns1997,
JoMa96,
johnson1,
scipy,
blodgett1,
JuNeMe2002,
Kaertner1989,
KaTtWh94,
KaWaWhTCASII2000,
KaLoRo96,
nchip1,
KashyapPersComm06,
KaTa97,
katzenelson,
KeWeYa1995,
kerr79,
BioPattern2,
Kevorkian90,
KevorkianCole81,
Kevrekidis2007,
TPL1,
Kimura64,
kinget,
Melville02,
Kish2002,
nanobox-02,
nanobox-03,
Kobayashi80,
BioPattern1,
KoYuCrCrCh2002,
krage1,
kreyszig1,
KundertPLL,
Kundert95,
sparsemanual,
Kundert86,
Kundert1988,
kundertwhite,
kundert89,
KuWhSaICCAD88,
kundert-pers-comm,
kundert3,
kundert1,
kundert2,
kuo1,
Kuramoto2003,
Kuramoto84,
Kuramoto89,
Kurokawa1973,
kurokawa1968,
Kaertner90,
ljiljana,
hompack,
WuJiBlCICC2000,
quantic1,
LaTr99,
LaRoICCAD2006TPPPV,
LaRoDAC2006MultiLevelPPV,
LaRoASPDAC06krylov,
MaRuTCAD2008,
LaRoASPDAC06nano,
LaRoCICC2005,
LaRoMTTS2005,
LaRoCICC2004,
LaRoICCAD04,
LaRoICCAD2004,
LaRoMTT2004,
LaWaRoASPDAC2005,
LaTsWo2004,
lax,
rickSelf,
lean1,
LeeZoBlaauwDAC2004,
lee1,
Lee03,
Lee2003,
Leeson66,
lelarasmee1,
LeLPTVTM97,
Li89,
LiWhICCAD99,
LiPiDAC2003,
nanoworkshop-02,
Lin00-2,
Lin00,
Li2000,
LiKu92,
lin1,
lindell1,
liu1,
LiKiAPS2003,
LoMeCICC97,
Lo63,
luke2,
luke1,
ChAlASPDAC05one,
ChAlASPDAC05two,
Livio2003,
Grattarola77,
MaTrMa2002,
maas,
Huh01,
MaReHuFeZh2003,
Mar99,
marino1,
rosch92b,
marx2,
marx1,
Maxim01,
mayaram1,
MaLeMoRiRo2000,
colin,
mcknight1,
McNeill94,
MehrotraPLL02,
MeRoNEWCAS2005,
MeRoCICC2006,
MeRoICCAD2006PPVHB,
MeRoDATE2006LSENV,
MeRoDAC2006LSENV,
MeRoICCAD2005MPCENV,
MeRoICCAD2005ssGeMPDE,
MeRoTCAD2007ssGeMPDE,
MeRoEtAlTCAD2005,
MeRoEtAlDAC2004,
Phinest,
melville2,
melville94a,
MeFeRo95,
melville93,
Me94,
Mickens95,
MCCS96,
Mink86,
Moyer00,
Murdock91,
Ja2000,
DoRoCICC2004,
nabors1,
advice1,
Nagel1975,
nakhla76,
NaRoTCASwampde,
Narayan,
NaRoDAC99,
NaRoWampdeTM98,
narayanan1,
NayfehBalachandran95,
copasi1,
NayfehMook79,
neug1,
NgWoLe99,
NgGaRo88,
NgLaMTTS96,
Ngoya,
Novof95,
rutenbarbook,
OdCePiTCAD98,
OdCePiICCAD97,
Kiehl96,
Ohta68,
ohtsuki,
Okumura97,
Okumura1993,
ortegarheinboldt,
OsPers98,
OtChRaISSCC2005,
Otis2005,
GoLaRoASPDAC2006,
LiAcICCD05,
LiLiLiPiNaDATE05,
palusinski1,
pan1,
Panfilov,
PapoulisSA,
papoulis,
ParkerChua89,
PaCh87,
PaOg95,
Parzen83,
dop1,
Petzold1981,
dassl,
PhDAC2000,
PhTCAD2003,
PhSiPMTBRDATE2004,
HotellingPOD1993,
BeHoLuPODfluidmech1993,
NoorNonlinearMOR1981,
RaPePODNewLook2003,
HeKrNonlinearControllabilityObservability1977,
ScherpenNonlinearBalancingSystControlLet1993,
PhPers99,
jrppvt,
PhICCAD98,
PhDaSiDAC2002,
BoDaICCAD2007,
JoSiTransAutCont1983,
DePaTransAutCont1984,
JoelJosephson,
PiChBrISCAS2001,
pillage1,
vanderPol22,
VanDerPol27,
PVCC01,
catastrophe,
numericalrecipes,
Brusselator,
pucel1,
Pulch2002,
QiSe1996,
quarles1,
Quarles1989,
quarles2,
rick6,
RabaeyPicoRadio2000,
Radparvar85,
Raghavan91,
rajput1,
ramo1,
rantzer94system,
Razavi03,
RazaviCICC95,
reinhardt1,
ReWhTCAD2003,
TiRuICCAD2006,
TiRuDAC2005,
ReWhICCAD2001TPWL,
rice44,
Risken89,
rizzoli94,
rizzoli88,
RoCaMonteCarlo,
robins,
almupvt,
Rohde97,
Rohde83,
rohrer71,
romeo1,
CNNbook,
RO97-hsnotes,
RoIMA97,
RoVLSID05,
Roychowdhury05,
Roychowdhury04,
SrRoTCAS2007,
RoICCAD2002Fenv,
RoICCAD2002opensrc,
RoISCAS2002,
Roychowdhury2002,
Ro2001BookChap1,
RoTCAS2001,
Roychowdhury2001,
RoTVPASPDAC99,
RoTVPTCAS99,
Royc99,
NaRoWaMPDEnotes98,
RoCICC98,
RoTcas97sub,
RoTVPICCAD98,
RoTVPNotes98,
RoTVPTM98,
RoWamSSNoisedraft98,
RoWamTVPdraft98,
Ro97tm1,
RoDac97,
RoTVPNotes97,
Royc97,
TR97-3,
multitoneinprep96,
RoMCMC95,
roychowdhury-disto,
RoFe97a,
RoychFeld-internal,
ROcicc97sub,
RoLoFeJSSC98,
RoMeTCAD2006,
RoMeDAC96,
docinprep,
roychowdhury-tcad92,
roychowdhury4,
roychowdhury5,
RoNePe94,
roychowdhury-dac92,
roychowdhury-eurodac92,
roychowdhury-iccad91,
roychowdhury-tcad92-2,
roychowdhury3,
roychowdhury1,
roychowdhury-dac91,
rubin1,
ruehli-pers-comm,
ruehli1,
ruehli2,
RughNonlin,
Runge76,
Rutledge90,
rosch92a,
DaDoRoASPDACZEROSEVENADME,
NassifCICC2001,
SrRoDACZEROSEVEN,
SrRoDATEZEROSEVENlatchsetup,
TaShASPDac2003,
TaShTCAD2003,
rick15,
Saad,
sainati1,
Saito88,
sakurai1,
sanicolinperscom,
SaSu02,
sard42,
schendel,
Schetzen,
Schiek05,
schneider1,
ScWoTuUsBaRo2000,
schuttaine1,
schuttaine3,
schuttaine2,
FATE,
semlyen1,
Seydel,
Sh96,
ShBlGrCaPhysRev84,
ShKi00,
ShTa2000,
Siegman86,
SiKaElWh1996,
Silveira1991,
silvester1,
singhal1,
singhal2,
Skelboe1980,
skelboe82,
SRIreportOnNSFsupportOfEDA,
SrLaRoCICC2006,
svru94,
stasinski1,
Stensby,
Stephan87,
Stover,
Strogatz00,
Likharev04,
strutt46,
Surette,
sussfort1,
SynopsysCCSwp05,
MeRoCoHuDa2005,
NiLaHo2004,
stromsignell77,
rick18,
rick19,
Kundert,
tang2,
tang1,
Asymp1,
telichevesky96,
telichevesky95,
thornber1,
TrFuSa98,
tricomi1,
TsividisPersComm2005,
tsividis,
Turing52,
tzuang1,
ChViCICC90,
ChViISCAS90,
Ueberhuber,
UsCh84,
ChSaDAC96,
rick17,
rickVPR,
Vanassche03,
VaGiSa2002,
Vanassche00,
vandenberghe,
Vannicola,
Vendelin82,
veaw96,
usarmy,
vlach1,
volterra1,
LaWaRoCICC2005,
WanRoDAC2005,
wang2,
wang1,
WaRoCICC2007,
WaLaRoDAC2007PVPPV,
webster1,
WeeksEtAlASTAP1973,
weeks1,
Weigandt94,
WeinerSpina,
wheeler1,
White1991,
white1,
Wiener61,
Wiener58,
WikipediaSPICEentry,
ngspice,
Winfree67,
wing1,
wlodarczyk1,
WoSa96,
WolframNewKind,
WolframCNN,
WoRo2003,
TheGoldenMean,
Wu00,
LiLeGoPiICCAD04,
LaRoInPrepFeb2005,
WaLaRoCICC2005,
yamamura,
Kiehl01,
yen1,
WaMuRoDATE04,
WaMuRoTCAD2005,
TiGuPhPiZlfSPICE2009,
WaMuRoISCAS2004,
XiuPapaEtcISPD2005,
Z.2000,
zadeh1,
ZeCh,
ZhChLaRAWCON2000,
vanderziel,
abramowitz1,
SPECTREuserguide,
SPICEhomepage,
ITRS2005,
SRCneedsLogicPhysical2005,
SRCneedsLogicPhysical2002,
ITRS2001,
ITRSms2001,
NSFsrcNIST2001,
Semi01,
ZhZhSIAMreview2009,
WaDoYeastSignallingSCIENCE2004,
ThEn2005,
KoKlYeastPheromoneModel2004,
lle,
riemannian1,
thinkglobally,
LTSA,
isomap,
Mammalian1,
Mammalian2,
Drosophila1,
Ueda_coupling,
formalbio,
molecularloops,
biowiki,
cirwiki,
melanopsinwiki,
melatoninwiki,
touitou,
syncbiowiki,
allpubs,
Hajimiri98,
circrhythm,
UedaSB30,
transcriptionwiki,
translationwiki,
phosphowiki,
Kuramoto,
Strogatz,
Coupled,
SinusoidalLight,
SCNsyncModel,
SCNspatiotemporal,
CircadianAndAddiction,
CircadianAndObesity,
CircadianAndHeart,
SchiblerCircadianEpilepsy,
ASPSNatureMed,
DSPS,
non24,
HalbergDiurnalMice1950,
PetzoldCircadian,
SCNinfluenceOnBody,
ipRGCs,
SchiblerCircadianLiver,
IshidaCircadianCancer,
phylliszeeNSMC2007talk,
AgRoPSB2008,
NaRoJSSC71CANCER,
InceODEs,
SastryNonlinearSystems,
KEGGdatabasePaper,
NetPathPaper2010,
TRANSPATHpaper2006,
PIDpaper2009,
MetaCycBioCycPaper2008,
ReactomePaper2011,
PathCasePaper2008,
ExPASyPaper2003,
ShanbhagEtalDesignAndTest2008,
BhSrLaRoICCAD2008,
IzhikevichLargeScale,
IBMcatCortexSimulation2009,
RoNOWmonograph2009,
Izhikevich2006,
KramerSzeriEtalSyncMeasures2007,
KramerSzeriEtalCorticalSeizurePropagation2007,
KramerKirschSzeriEpilepticPatternFormation2005,
CadieuKoepsellPhaseCouplingEstimation2009,
StrogatzSync2003,
HodgkinHuxley1952,
BhRoASPDAC2009,
BaRoDoBaAICHEjournal2011,
BSIMwebsite,
IBISwebsite,
VeRaLe03,
NeRoDATE2012SHIL,
MeRoDAC2012BLAST,
Ladd86,
Vemulapalli93,
wikipediaSCpage,
Klipp06,
Yi03,
Dohlman04,
Gillespie76,
Arkin97,
Freund98,
PRIMA97,
Saad96,
Ty05,
Kofahl04,
Clark89,
AldridgeEtAl2006, 
KlamtEtAl2006,
KlamtEtAl2007, 
SaezRodriguez2009Discrete,
PieroniProteinNetworking2008,
KrishnamurthyChungProcIEEE2007MD,
BSIMv3TechReport,
KamEtAlnondeterministicFSMs,
Bryant1986BDDs,
MaDeRoICCADTWENTYTHIRTEENGILLESPIENOISE
}


==> bib/test-tianshi.tex <==
\cite{
MO1965mooreslaw,
lyapunov1992general,
hisamoto2000finfet,
weinstein2010RBT,
Simpson2011interfacialPCM,
Wolf2006spintronics,
BehinDatta2010allSpinLogic,
Wolf2001spintronics,
Esmaeilzadeh2011darkSilicon,
Wilson2013ITRS,
Arsenault2012opticalComputing,
Caulfield2010opticalComputing,
Deng2007carbonNanotube,
Maass2002neural,
Patil2007misalignedCNT,
Singh2007heterogeneous,
Liu2000dnaComputing,
Goto1960patent,
Shulaker2013CNTcomputer,
Novoselov2012graphene,
Borghetti2010memristive,
Esmaeilzadeh2013power,
Mahboob2008bit,
Freeman2008nems,
vonNeumann:1954:NLC:nonote,
BhRoCON2011,
pederson1994SPICE3F5,
paydavosiBSIM4v4,
ashar1989SSPICE,
watson1987HOMPACK,
davis2006gnucap,
brinson2009qucs,
keiter2014xyce,
nenzi2014ngspice,
amsallem2011modspec,
nanohub2014MVS,
vladimirescu1994spice,
petermann1991laser,
kononov2013opticalVA,
joachim2013molecular,
touati2014advanced,
sze2006physics,
agarwal2014bsim6,
tudelft2014PSP,
GeofferyMOS11,
li2010PSP,
lemaitre2002adms,
coram2004VA,
lemaitre2003extensions,
WaAaWuYaRoCICC2015MAPP,
WaRoDAC2015MAPPforPHLOGON,
tiebout2004cmos,
kinget2002injection,
kratyuk2005analysis,
razavi1996phasenoise,
ohira2005Qdef,
randall2001Qdef,
deng2013CVCO,
vannerson1974RCosc,
chua1971memristor,
chua1976memristor,
lin2012IEDM,
WaRo2013VAnanoHUB,
mcandrew2015VA,
UMich2011RRAM,
Stanford2014RRAMverilog,
Stanford2012RRAMspice,
ASU2015RRAMverilog,
yakopcic2013memristor,
mcpherson2003thermochemical,
yu2012neuromorphic,
yakopcic2014memristor,
kvatinsky2011memristor,
kvatinsky2013team,
meuffels2012RRAMnotMemristor,
di2013RRAMnotMemristor,
slipko2013RRAMnotMemristor,
li2015RRAM,
Hoppensteadt2000pattern,
Hoppensteadt2000synchronization,
Hoppensteadt2004oscillatory,
Hoppensteadt2011anisotropic,
Hoppensteadt2011spin,
Hoppensteadt2013spin,
Hoppensteadt2014STO,
Hoppensteadt2015STO,
Porod2012STOassociative,
Porod2013STOnonBoolean,
Nikonov2015coupled,
Porod2015nonBoolean,
Porod2012associativeCNN,
Porod2015physical,
Roy2013beyond,
Roy2014brain,
Roy2014nonBoolean,
Roy2013associativeCrossbar,
Roy2015DPSTO,
SumanDatta2014neuro,
maffezzoni2015hys,
maffezzoni2015VO2osc,
maffezzoni2015coupledLCosc,
maffezzoni2015oscArray,
Pileggi2015RRAMONN,
Pileggi2015ONNRRAM,
Pileggi2015RRAM1T1Rosc,
Wang2015ONNPPV,
hopfield1982,
wang2004CNNvsLEGION,
wang2002dynamically,
Nikonov2012cmos,
Nikonov2012nonBoolean,
chua2011memristor,
keiter2015xyce,
xu2014twoMemristors,
wong2012RRAM,
kund2005CBRAM,
tehrani1999MRAM,
pickett2009TiO2,
kvatinsky2015VTEAM,
Wa2016MAPPhandson,
Wa2016MAPPmultiphysics,
WaKaRo2015MAPPvmc,
WaKaRo2015highQ,
WaKaWuRo2015MAPPnemo,
WaRo2015MAPPhandson,
RoWa2015PHLOGONneeds,
RoWa2015NEEDSgrc,
Wa2015BEARS,
Wa2015TGIF,
RoWa2014MOSAK,
Wa2014ModSpecNEEDS,
Wa2014XMIneeds,
Wa2014MVSneeds,
RoWa2013NEEDSteleseminar,
RoWa2013PurdueWorkshop,
WaKaWuRo2015MAPPposter,
YaStSt2013MemristorComputing,
AlZaSt2013NNcrossbar,
ShChLi2009fastRRAM,
ShFaAiRo2014nonBooleanRRAM,
StSnDuWi2008memristorFound,
JoChLu2010memsynapse,
LiRoKuWa2010complementary,
thakoor1990solid,
buot1994binary,
erokhin2008memristor,
JoLu2009crossbar,
samsung2009crossbar,
vourkas2015memristor,
pinaki2012memristor,
zhu2002sugar,
sheu1987bsim,
semiconductor2015itrs,
schiek2012Xyceneuron,
liu2012river,
VALRM24,
camsari2015spinlib,
rudolph2004uniqueness,
williams1995magnetics,
zhou2005modeling,
ida2012physically,
kundert2003hidden,
fitzpatrick2007analog,
wang2016well,
zhou2007modeling,
li2006compact,
diaz1992new,
mertens2013physics,
wei2011convergence,
jiao2006robust,
juliano2001novel,
stoner1948mechanism,
tannous2008stoner,
WaRo2016multiphysics,
semenov2008esd,
maehara2014highQstno,
makkar2005friction,
lee2016bloch,
festa2002randomized,
lucas2013ising,
gu2012encoding,
bian2014discrete,
marandi2014network,
sutton2017intrinsic,
mahboob2016electromechanical,
tsakmakidis2017QfactorScience,
WaRoOscIsing2017,
BMMwebsite,
metronomewebsite,
pantaleone2002metronome,
jia2015triplet,
inagaki2016ScienceIsing2000,
mcmahon2016ScienceIsing100,
camsari2017pbits,
yamaoka2016IsingCMOS,
kim1997multistability,
hoppensteadt2012weakly,
ising1925beitrag,
metropolis1953equation,
kadowaki1998quantum,
bian2014Ising,
johnson2011quantum,
harris2010flux,
ronnow2014defining,
denchev2016tunneling,
acebron2005kuramoto,
smale1961gradient,
yuan2010lyapunov,
landau1969statistical,
jadbabaie2004kuramoto,
wang2013expsync,
dorfler2014synchronization,
patra2016lyapunov,
coletta2017finite,
chung2001diameter,
karp1972np,
chen2011RTWO,
Wa2017arXivMetronomes,
bank2006harmonic,
vidal2001describing,
vander1968multiple,
verhoeven2010structured,
van2001structured,
miri2010design,
nguyen1999integrated,
nguyen1995micromechanical,
danino2010synchronized,
rosenblum2003synchronization,
dixit2012spintronic,
villard2010ghz,
finocchio2013nanoscale,
rappaport1996wireless,
best2007PLL,
Wa2017ESD,
gizynski2017chemical,
zhou2007esd,
monnereau2011behavioral,
mertens2013physics,
juliano2001novel
}


==> bib/test-verification-and-hybrid-systems-jr.tex <==
\cite{
Ghosh99,
Hanna94,
Hanna00,
Kurshan91,
Hartong02,
Steinhorst08,
Gupta04,
Alur00Discrete,
hytech,
Alur93,
Nerode93,
Alur95,
Henzinger96,
Sammane07,
Sammane072,
ddt,
ddttool,
Ray10,
Checkmate,
checkmateClarke,
Phaver,
Little07,
Little06,
Little08,
Batchu10,
Zonotopes10,
Support09,
HRDs05,
LiPLL10,
HWMCC11,
Stabilization,
VillaEtAlbook,
PartitionedFSMs,
AIGrewriting,
SeqSimulation,
FrehseLGDCRLRGDM11,
MitchellHSCC2011,
DBLP:conf/hybrid/2011,
MitchellHSCC2007,
DBLP:conf/hybrid/2007,
TomlinEtAlProcIEEE2003,
Kevin98timedpetri,
TizianoBook,
QBFBMC,
QBFFault,
QBFProg,
QBFSolving,
QBFGame,
kronos97,
uppaal,
botchkarev2000verification,
hybridsal,
Frehse2008,
Frehse2011,
Benvenuti2008ifac,
hsolver,
Platzer2008,
gaio,
cosy,
mitchell03,
KearnsVaziraniBook1994,
RivestSchapire1993DFAlearning,
BiermannFeldman1972,
OncinaGarcia1992,
BolligEtAl2009NLstar,
DenisLemayTerlutte2004DeLeTe2,
VidalEtAl2005probabilisticFSMs1,
VidalEtAl2005probabilisticFSMs2,
RonSingerTishby1996LearningProbabilisticAutomata,
Thollard00probabilisticdfa,
CarrascoOncina99stochasticinference,
seshia-thesis05,
Barrett:SMT09,
Seshia:ICCAD08,
Seshia:ICAC07,
bryant-tacas07,
solar2006combinatorial,
solar2007stencils,
henzinger-icalp03,
frehse-hscc08,
Kress-Gazit-icra07,
fainekos-hscc07,
clarke-cav00,
clarke-00,
tiwari-fmsd08,
donze-hscc07,
cook-vmcai09,
gulwani-cav08,
pnueli-focs77,
biere-bmc03,
sturton-ccs09,
seshia-acmtecs10,
jha-icse10,
jha-cps10,
li-dac10,
leeseshia-book11,
pappas-CDC96,
nuzzo-fmcad10,
jha-cav09,
beaver-www,
seshia-date07,
kupferman-fmcad08,
jha-formats07,
DBLP:journals/fmsd/PlatzerC09,
kl-thesis99,
abc-citation,
clarke-11,
alur-tcs95,
henzinger-ieeetac98,
live1,
live2,
game1,
game2,
girard-hscc06,
agrawal-hscc06,
agrawal-hscc05,
agrawal-hscc04,
cousot-popl77,
giannakopoulou-fmsd08,
chen-cav10,
kurshan-tcad91,
lafferriere-hscc99,
krogh-hscc03,
frehse-hscc05,
dang-fmcad04,
gupta-iccad04,
hartong-cav02,
frehse-date06,
walter-tcad08,
little-atva07,
Kurzhanski-hscc00,
Botchkarev-hscc00,
gao-fmcad10,
platzer-fmsd09,
BrMiCAVABC2010,
IntelAMSworkshop2010,
Chebotarev1997,
Mi2000,
BVSRCMVSIS,
BVSRCBALM,
BVSRCABC,
SoLeTaBoSaSe2006,
DawsonDigitallyAssistedRF2010,
guernic-cav09,
girard-hscc06a,
tomlin-procieee03,
FrKrRuDATE2006oscVerification,
AlYaRaLiKrPiICCAD2011PLLverification,
WalterPhD2007symbolicModelCheckingForAMS,
LiSeWaMyYoICCAD2006PetriNetsForAMS,
alur-procieee00
}


==> bib/test-von-Neumann-jr.tex <==
\cite{
vonNeumann:1922:LNG,
vonNeumann:1923:ETZ,
vonNeumann:1925:AM,
vonNeumann:1925:ESS,
vonNeumann:1926:PTI,
vonNeumann:1926:XXX,
vonNeumann:1927:GQG,
vonNeumann:1927:HB,
vonNeumann:1927:MBQ,
vonNeumann:1927:TDK,
vonNeumann:1927:TQG,
vonNeumann:1927:WAQ,
vonNeumann:1928:AES,
vonNeumann:1928:AMG,
vonNeumann:1928:DDT,
vonNeumann:1928:EBD,
vonNeumann:1928:EEEa,
vonNeumann:1928:EEEb,
vonNeumann:1928:EEEc,
vonNeumann:1928:ESF,
vonNeumann:1928:SAU,
vonNeumann:1928:TGG,
vonNeumann:1928:TJF,
vonNeumann:1928:ZIA,
vonNeumann:1929:AEG,
vonNeumann:1929:AEH,
vonNeumann:1929:AFT,
vonNeumann:1929:ATM,
vonNeumann:1929:BET,
vonNeumann:1929:BMS,
vonNeumann:1929:MDE,
vonNeumann:1929:TUM,
vonNeumann:1929:VEA,
vonNeumann:1929:WAM,
vonNeumann:1929:ZAA,
vonNeumann:1930:HVG,
vonNeumann:1931:ARS,
vonNeumann:1931:BAH,
vonNeumann:1931:ESO,
vonNeumann:1931:FFG,
vonNeumann:1931:FGM,
Koopman:1932:DSC,
vonNeumann:1932:AF,
vonNeumann:1932:AFG,
vonNeumann:1932:ESM,
vonNeumann:1932:MGQ,
vonNeumann:1932:OKM,
vonNeumann:1932:PAE,
vonNeumann:1932:PQE,
vonNeumann:1932:SHM,
vonNeumann:1932:ZAO,
Neumann:1933:BGK,
vonNeumann:1933:EAP,
Jordan:1934:AGQ,
Taub:1934:DEP,
vonNeumann:1934:APFa,
vonNeumann:1934:APFb,
vonNeumann:1934:HMT,
vonNeumann:1934:MFS,
Bochner:1935:APFa,
Bochner:1935:APFb,
Bochner:1935:CSO,
Jordan:1935:IPL,
vonNeumann:1935:CSI,
vonNeumann:1935:CTSa,
vonNeumann:1935:CTSb,
vonNeumann:1935:DRE,
vonNeumann:1935:NO,
vonNeumann:1935:RGD,
vonNeumann:1935:RRR,
vonNeumann:1935:SSE,
Birkhoff:1936:LQM,
Murray:1936:RO,
vonNeumann:1936:AGQ,
vonNeumann:1936:CG,
vonNeumann:1936:CTR,
vonNeumann:1936:ECG,
vonNeumann:1936:RO,
vonNeumann:1936:RR,
vonNeumann:1936:UHM,
vonNeumann:1936:UIL,
Kuratowski:1937:SAS,
Murray:1937:ROI,
Veblen:1937:GCD,
vonNeumann:1937:ATC,
vonNeumann:1937:CGT,
vonNeumann:1937:CRT,
vonNeumann:1937:OGV,
vonNeumann:1937:QLS,
vonNeumann:1937:SMI,
vonNeumann:1937:TPM,
vonNeumann:1938:IDP,
vonNeumann:1939:FIM,
vonNeumann:1939:RCL,
vonNeumann:1940:DSS,
vonNeumann:1940:EPE,
vonNeumann:1940:LAG,
vonNeumann:1940:MAP,
vonNeumann:1940:ROI,
vonNeumann:1940:TPM,
vonNeumann:1941:AOA,
vonNeumann:1941:DRM,
vonNeumann:1941:FIM,
vonNeumann:1941:GLT,
vonNeumann:1941:MSS,
vonNeumann:1941:OMC,
vonNeumann:1941:SWS,
Chandrasekhar:1942:SGF,
Halmos:1942:OMC,
Hart:1942:TPR,
vonNeumann:1942:APM,
vonNeumann:1942:FRC,
vonNeumann:1942:TDW,
Chandrasekhar:1943:SGF,
Murray:1943:ROI,
vonNeumann:1943:ORC,
vonNeumann:1943:ORS,
vonNeumann:1943:SAP,
vonNeumann:1943:TSW,
Chandrasekhar:1944:SGFa,
Chandrasekhar:1944:SGFb,
vonNeumann:1944:IRS,
vonNeumann:1944:PAN,
vonNeumann:1944:RMS,
vonNeumann:1944:TGE,
Goldstine:1945:PLS,
vonNeumann:1945:FDR,
vonNeumann:1945:FWT,
vonNeumann:1945:MGE,
vonNeumann:1945:RET,
vonNeumann:1945:RIR,
vonNeumann:1945:UVM,
Bargmann:1946:SLS,
Burks:1946:PDL,
Schatten:1946:CSLa,
Schatten:1946:CSLb,
vonNeumann:1946:PLS,
vonNeumann:1946:SBS,
vonNeumann:1946:SSS,
Goldstine:1947:MLA,
Goldstine:1947:PCP,
Ulam:1947:CSD,
vonNeumann:1947:CSD,
vonNeumann:1947:ECP,
vonNeumann:1947:FMM,
vonNeumann:1947:FRR,
vonNeumann:1947:GHS,
vonNeumann:1947:M,
vonNeumann:1947:MP,
vonNeumann:1947:NIM,
vonNeumann:1947:NSP,
vonNeumann:1947:SEN,
vonNeumann:1947:SMN,
vonNeumann:1947:TGE,
Schatten:1948:CSLa,
Schatten:1948:CSLb,
vonNeumann:1948:FRN,
vonNeumann:1948:NMD,
vonNeumann:1948:PCPa,
vonNeumann:1948:PCPb,
vonNeumann:1948:SRN,
vonNeumann:1948:TSD,
vonNeumann:1949:FMM,
vonNeumann:1949:MGQ,
vonNeumann:1949:ROR,
vonNeumann:1949:RTT,
vonNeumann:1949:WCR,
Brown:1950:SGD,
Charney:1950:NIB,
Metropolis:1950:STV,
Reitwiesner:1950:EDM,
Segal:1950:TUR,
vonNeumann:1950:FOV,
vonNeumann:1950:MNC,
Goldstine:1951:NIM,
vonNeumann:1951:DCM,
vonNeumann:1951:DEU,
vonNeumann:1951:FHS,
vonNeumann:1951:GLT,
vonNeumann:1951:SAO,
vonNeumann:1951:VTU,
vonNeumann:1952:DRC,
vonNeumann:1952:FNC,
Gillies:1953:TVP,
vonNeumann:1953:CBN,
vonNeumann:1953:CZS,
vonNeumann:1953:NPD,
vonNeumann:1953:NSC,
vonNeumann:1953:TGEa,
vonNeumann:1953:TGEb,
vonNeumann:1953:TIB,
vonNeumann:1953:TIP,
vonNeumann:1954:NLC,
vonNeumann:1954:NMD,
vonNeumann:1954:NPH,
vonNeumann:1954:RMS,
Wigner:1954:SLT,
Devinatz:1955:PSA,
Dulmage:1955:TFK,
Goldstine:1955:BWC,
vonNeumann:1955:CFE,
vonNeumann:1955:CWS,
vonNeumann:1955:DAW,
vonNeumann:1955:EAN,
vonNeumann:1955:IAE,
vonNeumann:1955:MFQ,
vonNeumann:1955:MPS,
vonNeumann:1956:IRD,
vonNeumann:1956:PLS,
Anonymous:1957:ONJ,
Anonymous:1957:SLW,
Szokefalvi-Nagy:1957:JNW,
vonNeumann:1957:MEH,
vonNeumann:1957:PSS,
Oxtoby:1958:JN,
Tarjan:1958:WJN,
vonNeumann:1958:CB,
vonNeumann:1958:NIC,
Bargmann:1959:TGS,
Blair:1959:SNS,
Goldstine:1959:JMR,
Hajnal:1959:WJN,
Neumann:1959:SNL,
Kato:1960:EIM,
Turing:1960:KMD,
Turing:1960:MLM,
vonNeumann:1960:CG,
vonNeumann:1960:RGG,
Burks:1961:NJN,
vonNeumann:1961:CC,
vonNeumann:1961:CFT,
vonNeumann:1961:SWV,
Holland:1962:OLT,
vonNeumann:1962:IFS,
Goldstine:1963:PLS,
Kovetz:1963:EES,
vonNeumann:1963:DMP,
vonNeumann:1963:GLT,
vonNeumann:1963:PLS,
vonNeumann:1963:VTU,
vonNeumann:1964:MGQ,
vonNeumann:1964:TGE,
vonNeumann:1965:RGG,
Nowak:1966:JND,
vonNeumann:1966:SSG,
Eberl:1967:BRJ,
vanHeijenoort:1967:FGS,
vonNeumann:1967:MGQ,
vonNeumann:1967:SWV,
vonNeumann:1967:TGE,
vonNeumann:1968:MGQ,
Burks:1970:ECA,
Knuth:1970:VNF,
vonNeumann:1970:RGG,
vonNeumann:1970:TGE,
Bell:1971:CSR,
vonNeumann:1971:MGQ,
vonNeumann:1971:TSA,
Wilkinson:1971:MEA,
Benioff:1972:PQM,
Forsythe:1972:NCMa,
Forsythe:1972:NCMb,
Goldstine:1972:CPN,
vonNeumann:1973:SWV,
vonNeumann:1974:DMP,
vonNeumann:1974:TGE,
Lighthill:1976:FHJ,
Backus:1978:CPL,
Abraham-Frois:1979:TVP,
Monahan:1979:ENM,
Aspray:1980:MCC,
Friedrichs:1980:NHS,
Heims:1980:JNN,
Stern:1980:CQD,
Stern:1980:JNI,
Ulam:1980:NIM,
vonNeumann:1980:RGG,
vonNeumann:1980:TGE,
Stern:1981:EUA,
vonNeumann:1981:CGT,
vonNeumann:1981:NPH,
vonNeumann:1981:PLS,
Burks:1982:PDL,
Ulam:1982:BJN,
vonNeumann:1982:FDR,
Legendi:1983:LWJ,
McClelland:1983:RCC,
Kennaway:1984:TSN,
Richtmeyer:1985:SMN,
vonNeumann:1986:RGG,
Williams:1986:WNN,
XXX:1986:JNN,
Backus:1987:CPL,
Center:1987:SJN,
Eckhardt:1987:SUJ,
Goldstine:1987:RED,
Tropp:1987:AIM,
Vonneuman:1987:JNS,
vonNeumann:1987:ITP,
Anonymous:1988:SJN,
Howell:1988:JN,
Schnelle:1988:TNN,
vonNeumann:1988:PLS,
Weiss:1988:BOP,
Aspray:1989:DJN,
Aspray:1989:JNC,
Brink:1989:JNR,
Brunn:1989:AFV,
Ceruzzi:1989:RNB,
Dore:1989:JNM,
Grzesik:1989:NRT,
Hartmanis:1989:GNPa,
Hartmanis:1989:GNPb,
Laffont:1989:EUI,
Nagy:1989:NOC,
Salzman:1989:GSL,
Vonneuman:1989:JNF,
Aspray:1990:JNO,
Aspray:1990:OJN,
Heppenheimer:1990:HNS,
Ceruzzi:1991:RCK,
Ceruzzi:1991:RPI,
Scheibe:1991:JVN,
Vonneuman:1991:JNS,
vonNeumann:1991:FMM,
vonNeumann:1991:RGG,
Hamming:1992:RJN,
Macrae:1992:JN,
Macrae:1992:JNS,
Panday:1992:BRJ,
Weintraub:1992:THG,
Godfrey:1993:CNP,
Hicks:1993:ANC,
Poundstone:1993:PDJ,
Toth:1993:ITH,
vonNeumann:1993:FDR,
Kovacs:1994:JNH,
Macrae:1994:JNM,
DellAglio:1995:DHM,
Herken:1995:UTM,
Israel:1995:MCG,
Kaplansky:1995:CNT,
vonNeumann:1995:NC,
Anonymous:1996:QIO,
vonNeumann:1996:MGQa,
vonNeumann:1996:MGQb,
vonNeumann:1996:PJN,
vonNeumann:1996:TGL,
Emch:1997:FQM,
Kahan:1997:JNL,
Knuth:1997:SA,
Kunze:1997:LCP,
Marchal:1998:JNF,
Northrup:1998:ACP,
vonNeumann:1998:CGF,
Jun:1999:IRN,
Macrae:1999:JNS,
Redei:1999:UPM,
Turing:1999:MLM,
vonNeumann:1999:IM,
vonNeumann:19xx:PSM,
vonNeumann:19xx:PSS,
Pais:2000:GSP,
vonNeumann:2000:CB,
Bub:2001:NTQ,
Israel:2001:MCJ,
Petz:2001:ENN,
Redei:2001:NCQ,
Grier:2003:CJN,
Pellicer:2003:CJN,
Poundstone:2003:DDP,
Brewster:2004:JNM,
Csobadi:2004:SML,
vonNeumann:2004:TGE,
DeWitt:2005:SRI,
Grcar:2005:JNB,
Lax:2005:JNE,
vonNeumannWhitman:2005:LF,
Hargittai:2006:MSF,
Hargittai:2006:OVM,
Israel:2008:MCG,
Dederick:1941:OSB,
Bethe:1944:LSH,
Bethe:1947:BW,
Heywood:1947:WM,
Courant:1948:SFS,
Anonymous:1951:PCA,
Jeffress:1951:CMB,
ASM:1952:MIS,
Leary:1955:UK,
Shannon:1956:AS,
Taub:1961:JNCa,
Taub:1961:JNCb,
Taub:1961:JNCc,
Taub:1962:JNC,
Taub:1963:JNCa,
Taub:1963:JNCb,
vonNeumann:1966:TSR,
Swartzlander:1976:CDD,
Metropolis:1980:HCT,
Randell:1982:ODC,
Chambers:1984:DC,
Anonymous:1987:ATA,
Aspray:1987:PJN,
Herken:1988:UTM,
NGBS:1988:IDC,
Vargha:1988:CBP,
Glimm:1990:LJN,
Brunnstein:1994:IPP,
Arveson:1996:QNP,
Laplante:1996:GPC,
Wahlster:1996:EEC,
Anonymous:1997:NDB,
Esser:2000:WMD,
Frommer:2000:NCL,
McCartney:2001:ETT,
Redei:2001:AGR,
Stone:2004:OAQ}

